Better Trees for Santa Claus

We revisit the problem max-min degree arborescence, which was introduced by Bateni et al. [STOC'09] as a central special case of the general Santa Claus problem, which constitutes a notorious open question in approximation algorithms. In the former problem we are given a directed graph with sources and sinks and our goal is to find vertex disjoint arborescences rooted in the sources such that at each non-sink vertex of an arborescence the out-degree is at least $k$, where $k$ is to be maximized. This problem is of particular interest, since it appears to capture much of the difficulty of the Santa Claus problem: (1) like in the Santa Claus problem the configuration LP has a large integrality gap in this case and (2) previous progress by Bateni et al. was quickly generalized to the Santa Claus problem (Chakrabarty et al. [FOCS'09]). These results remain the state-of-the-art both for the Santa Claus problem and for max-min degree arborescence and they yield a polylogarithmic approximation in quasi-polynomial time. We present an exponential improvement to this, a $\mathrm{poly}(\log\log n)$-approximation in quasi-polynomial time for the max-min degree arborescence problem. To the best of our knowledge, this is the first example of breaking the logarithmic barrier for a special case of the Santa Claus problem, where the configuration LP cannot be utilized.

==> Chernoff_bounds.tex <==
\begin{theorem}[Chernoff-Hoeffding bounds (see e.g.~\cite{chernoff1952measure})]
\label{chernoff}
Let $X=\sum_{i=0}^n X_i$ be a sum of $n$ independent random variables such that each $X_i$ can take values in a range $[0,a]$. We then have the following bound

\begin{equation*}
    \mathbb P \left(X\geq (1+\delta)\mathbb E(X) \right) \leq \exp\left(\frac{-\delta^2\cdot \mathbb E(X)}{a\cdot (2+\delta)} \right).
\end{equation*} for any $\delta>0$.
\end{theorem}

==> LocallyGoodFinal.tex <==
\section{Computing a solution with locally low congestion}\label{sec:locallygood}
The goal of this section is to prove Lemma~\ref{lem:locallygood}. We recall that we are in a layered graph with vertices partitioned into layers $L_0, L_1,\dotsc, L_{h}$ where $h = \log n$. The sources $S$ belong to layer $L_0$ and edges can only go from vertices in some layer $L_i$ to
the next layer $L_{i+1}$. 

In the following we will extensively argue about
paths that start in one of the sources. For the
remainder of the section every path $p$ that
we consider is implicitly assumed to start at one of the sources and then traverse (a prefix of)
the layers one by one.
Slightly abusing notation, we sometimes
use $L_i$ also to denote the set of paths
ending in a vertex of $L_i$, that is,
\begin{equation*}
    \bigcup_{v\in L_i} I(v) \ ,
\end{equation*} 
and $T$ to describe the set of closed paths (recall that those are the paths that end at a sink). Let $P$ refer to the set of all possible paths and notice that by virtue of the layers
we have that $|P| \le n^{h} \le n^{\log n+1}$.
We will now describe
a linear programming relaxation, which goes back to
Bateni et al.~\cite{bateni2009maxmin}. The intuition behind the linear program is to select paths similarly to the way we describe solutions,
see Section~\ref{sec:prelim}.
We have a variable $x(p)$ for each path $p$ that in an integral solution takes value $1$ if the path $p$ is contained in an arborescence and $0$ otherwise.
\begin{align}
    \sum_{q\in C(p)} x(q) &= k \cdot x(p) &\forall p\in P\setminus T \label{eqLP:flowLPdemand}\\
     \sum_{q\in I(v)} x(q) &\leq 1 &\forall v\in V \label{eqLP:flowLPcapacity0}\\
     \sum_{q\in I(v)\cap D(p)} x(q) &\leq x(p) &\forall p\in P,v\in V \label{eqLP:flowLPcapacity}\\
    x((s)) &= 1 &\forall s\in S \label{eqLP:flowLPdemandroot}\\
    x &\ge 0 & 
\end{align}
Here we assume that $k$ is the highest value for which the
linear program is feasible, obtained using
a standard binary search framework.
The first two types of constraints describe that each open
path has many children and each vertex has low congestion
(in fact, no congestion).
Constraint~\eqref{eqLP:flowLPcapacity} comes from a lift-and-project idea.
For integral solutions it would be
implied by the other constraints, but
without it, there
could be situations with continuous variables, where for example we take a path $p$ with only value $1/k$ and then a single child of $q$ with value $1$. Such situations easily lead to large integrality gaps, which we can avoid by this constraint.

Since the graph has $h+1$ many layers, this linear program has $n^{O(h)}$ variables and constraints and therefore can be solved in time $n^{O(h)}$. We refer to this relaxation as the \textit{path LP}. In order to prove Lemma \ref{lem:locallygood}, we will design a rounding scheme. Before getting to the main part of the proof, we will first preprocess the fractional solution to sparsify its support.

\subsection{Preprocessing the LP solution}
Our first step is to sparsify the path LP solution $x$ to get another sparser solution (i.e., with a limited number of non-zero entries). For ease of notation, we might need to take several times a copy of the same path $p\in P$. We emphasize here that two copies of the same path are different objects. To make this clear, we will now have a \textbf{multiset} $P'$ of paths but we will slightly change the parent/child relationship between paths. Precisely, for any path $q'\in P'$ is assigned as child to a \textbf{unique} copy $p'\in P'$ such that $q$ was a child of $p$ in the set $P$. With this slight twist, all the ancestors/descendants relationships extend to multisets in the natural way. For instance, we will denote by $D_{P'}(p)$ the set of descendants of $p$ in the multiset $P'$. Again, the set of closed path in $P'$ will be denoted by $T'$ and $S'$ refers to the sources. We assume that there is a unique copy of the trivial path $(s)\in P'$ for any source $s\in S$.

In this step we will select paths such that each open path
has $k \log^2 n$ children instead of the $k$ children one would expect. However, we use a function $y(p)$ that assigns a
weight to each path and this weight decreases from layer
to layer, modelling that the children are actually picked fractionally each with a $1/4\log^2 n$ fraction of the weight of the parent. Thus, according to weights we are picking only $k/4$ children for each path.

Formally, the preprocessing of the LP will allow us to obtain a multiset of path $P'$ such that 
\begin{align}
    \sum_{q\in C_{P'}(p)} y(q) &= \frac{k}{4} \cdot y(p) &\forall p\in P'\setminus T'\label{eqSparseLP:demand}\\
     \sum_{ q\in I_{P'}(v)} y( q) &\leq 2 &\forall v \in V\label{eqSparseLP:capacity0}\\
     \sum_{ q\in I_{P'}(v)\cap D_{P'}( p)} y( q) &\leq 2y( p) &\forall p\in P',v \in V\label{eqSparseLP:capacity}\\
     \text{where }y(p) &=  \frac{1}{(4\log^2 (n))^i}  & \forall i\leq h, \forall  p\in L_i\label{eqSparseLP:granularity}
\end{align}
\larstodo{Need to verify the new constraint}
We obtain such a solution $y$ in a similar way as the randomized rounding in~\cite{bateni2009maxmin, chakrabarty2009allocating}, which achieves polylogarithmic congestion. 
The fact that we select more paths, but only fractionally
gives us better concentration bounds, which allows us
to lose only a constant congestion here.
For completeness we give
the proof in Appendix~\ref{sec:Sparsify}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The main rounding}
We start this part with the sparse multiset of paths $P'$ with
the properties as above. The discount value $y$ can be thought of fractionality in the sense that each $p\in P'$ is taken to an extend of $y(p)$.
We will proceed to round this fractional solution to an integral solution $Q$ that is \textit{locally nearly good}, a concept we will define formally below. Intuitively, this specifies that
the number of paths that have locally high congestion can be removed with Lemma~\ref{lem:bot-to-top}. 
We fix $\ell=10 \log \log n$ for the rest of this section.
Let $\textrm{cong}(v \mid Q)$ be the global congestion of vertex $v$ induced by $Q$, that is, the number of paths in $Q$ ending in $v$. 
For paths $p\in Q\cup\{\emptyset\}$ and $q\in D_Q(p)$ We denote by $\textrm{cong}_p(q \mid Q)$ the \textit{local congestion} induced on the endpoint of $q$ by descendants of $p$.
We consider all paths descendants of $\emptyset$.

A locally nearly good solution is a multiset of paths $Q\subseteq P'$ (where again every path has a \emph{unique} parent among the relevant copies of the same path) that has the following properties:
\begin{enumerate}
    \item one copy of the trivial path $(s)$ belongs to $Q$ for each source $s\in S$;
    \item every open path has $k/32$ children;
    \item no vertex has global congestion more than $2^{10} \log^3(n)$;
    \item\label{en:local-cong} for every $p\in Q \cup \{\emptyset\}$ and $\ell'\le \ell$ we have
    \begin{equation*}
        |\{q \in D_Q(p, \ell') \mid \mathrm{cong}_p(q \mid Q) > 2^{11} \ell^2\}| \le \frac{1}{\ell^2} \left(\frac{k}{32}\right)^{\ell'} \ .
    \end{equation*}
%    \item For every path $p\in Q$ and $\ell' \le \ell$ we have that
%    \begin{equation*}
%        \left| \{q\in D_{Q}(p, \ell') \mid \textrm{cong}_{p}(q\mid Q)\ge 10^3(\log \log (n))^2 \}\right|\le \frac{|D_Q(p, \ell')|}{\log^{10} (n)} \ .
%    \end{equation*}
\end{enumerate}
From a locally nearly good solution we will then derive
a solution of low local congestion by removing all paths
with high local congestion using bottom to top pruning (Lemma~\ref{lem:bot-to-top}).
Condition~\ref{en:local-cong} is tailored to ensure that the number
of such high local congestion paths is small enough so that the
lemma succeeds.

To obtain such a nearly good solution, we will proceed layer by layer, where the top layers are already rounded integrally and the bottom layers are still fractional (as in the preprocessing). However, unlike the case of the preprocessing, we cannot argue with high probability and union bounds, since some properties we want only deviate from expectation only by $\textrm{poly}(\log\log n)$ factors. To obtain a locally nearly good solution, we will use Lov\'asz Local Lemma (LLL) in every iteration, where one iteration rounds one more layer. In the following, we describe the rounding procedure, the bad events and an analysis of their dependencies and finally we apply LLL.

\paragraph{The randomized rounding procedure.} We proceed layer by layer to round the solution $P'$ (with discount $y$) to an integral solution $Q$. We start by adding a single copy the trivial path $(s)$ for each source $s\in S$ to the partial solution $Q^{(0)}$. Assume we rounded until layer $i$, that is, we selected the final multiset of paths $Q^{(i)}$ to be used from all paths in $L_{\le i}$.

To round until layer $i+1$ we proceed as follows. Every open path $p\in Q^{(i)}\cap L_i$ selects exactly $k/16$ children where the $i$-th child equals $q\in C_{P'}(p)$ with probability equal to 
\begin{equation*}
    \frac{1}{\etienne{k}\log^2 n} = \frac{y(q)}{\sum_{q'\in C_{P'}(p)}y(q')}\ .
\end{equation*}
The selection of each child is independent of the choices made for other children. We then let $Q^{(i+1)}$ be the union of $Q^{(i)}$ and all
newly selected paths.
The reason that each path selects $k/16$ children
instead of the $k/32$ many that were mentioned before is
that we will later lose half of the children.
We will repeat this procedure until reaching the last layer $h$ and we return $Q=Q^{(h)}$.

\paragraph{Definitions related to expected congestion.}
In order for this iterated rounding to succeed we need to
avoid that vertices get high congestion (in the local and the global sense). It is not enough to keep track only of the congestion of vertices
in the next layer that we are about to round, but we also need to maintain that
the expected congestion (over the remaining iterations) remains low on all vertices in later layers. Hence, we will define quantities that
help us keep track of them. To avoid confusion, we remark
that the quantities we
will define do not exactly correspond to the expected congestion of the vertices: notice that we sample less children for each path than $P'$ has.
Intuitively, $P'$ has $k/4$ children per open path (see Equation~\ref{eqSparseLP:demand}), but we only sample $k/16$ many.
The quantities we define below would be the expectations if we would sample $k/4$ children instead. Roughly speaking, this gives us an advantage
of the form that the expectation always decreases by a factor $4$ when
we round one iteration.
Apart from the intuition on the expectation, the definitions also
incorporate a form of conditional congestion, which means that we
consider the (expected) congestion based on random choices made so far.
This is similar to notions that appear in Appendix~\ref{sec:Sparsify} for the preprocessing step.

First, we define the fractional congestion induced by some path $p\in P'$ on a vertex $v\in V$ as follows.
\begin{equation*}
      \textrm{cong}(p,v) := \sum_{q\in D_{P'}(p)\cap I_{P'}(v)} y(q).
\end{equation*}
Using this definition, we will define the conditional fractional congestion at step $i$ induced by $p$ on a descendant $q$ as follows (writing $v_q$ for the endpoint of $q$).
\begin{equation*}
    \textrm{cong}_p(q \mid Q^{(i)}) := \begin{cases}
   |\{q' \in D_{Q^{(i)}}(p)\cap I_{Q^{(i)}}(v_q) \}| & \textrm{if }
    q\in L_{\le i}\\
    \sum_{q'\in D_{Q^{(i)}}(p)\cap L_i} \frac{1}{y(q')} \textrm{cong}(q',v_q)  & \textrm{otherwise.}
    \end{cases}
\end{equation*}
We will use this definition only for $p\in Q^{(i)}$. If $v_q$ belongs to one of the first $i$ layers (i.e., $v_q$ is in the integral part corresponding to the partial solution), this is simply the number of descendants of $p\in Q^{(i)}$ in our partial solution that end at $v_q$. Otherwise, this is the total fractional congestion induced by all the paths that we actually selected in our partial solution $q\in Q^{(i)}\cap L_i$ and that are descendants of $p$. The name \textit{conditional} comes from the term $1 / y(q')$ which is simply the fact that we condition on having already selected the path $q'$ once integrally.
The global congestion at step $i$ on a vertex $v\in V$ is defined similarly with
\begin{equation*}
    \textrm{cong}(v\mid Q^{(i)}) := \begin{cases}
     |\{q \in Q^{(i)}\cap I(v)\}| & \textrm{if }
    v\in L_{\le i}\\
    \sum_{q\in Q^{(i)}\cap L_i} \frac{1}{y(q)} \textrm{cong}(q,v)  & \textrm{otherwise.}
    \end{cases}
\end{equation*}

\paragraph{The first type of bad event: global congestion.} The naive way to bound the global congestion would be to simply to bound the global congestion on each vertex and make a bad event from exceeding this. However, to manage dependencies between bad events and get better concentration bounds, we partition the set of paths according to how much fractional load their ancestors are expected to put on $v$ and then bound the congestion incurred by each group on $v$. More precisely, assume we rounded until layer $i$ and are now trying to round until layer $L_{i+1}$. Consider any vertex $v\in L_{\ge i+1}$. The decisions made in this step
of the rounding concern which paths in $L_{i+1}$ will be selected.
Fix an integer $t\ge 0$ and and let $P^{(i+1)}_{v,t}$ to be the set of all paths $p \in L_{i+1}$ such that 
\begin{equation*}
    \frac{\textrm{cong}(p,v)}{y(p)} \in ((\beta_{t+1})^{-1},(\beta_{t})^{-1}],
\end{equation*}
where $\beta_{t} = 2^{t-1}$ (we use $\beta_t$ for clarity of notations later).

We define the bad event $\mathcal B_1(p, v)$ as the event that
\begin{equation*}
    \sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em} \frac{\mathrm{cong}(p, v)}{y(p)}  > 2 \mathbb E\bigg[\sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em}\frac{\mathrm{cong}(p, v)}{y(p)}\bigg] + 2^{10} \log n \ .
\end{equation*}
Since $P^{(i+1)}_{v,t}$ partitions the paths in $L_{i+1}$, the bad events
for all $t$ together will bound the increase in the congestion on $v$:
this is because $\mathrm{cong}(v \mid Q^{(i+1)}) = \sum_{p\in Q^{(i+1)}\cap L_{i+1}} \mathrm{cong}(p, v) / y(p)$.

At this point, it is worthwhile to mention that $t$ can only take values in $\{0,1,\dotsc,\log^2 n\}$.
Indeed, by Constraint~\eqref{eqSparseLP:capacity} we have that
\begin{equation*}
    \frac{\textrm{cong}(p,v)}{y(p)} \le 2
\end{equation*}
is ensured for all $p\in P'$. Moreover, we notice that $y$ has a low granularity (i.e. $y$ satisfies Equation \eqref{eqSparseLP:granularity}) which implies that either $ \textrm{cong}(p,v)=0$ or
\begin{equation*}
 \frac{\textrm{cong}(p,v)}{y(p)} \ge \frac{1}{(4\log^2 n)^{h-|p|}}\ge \frac{1}{(4\log^2 n)^{h}}\ .
\end{equation*}
Hence bad events $\mathcal B(v,t)$ will be instantiated only for $t= 0,1,\dotsc,\log^2 n$ (assuming here that $n$ is sufficiently large).



%%%%%%%%%%%
\begin{comment}
For a path $p\in L_{i+1}$, we define $N_p$ to be the number of copies of $p$ that are selected in $Q^{(i+1)}$. 
\begin{equation*}
    C_{v,t}:=\sum_{p \in P_{v,t}\cap L_{i+1}} N_p\cdot \frac{\textrm{cong}(p,v)}{y(p)} \ ,
\end{equation*}
i.e. the fractional load on vertex $v\in L_{\ge i+1}$ that is induced by paths actually selected in $Q^{(i+1)}\cap L_{i+1}$ (counted with multiplicity). Note that $C_{v,t}$ is a random variable depending on the random choices that are made to round from layer $i$ to layer $i+1$. We also notice that $C_{v,t}$ can be written as a sum of independent random variables that each take value in $\{0\}\cup (2^{-(t+1)},2^{-t}]$. Given this, we define
$\mathcal B(v,t)$ as the bad event that 
\begin{equation*}
    C_{v,t} \ge 2\mathbb E [C_{v,t}]+100 \log (n)\ .
\end{equation*}
We prove below that if these bad events do not happen then we maintain the following low global congestion property for any vertex $v\in V$.
\begin{equation}
\label{eq:lowcongestion_partialrounding}
    \textrm{cong}(v\mid Q^{(i+1)})\le 1500\log^3(n).
\end{equation} 
Towards this, we define $N_q$ to be the number of copies of $q\in P'$ that are selected during the rounding. Denote by $P(q)$ the parent of $q$ in $P'$. Then note that each path $q$ is selected in expectation 
\begin{equation*}
    \frac{k}{100}\frac{y(q)}{\sum_{q'\in C_(P(q))} y(q')} = \frac{y(q)}{25y(C(q))}
\end{equation*} times by its parent $C(q)$ (here we used constraint \eqref{eqSparseLP:demand} of the path LP). Hence we can compute
\begin{align*}
    \mathbb E[\textrm{cong}(v\mid Q^{(i+1)})] &= \sum_{p\in Q^{(i)}\cap L_i} \left[\sum_{q\in D_{Q^{(i+1)}}(p)\cap L_{i+1}} \mathbb E[N_{q}] \cdot \frac{ \textrm{cong}(q,v)}{y(q)}\right]\\
    &= \sum_{p\in Q^{(i)}\cap L_i} \left[\sum_{q\in D_{Q^{(i+1)}}(p)\cap L_{i+1}} N_{p}\cdot \frac{y(q)}{25y(p)} \cdot \frac{ \textrm{cong}(q,v)}{y(q)}\right]\\
     &= \frac{1}{25}\sum_{p'\in Q^{(i)}\cap L_i}N_p \left[ \frac{\sum_{q\in D_{Q^{(i+1)}}(p)\cap L_{i+1}}  \textrm{cong}(q,v)}{y(p)}\right]\\
   &= \frac{1}{25}\sum_{p\in Q^{(i)}\cap L_i} N_p\left[ \frac{\textrm{cong}(p,v)}{y(p)}\right]\\
    &= \frac{\textrm{cong}(v\mid Q^{(i)})}{25}\ .
\end{align*} 
Therefore if no bad event $\mathcal B(v,t)$ happened before step $i$, and none happens at step $i+1$, we maintain Equation \eqref{eq:lowcongestion_partialrounding} with the following calculation.
\begin{equation*}
    \textrm{cong}(v\mid Q^{(i+1)}) \le \sum_{t=0}^{10\log^2(n)}2\mathbb E[ C_{v,t}] + 100\log(n) \le \frac{\textrm{cong}(v\mid Q^{(i)})}{25} + 10^3 \log^3 (n) \le 1500 \log^3(n).
\end{equation*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%


\begin{lemma}\label{lem:iterlowcong}
  Assuming no bad event $\mathcal B_1(v, t)$ has occurred in any iteration up
  to $i$, we have for every $v$ that
  \begin{equation*}
      \mathrm{cong}(v \mid Q^{(i)}) \le 2^{11} \log^3 n \ .
  \end{equation*}
\end{lemma}
\begin{proof}
  We argue inductively. For $i = 0$ we have
  \begin{equation*}
      \mathrm{cong}(v \mid Q^{(i)}) = \sum_{p\in Q^{(i)}\cap L_i} \frac{\mathrm{cong}(q, v)}{y(q)} = \sum_{s\in S} \mathrm{cong}((s), v) = \sum_{p\in I_{P'}(v)} y(v) \le 2 \ . 
  \end{equation*}
  Now assume that for $i \ge 0$ we have
  \begin{equation*}
      \mathrm{cong}(v \mid Q^{(i)}) \le 2^{11} \log^3 n \ .
  \end{equation*}
  Since the congestion of any $v\in L_{\le i}$ cannot change anymore,
  we may assume w.l.o.g.\ that $v\in L_{\ge i+1}$.
  For each $t$ let
  \begin{equation*}
      \mu_t = \mathbb E\bigg[\sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em}\frac{\mathrm{cong}(p, v)}{y(p)}\bigg] \ .
  \end{equation*}
  Then $\sum_t \mu_t = 1/4 \cdot \mathrm{cong}(v \mid Q^{(i)}) \le 2^{9} \log^3 n$. To see this, denote by $N^{(i)}_q$ the number of copies of a path $q\in P'$ that is selected in $Q^{(i)}$. As a shorthand, we write $P(q)$ for the parent of $q$ in $Q^{(i+1)}$. By linearity of expectation we can write
  \begin{align*}
      \sum_t \mu_t &= \sum_t \ \mathbb  E\bigg[\sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em}\frac{\mathrm{cong}(p, v)}{y(p)}\bigg]\\
      &=  \sum_t \ \mathbb  E\bigg[\sum_{p\in P' \cap P^{(i+1)}_{v,t}} \hspace{-1em}N^{(i+1)}_p\cdot \frac{\mathrm{cong}(p, v)}{y(p)}\bigg]\\
      &=  \sum_t  \sum_{p\in P' \cap P^{(i+1)}_{v,t}} \hspace{-1em}\mathbb E[N^{(i+1)}_p]\cdot \frac{\mathrm{cong}(p, v)}{y(p)}\\
      &=  \sum_t  \sum_{p\in P' \cap P^{(i+1)}_{v,t}} \  \frac{(k/16)\cdot y(p)}{(k/4)\cdot y(P(p))}\cdot \frac{\mathrm{cong}(p, v)}{y(p)}\\
      &= \frac{1}{4}\cdot \bigg[\sum_t  \sum_{p\in P' \cap P^{(i+1)}_{v,t}} \ \frac{\mathrm{cong}(p, v)}{y(P(p))}\bigg]\\
      &= \frac{1}{4}\cdot \bigg[\sum_t  \sum_{p\in P' \cap P^{(i)}_{v,t}} \ \frac{\mathrm{cong}(p, v)}{y(p)}\bigg] =  (1/4) \cdot \mathrm{cong}(v \mid Q^{(i)})\le 2^{9} \log^3 n\ .
  \end{align*}
  It follows that
  \begin{align*}
      \mathrm{cong}(v \mid Q^{(i+1)}) &= \sum_{p\in Q^{(i+1)}} \frac{\mathrm{cong}(p,v)}{y(p)} \\
      &= \sum_{t} \sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \frac{\mathrm{cong}(p,v)}{y(p)} \\
      &\le \sum_{t} [2 \mu_t + 2^{10} \log n] \\
      &\le 2^{10} \log^3 n + 2^{10} \log^3 n \\
      &\le 2^{11} \log^3 n \ . \qedhere
  \end{align*}
\end{proof}

\paragraph{The second type of bad event: Local congestion at the sources.}
Although the type of bad event we define here is to limit the
local congestion at the first layers, some of the definitions are made
more generally to be applied also for local congestion at later layers in the subsequent bad events.
Recall that we want to bound the congestion between
close descendants of some path.
Let $\ell'\le \ell$ and $p\in Q^{(i)}\cap L_{i'}$, where $i - \ell' \le i'\le i$.
Consider the set $D_{P'}(p,\ell')$. The potential descendants of $p$ in the solution we are constructing ($\ell'$ layers away) must all come from this set.
Notice that by sparsity of $P'$ we have
\begin{equation*}
    |D_{P'}(p,\ell')| \le (k \log^2 n)^{\ell'} \ .
\end{equation*}
It is our goal to achieve that only a small fraction of these will
get high local congestion in the next rounding step.
In a similar spirit as global congestion events, we partition the sources $s'$ according to how much their descendants intersect with the descendants of $s$. For any $s\in S$, let $S(s, t, \ell')$ be the set of sources $s'\in S$ with
\begin{equation*}
    |V(D_{P'}((s),\ell')) \cap V(D_{P'}((s'),\ell'))| \in \left((\alpha_{t+1})^{-1}\cdot (k \log^2 n)^{\ell'} ,(\alpha_t)^{-1}\cdot  (k \log^2 n)^{\ell'} \right],
\end{equation*}
where $\alpha_t= \etienne{TBD}$ for any $t\ge 0$. Here $V(\cdot)$ denotes the end vertices of the given paths. Note that we will be only interested in sources $s'$ such that $|V(D_{P'}((s),\ell')) \cap V(D_{P'}((s'),\ell'))|\neq 0$ and therefore we instantiate the above definition only for $0\le t\le \etienne{TBD} \le \ell$.

The separation of sources is to exploit better concentration in the case that
the descendants of one source intersect only little with the descendants of the other source.
We define
\begin{align*}
    N^{(i+1)}(s, t, \ell') = |\{q\in D_{P'}((s),\ell') \mid \ &\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i)}) \le 2^{10} \ell^2 \\ &\text{and } \sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i+1)}) > 2^{10} \ell^2\}| \ .
\end{align*}
These are the number of vertices with newly high local congestion (counting only the congestion induced by descendants of paths in $S(s, t, \ell')$).
We now define bad events
for every source $s\in S$, $t=0,1,\ldots, \ell$, and
each $\ell' \le \ell$. The event  $\mathcal B_2((s), t, \ell')$ 
describes that
\begin{equation*}
    N^{(i+1)}(s, t, \ell') > \frac{1}{\log^{10} n} \left(\frac{k}{32}\right)^{\ell'} \ .
\end{equation*}
Similar events for $p$ with $|p| > 1$ will be relevant
as well, but we will need to slightly tweak some definitions in order to be able to amplify their probability enough.
\paragraph{The third type of bad event: Local congestion for non-source paths.}
For this last type of bad event, we define for any path $p\in Q^{(i)}$
\begin{align*}
    N^{(i+1)}(p, \ell') = |\{q\in D_{P'}((s),\ell') \mid \ &\mathrm{cong}_{p}(q \mid Q^{(i)}) \le 2^{10} \ell^2 \\ &\text{and } \mathrm{cong}_{p}(q \mid Q^{(i+1)}) > 2^{10} \ell^2\}| \ .
\end{align*}

Note that this is a similar notation as for events of the second type, except that we count the congestion only induced by descendants of $p$ in a strict sense. If $t$ is not in argument, the number $N^{(i+1)}$ will implicitly mean that we sum the induced congestion by strict descendants.


For any $p\in L_{i'}\cap Q^{(i)}$ where $i - \ell - 1 \le i' \le i - 1$, and $t\ge 0$, we define the set of \emph{marked} children of $p$ at step $i+1$ as the set $M^{(i+1)}(p)$ of all $q \in C_{Q^{(i)}}(p)$ such that
\begin{equation*}
    N^{(i+1)}(p, \ell') > \frac{1}{\log^{10} n} \left(\frac{k}{32}\right)^{\ell'}
\end{equation*}
for at least one $\ell' \le \ell$. Notice that the children of $p$ (in $Q^{(i)}$) are
already determined because $p$ is in $L_{\le i - 1}$.
We are now ready to state the third type of bad event. We define the bad event $\mathcal B_3(p)$ for any $p\in L_{i'}$ where $i - \ell -1 \le i' \le i - 1$, as the event that 
\begin{equation*}
    |M^{(i+1)}(p)|\ge \frac{1}{\ell^3} \cdot \frac{k}{16} \ ,
\end{equation*}
which means that a lot of children selected by $p$ become marked at step $i+1$. As we will ensure that this bad event never happens, we can guarantee that a large fraction of children $q$ of each path $p$ always satisfies that $N^{(i+1)}(p, \ell')$ is low for all $\ell'\le \ell$.
As we explain later, we will simply remove all other children and this way indirectly
prevents of having too many locally congested descendants for all the remaining paths. The advantage
of this indirect method is that we can apply good concentration bounds
on the children and thereby amplify the probability.

%\paragraph{A third type of bad event: Preserving the source path $(s)$.}\todo{here does not work for multiple sources} Because our algorithm will delete in the end all the paths that have been marked in some round, we need to ensure that the source path $(s)$ is not marked in any relevant round. Hence for the first $\ell$ steps of rounding, we define a single bad event $\mathcal B (s)$ that is that $(s)$ is marked during this step. Note that this new definition overrules the previous definition of $\mathcal B(s)$.

\paragraph{The probabilities of the bad events.} In this part, we derive upper bounds for the probability of each bad event.
Some bounds are sub-optimal to simplify later formulas.
\begin{lemma}
For any $v\in V$ and integer $t$ we have that
\begin{equation*}
    \mathbb P[\mathcal B_1(v,t)]\leq n^{-10 \cdot \beta_{t}} \ .
\end{equation*}
\end{lemma}
\begin{proof} We need to prove that
\begin{equation*}
    \mathbb P\Bigg[\sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em} \frac{\mathrm{cong}(p, v)}{y(p)}  > 2 \mathbb E\bigg[\sum_{p\in Q^{(i+1)} \cap P^{(i+1)}_{v,t}} \hspace{-1em}\frac{\mathrm{cong}(p, v)}{y(p)}\bigg] + 2^{10} \log n\Bigg]
    \le n^{-10 \cdot \beta_{t}} \ .
\end{equation*}
Notice that $\mathrm{cong}(p, v) / y(p)$ is upper bounded by $(\beta_{t})^{-1}$ by definition of $P^{(i+1)}_{v,t}$ and the sum can be
rewritten as a sum over the paths chosen in iteration $i+1$, where a path $p$
contributes $\mathrm{cong}(p, v) / y(p)$ to the sum.
These paths are chosen independently and
thus by a standard Chernoff bound we obtain that the probability is at most 
\begin{equation*}
    \exp\left( \frac{-2^{10} \log n}{2 \cdot (\beta_{t})^{-1}}\right)\le n^{-10 \cdot \beta_{t}} \ . \qedhere
\end{equation*}
\end{proof}

Before moving forward with other events, we prove here a simple upper bound on $|S(s,t, \ell')|$ that will be helpful in many other lemmas.
\begin{lemma}
\label{lem:S_B_upperbound}
For any source $s\in S$ and distance $\ell'$, we have that
\begin{equation*}
    |S(s,t,\ell')|\le \alpha_{t+1}(\log n)^{3\ell}\ .
\end{equation*}
\end{lemma}
\begin{proof}
By Constraint~\eqref{eqSparseLP:demand} we have that $|V(D_{P'}((s),\ell'))| \le |D_{P'}((s),\ell')| \le (k\log^2 n)^{\ell'}$ for any $s\in S$.
  Now let $v\in V(D_{P'}((s'),\ell'))$ for some $s'\in S$. Then by Constraints~\eqref{eqSparseLP:capacity0} and \eqref{eqSparseLP:granularity} there are at most
  $2 (4\log^2 n)^{\ell'}$ many paths in $\cup_{s'\in S}D_{P'}((s'))$ that end in $v$. Hence in total at most
  \begin{equation*}
      2 (4\log^2 n)^{\ell'} \cdot (k\log^2 n)^{\ell'}
  \end{equation*}
  many paths from $\cup_{s'\in S}D_{P'}((s'))$ end in $V(D_{P'}((s),\ell'))$.
  Each source in $S(s, t, \ell')$ accounts for at least $(\alpha_{t+1})^{-1}\cdot (k\log^2 n)^{\ell'}$
  many of these paths. 
  
  It follows that (for $n$ big enough)
  \begin{equation*}
      |S(s, t, \ell')| \le \frac{2 (4\log^2 n)^{\ell'} \cdot (k\log^2 n)^{\ell'} }{(\alpha_{t+1})^{-1}\cdot (k\log^2 n)^{\ell'}} \le \alpha_{t+1} (\log n)^{3\ell} \ . \qedhere
  \end{equation*}
\end{proof}



\begin{lemma}\label{lem:problocal}
Assume no bad event happened until the current iteration of rounding. Let $\ell' \le \ell$, $s\in S$, and $t\ge 0$.
Then
\begin{align}
    \mathbb P[N^{(i+1)}(s, t, \ell') > (1/\log^{10} n) \cdot (k / 32)^{\ell'}] &\le (\log n)^{-40\ell}\textrm{, and}\\
    \mathbb P[N^{(i+1)}(s, t, \ell') > (1/\log^{10} n) \cdot (k / 32)^{\ell'}] &\le (\log n)^{-10\ell}\exp\left(-\frac{\alpha_t}{(\log n)^{7\ell}}\right) \textrm{ if $t\ge 1$}\ .
\end{align}
In particular,
\begin{align}
    \mathbb P[\mathcal B_2((s), t, \ell')] &\le (\log n)^{-40\ell}\textrm{, and}\\
    \mathbb P[\mathcal B_2((s), t, \ell')] &\le (\log n)^{-10\ell}\exp\left(-\frac{\alpha_t}{(\log n)^{7\ell}}\right) \textrm{ if $t\ge 1$}\ .
\end{align}
for any $s\in S$. Moreover for any $p\in Q^{(i)}$, and $\ell'\le \ell$,
\begin{equation*}
    \mathbb P[N^{(i+1)}(p,\ell')\ge (1/\log^{10}n)\cdot (k/32)^{\ell'}]\le (\log n)^{-40\ell}\ . 
\end{equation*}
\end{lemma}
\begin{proof} Recall that we are bounding the number of descendants of $s$ that
had low local congestion of at most $2^{10} \ell^2$ before, but now
get high local congestion.
More concretely,
consider some $q\in D_{P'}((s), \ell')$ with $\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i)}) \le 2^{10}\ell^2$.
Then
\begin{equation*}
    \mathbb E\bigg[\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i+1)})\bigg] = \frac{1}{4} \sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i)}) \le 2^8 \ell^2 \ .
\end{equation*}
Further, $\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i+1)})$
can be decomposed into a sum of
independent random variables bounded by $2$. Indeed, recalling the definition of $\mathrm{cong}_{(s')}(q \mid Q^{(i+1)})$ we see that the quantity $\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i+1)})$ can be written as a sum over a certain multiset of chosen paths $q'$ of the value $\frac{\mathrm{cong}_{q'}(q \mid Q^{(i+1)})}{y(q')}$. Constraint \eqref{eqSparseLP:capacity} of the path LP ensures that this is always less than 2. Those variables are independent because of the randomized rounding that selects children independently of each other.
Hence, by a Chernoff bound we have
\begin{equation*}
    \mathbb P\bigg[\sum_{s'\in S(s, t, \ell')} \mathrm{cong}_{(s')}(q \mid Q^{(i+1)}) > 2^{10} \ell^2\bigg] \le \exp(-2^8\ell^2) \ .
\end{equation*}
Therefore
\begin{equation*}
    \mathbb E[N^{(i+1)}(s, t, \ell')] \le \frac{(k\log^2 n)^{\ell'}}{\exp(2^8\ell^2)} \le \frac{1}{(\log n)^{2^8\ell}} \left(\frac{k}{32}\right)^{\ell'} \ .
\end{equation*}
By Markov's inequality, we obtain easily that
\begin{equation*}
    \mathbb P[N^{(i+1)}(s, t, \ell') > (1/\log^{10} n) \cdot (k / 32)^{\ell'}] \le (\log n)^{-40\ell}\ .
\end{equation*}
By exactly the same argument we obtain the same upper-bound for $\mathbb P[N^{(i+1)}(s, t, \ell') > (1/\log^{10} n) \cdot (k / 32)^{\ell'}]$.
Then we prove a bound that will be better for $t$ greater than some threshold. We remark that there are at most $(2 (4\log^2 n)^{\ell'})\cdot (2^{11}\log^3 n)$ sources $s'\in S$,
on which the local congestion of each $q\in D_{P'}((s), \ell')$
can depend (by Constraints~\eqref{eqSparseLP:capacity} and~\eqref{eqSparseLP:capacity0} as well as Lemma \ref{lem:iterlowcong}). At the same time each source in $S(s, t, \ell')$ can only affect the congestion of $(\alpha_t)^{-1} (k\log^2 n)^{\ell'}$ many descendants of $(s)$ by definition.
It follows that $N^{(i+1)}(s, t, \ell')$ is the sum of $|D_{P'}((s),\ell')|$
many $0/1$ random variables where each variable depends
on at most 
\begin{equation*}
    (2 (4\log^2 n)^{\ell'})\cdot (2^{11}\log^3 n)\cdot ((\alpha_t)^{-1} (k\log^2 n)^{\ell'})\le (\alpha_t)^{-1}(k\log^5 n)^{\ell'}
\end{equation*}
other variables (for $n$ greater than a sufficiently large constant).
Hence with Lemma~\ref{lem:ChernoffDepend} we get (for $t\ge 1$)
\begin{align*}
    \mathbb P[N^{(i+1)}(s, t, \ell') > (1/\log^{10} n) \cdot (k / 32)^{\ell'}] &\le (\alpha_t)^{-1}(k\log^5 n)^{\ell'} \exp\left(-\frac{(1/\log^{10} n) \cdot (k / 32)^{\ell'}}{(\alpha_t)^{-1}(k\log^5 n)^{\ell'}}\right)\\
    &\le  (\alpha_t)^{-1}(k\log^5 n)^{\ell'} \exp\left(-\frac{\alpha_t}{(\log^{6} n)^{\ell'}} \right)\\
    &\le (\log n)^{-10\ell}\exp\left(-\frac{\alpha_t}{(\log^{7} n)^{\ell}}\right)\ .
\end{align*}
For the last step, we used the fact that if $t\ge 1$, then $\alpha_t\ge (\log n)^{20\ell}$.
\end{proof}



Next, we upper-bound the probability of $\mathcal B_3(p)$.

\begin{lemma}
Assume no bad event happened until the current iteration of rounding. Let $p \in L_{i'}$ where $i - \ell - 1 \le i' \le i - 1$.
Then we have that
\begin{equation*}
    \mathbb P[\mathcal B_3(p)]\le \exp\left(-\sqrt{k} \right) \ .
\end{equation*}
\end{lemma}
\begin{proof} To prove this, note that a child $q$ of $p$ (in the set $ Q^{(i)}$) is marked \textbf{independently} of other children of $p$. This is because $q$ being marked depends only on the random choices made by descendants of $q$, which are independent of descendants of other children of $p$. Therefore using Lemma \ref{lem:problocal} and a standard union bound we obtain that each child of $p$ is marked independently with probability at most $\ell \cdot (\log n)^{-40\ell}$. Note that $p$ has $k/16$ children in $Q^{(i)}$ therefore the probability that more than $(1/\ell^3)\cdot (k/16)$ of them are marked is at most (recall that $k\ge 2^{10} (\log\log n)^6\ge (32\ell^3)^2$)  
\begin{equation*}
    \exp\left(- \frac{k}{32\ell^3}\right)\le  \exp\left(- \sqrt{k}\right)\ . \qedhere
\end{equation*}



%%%%%%%%%%%
\begin{comment}
For the second claim, we first note that for a fixed path $p$ and distance $\ell'\le \ell$, any path $q$ ending in $v_q$ that does not belong to $B_{p,\ell'}^{(i)}$ must satisfy 
\begin{equation*}
    \textrm{cong}_p(q\mid Q^{(i)})\le (10^3 \log\log(n))^2,
\end{equation*} by definition. Furthermore, the random variable
\begin{equation*}
     \textrm{cong}_p(q\mid Q^{(i+1)}) = \sum_{q'\in D_{Q^{(i+1)}}(p)\cap L_{i+1}} \frac{ \textrm{cong}(q',v_q)}{y(q')}
\end{equation*} can be written as a sum of independent random variables that can take value at most 2 (again using Constraint \eqref{eqSparseLP:capacity} of the path LP). Moreover, when a sampled path $p'\in L_i$ chooses its children in $L_{i+1}$, each such path $q'\in L_{i+1}$ is chosen in expectation
\begin{equation*}
    \frac{k}{100} \cdot \frac{y(q')}{\sum_{q''\in C_{P'}(p')}y(q'') }= \frac{k}{100}\cdot  \frac{y(q')}{(k/4)\cdot y(p')} = \frac{y(q')}{25y(p')}\ .
\end{equation*} (using constraint \eqref{eqSparseLP:demand}). Let us call $N_{q'}$ the number of times a path $q\in L_{\ell+1}$ is taken in the process as a child of a fixed $p'$. Putting everything together, we can compute by linearity of expectation that
\begin{align*}
    \mathbb E[\textrm{cong}_p(q\mid Q^{(i+1)})] &= \sum_{p'\in D_{Q^{(i)}}(p)\cap L_i} \left[\sum_{q'\in D_{Q^{(i+1)}}(p')\cap L_{i+1}} \mathbb E[N_{q'}] \cdot \frac{ \textrm{cong}(q',v_q)}{y(q')}\right]\\
    &= \sum_{p'\in D_{Q^{(i)}}(p)\cap L_i} \left[\sum_{q'\in D_{Q^{(i+1)}}(p')\cap L_{i+1}} \frac{y(q')}{25y(p')} \cdot \frac{ \textrm{cong}(q',v_q)}{y(q')}\right]\\
     &= \frac{1}{25}\sum_{p'\in D_{Q^{(i)}}(p)\cap L_i} \left[ \frac{\sum_{q'\in D_{Q^{(i+1)}}(p')\cap L_{i+1}}  \textrm{cong}(q',v_q)}{y(p')}\right]\\
   &= \frac{1}{25}\sum_{p'\in D_{Q^{(i)}}(p)\cap L_i} \left[ \frac{\textrm{cong}(p',v_q)}{y(p')}\right]\\
    &= \frac{\textrm{cong}_p(q\mid Q^{(i)})}{25}\ .
\end{align*}
Hence the random variable $\textrm{cong}_p(q\mid Q^{(i+1)})$ has expectation at most $10^4 (\log \log (n))^2$ and is written as a sum of independent random variables that take value at most $2$. By a standard Chernoff bound, the probability that a path $q$ belongs to $B_{p,\ell'}^{(i+1)}\setminus B_{p,\ell'}^{(i)}$ is at most 
\begin{equation*}
    \exp(-100 (\log \log(n))^2).
\end{equation*}
Now fix a path $p'$. To be marked at step $i+1$, it must be (by definition) that 
\begin{equation*}
    \left| B_{p,\ell'}^{(i+1)}\setminus B_{p,\ell'}^{(i+1)} \right| \ge \frac{100(\log \log (n))^2}{\exp(100(\log \log (n)^2)}\cdot \left(k\log^2(n)\right)^{\ell'}.
\end{equation*} 
However, $p'$ has only at most $\left(k\log^2(n)\right)^{\ell'}$ potential descendants (i.e. descendants paths $q\in P'$ that have $|q|=|p'|+\ell'$ and $y(q)\neq 0$). Hence, for $p'$ to be marked at step $i+1$, it must be that the value $\left| B_{p',\ell'}^{(i+1)}\setminus B_{p',\ell'}^{(i)} \right|$ exceeds its expectation by a multiplicative factor of at least $100(\log \log (n))^2$. By Markov's inequality, this can happen only with probability at most 
\begin{equation*}
    \frac{1}{100 (\log \log (n))^2}\ .
\end{equation*}
This already proves that 
\begin{equation*}
    \mathbb P[\mathcal{B}(s)]\le \frac{1}{100(\log \log(n))^2}\ .
\end{equation*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
A child $q\in C_{Q^{(i)}}(p)$ will not be $t$-marked if
$N^{(i+1)}(q, t, \ell') \le 1/(\log^{10} n) \cdot (k/32)^{\ell'}$ for all $\ell'\le \ell$.

Hence, let $\ell' \le \ell$ and consider first $N^{(i+1)}_S(q, t, \ell')$ for the children $q$. By Lemma~\ref{lem:problocal} we have that
$\mathbb P[N^{(i+1)}_S(q, \ell') > (1/\log^{10} n) \cdot (k/32)^{\ell'}] \le (k\log n)^{-40\ell}$. Thus, by Markov's inequality we get
\begin{equation*}
    \mathbb P\left[|\{q\in C_{Q^{(i)}}(p) \mid N^{(i+1)}_S(q, \ell') > 1/\ell^2 \cdot (k/32)^{\ell'}\}| > \frac{1}{2\ell^3} \frac{k}{16}\right]
    \le \frac{1}{2\ell} (k \log n)^{-30\ell} \ .
\end{equation*}
Next consider $N^{(i+1)}_B(q, \ell')$. We have that this random variable depends
only on elements of $S_B(q, \ell')$. Notice that $|S_B(q, \ell')| \le (\log n)^{10\ell}$ \etienne{by Lemma \ref{lem:S_B_upperbound}}. \larstodo{TODO: it is explained in a later lemma}
In particular, the event that $N^{(i+1)}_B(q, \ell') > 1/\ell^2 \cdot (k/32)^{\ell'}$
depends only on the same event for $(\log n)^{10\ell}$ many other children. \etienne{The probability of a single one of those events is at most $(\log n)^{-40\ell}$ by Lemma \ref{lem:problocal}. Hence in expectation there are at most $(k/16)\cdot (\log n)^{-40\ell}$ children of $p$ such that $N^{(i+1)}_B(q, \ell') \ge 1/\ell^2 \cdot (k/16)^{\ell'}$.} We apply Lemma~\ref{lem:ChernoffDepend} and get
\begin{align*}
    &\mathbb P\left[|\{q\in C_{Q^{(i)}}(p) \mid N^{(i+1)}_B(q, \ell') > 1/\ell^2 \cdot (k/32)^{\ell'}\}| > \frac{1}{2\ell^3} \frac{k}{16}\right] \\
    &\le \frac{1}{2\ell} (k \log n)^{-30\ell} \ .
\end{align*}
By taking a union bound over $N_S, N_B$ and all values of $\ell'$ we
get that the probability any of these bounds is exceeded is at most $(k\log n)^{-30\ell}$.
If none of these bounds are exceeded, at most $2\ell \cdot (1/2\ell^3) \cdot (k/16)$ children can be marked, which completes the proof.
\end{comment}
%%%%%%%%%%%%%%%%%%%%
\end{proof}

\paragraph{The dependencies of the bad events.}
For any bad event $\mathcal B$ we define $\Gamma_1(\mathcal B)$ to be the set of bad events of the first type $\mathcal B_1(v,t)$ that depend on the bad event $\mathcal B$. Similarly, let $\Gamma_{(2,t)}(\mathcal B)$ the set of bad events $B_2((s),t'=t,\ell')$ that depend on $\mathcal B$ and $\Gamma_3(\mathcal B)$ be the sets of bad events of the third type that depend on $\mathcal B$.
We will also write $\Gamma_{(2,t),3}(\mathcal B)$ (and similarly for other
combinations) as the union of the corresponding dependent events. 
We will now upper bound the cardinality of these sets.
We remark that the focus here is on simplicity of the terms rather
than optimizing the precise bounds.
\begin{lemma}
For any bad event $\mathcal B$, we have that
\begin{equation*}
    |\Gamma_1(\mathcal B)|\leq n^2 \ .
\end{equation*}
\end{lemma}
\begin{proof}
The statement holds trivially, since there are at most $n\cdot (1 + \log^2 n)\le n^2$ bad events of the first type in total ($n$ possibilities of the choice of vertex $v$ and less than $n$ possibilities for the choice of $t$).
\end{proof}
Before proving the dependencies to events of type $(2,t)$, and $3$,
we will prove an auxiliary lemma that concerns the events affected
by the children picked by one particular path $p\in Q^{(i)}\cap L_i$.
\begin{lemma}\label{lem:p-influence}
  Assume that no bad event has happened until the current iteration of rounding, and let $p\in Q^{(i)}\cap L_i$. Then the choice of children picked by $p$ affects
  in total at most $\alpha_{t+1}(\log n)^{3\ell}$ events of type $(2,t)$, and at most $\log n$ events of type $3$.
  
  Furthermore, for a fixed path $q$ in $Q^{(i)}$ the number of events of type $(2,t)$ that depend on the children of \emph{any} descendant $p$ of $q$ is at most $\alpha_{t+1}(\log n)^{3\ell}$ many. Similarly, the number of events of type 3 that depend on the children of \emph{any} descendant $p$ of $q$ is at most $(k\log n)^{\ell}$ many.
\end{lemma}
\begin{proof} The bad event $B_{2}(s, t,\ell')$ is determined by the
  random variable $N^{(i+1)}(s, t, \ell')$. A path $p$ originating from the source $s'$ can influence this variable only if $s'\in S(s,t,\ell')$ which is equivalent to $s\in S(s',t,\ell')$. By Lemma \ref{lem:S_B_upperbound}, there are at most $\alpha_{t+1}(\log n)^{3\ell}$ such sources $s'$. Similarly, the choices made by any descendant path of a path $q$ can influence $B_{2}(s, t,\ell')$ only if the source $s'$ from which $q$ is coming belongs to $S(s,t,\ell')$. Hence the choices made by all descendant paths of a path $q$ can only influence $|S(s,t,\ell')|\le \alpha_{t+1}(\log n)^{3\ell}$ bad events of type $(2,t)$.
  
  For a bad event of type $3$, notice that $p$ can influence $B_{3}(p')$ only if $p$ is a descendant of $p'$ in the multiset $Q^{(i)}$. We now remark that any path $p$ has at most $h\le \log n$ ancestors, which finishes the first part of the lemma, regarding type 3 events. For the second part, fix a path $q$. Then this path has at most $(k/16)^\ell$ descendant paths in $Q^{(i)}$ (at distance at most $\ell$, each one influencing at most $\log n$ events of type $3$ by the previous argument. This concludes the proof of the lemma.
  \end{proof}
  %%%%%%%%%
\begin{comment}
  $B_{3}(q)$ determined by the
  random variables $N_S^{(i+1)}(q, \ell')$ and $N_B^{(i+1)}(q, \ell')$
  either for $q = q'$ or for $q\in C_{Q^{(i)}}(q')$. Hence,
  it suffices to analyze the number of these variables affected by the children picked for $p$.
  In order for them to be affected
  there must be a common ancestor $p'$ of $p$ and $q$
  within layers $L_{i-\ell},\dotsc,L_i$ (we also allow $p' = \emptyset$ if $i\le \ell$) and paths $p''\in D_{P'}(p)$, $q''\in D_{P'}(q)$ that end in the same vertex. Note that there are at most $(k\log^2 n)^\ell$ such potential descendant paths of $p$ (\etienne{because of the granularity of $y$}) and each of them shares its endpoint with at most $2 (k \log^2 n)^{2\ell}$ other paths that have a common ancestor in the previous $2\ell$ layers (\etienne{because of Constraints \eqref{eqSparseLP:capacity}, \eqref{eqSparseLP:capacity0}, and the granularity of $y$}). \todo{Lars: Explain more Etienne: added some explanations}
  Together with the fact that there are at most $2\ell$ such variables
  for a fixed $q$ \etienne{we conclude that $p$ can influence at most}
  \begin{equation*}
     (2\ell)\cdot  (k \log^2 n)^{\ell} \cdot 2 (k \log^2 n)^{2\ell} \le (k \log n)^{6\ell} 
  \end{equation*}
  \etienne{such random variables. Finally, we remark (since no bad event happened until layer $i$ we can apply Lemma \ref{lem:iterlowcong}) that each such random variable can be copied at most $2^{11}\log^3 n$ times. Hence the random choices of $p$ can influence at most
  \begin{equation*}
      (k \log n)^{6\ell} \cdot (2^{11}\log^3 n) \le (k\log n)^{10\ell}
  \end{equation*} bad events of type $2S,2B,3$. We note that the above proof also applies to count the number of events of type $2S,2B$ that are influenced by the choice of children for a descendant of $p$.}
  For the second part of the lemma, we observe that in order for $p$ to influence
  $N_B^{(i+1)}(q, \ell')$, $q$ must be in $S_B(p',\ell')$ for an ancestor $p'$ of $p$ in the aforementioned layers. \etienne{By Lemma \ref{lem:S_B_upperbound}, we have that $|S_B(p',\ell')| \le (\log n)^{10\ell}$ which concludes the proof.}
  \end{comment}
  %%%%%%%%%%%%


\begin{comment}
Next, we estimate the cardinality $|S_B(p',\ell')|$.
  By Constraint~\eqref{eqSparseLP:demand} we have that $|V(D_{P'}(p',\ell'))| \le |D_{P'}(p',\ell')| \le (k\log^2 n)^{\ell'}$.
  Now let $v\in V(D_{P'}(p',\ell'))$. Then by Constraint~\eqref{eqSparseLP:capacity} there are at most
  $2 (4\log^2 n)^{\ell'}$ many paths in $D_{P'}(P(p'))$ that end in $v$.
  Hence in total at most
  \begin{equation*}
      2 (4\log^2 n)^{\ell'} \cdot (k\log^2 n)^{\ell'}
  \end{equation*}
  many paths from $D_{P'}(P(p'))$ end in $V(D_{P'}(p',\ell'))$.
  Each element in $S_B(p',\ell')$ accounts for at least $k^{\ell'} / (4\log^{6} n)^{\ell'}$
  many of these paths. It follows that
  $|S_B(p',\ell')| \le (\log n)^{6\ell}$.
\end{comment}



\begin{lemma}
Assuming that no bad event has happened until the current iteration of rounding,
for any $v\in V$ and integers $t,t'\ge 0$, we have 
\begin{align}
    |\Gamma_{3}(\mathcal B_1(v,t))| \leq \beta_{t+1} \cdot (\log n)^{10} \text{ and}\\
    |\Gamma_{(2,t')}(\mathcal B_1(v,t))| \leq \beta_{t+1}\cdot  \alpha_{t'+1} \cdot (\log n)^{4\ell} \ .
\end{align}
\end{lemma}
\begin{proof} We first notice that the bad event $\mathcal B_1(v,t)$ depends only on the random choices made by paths $q\in Q^{(i)}\cap L_i$ that have at least one child $q' \in C_{P'}(q)$ such that 
\begin{equation*}
    \frac{\textrm{cong}(q',v)}{y(q')} \ge (\beta_{t+1})^{-1}.
\end{equation*}
Let us count how many such paths $q$ can exist in $Q^{(i)}$. For each such path we have that 
\begin{align*}
    \frac{\textrm{cong}(q,v)}{y(q)}= \sum_{q'\in C_{P'}(q)} \frac{\textrm{cong}(q',v)}{y(q)}
    &= \sum_{q'\in C_{P'}(q)} \frac{\textrm{cong}(q',v)}{(4\log^2 n)y(q')}\\
    &\ge \frac{ (\beta_{t+1})^{-1}}{4\log^2 n} \ ,
\end{align*}
where we used here the granularity of $y$, see Constraint \eqref{eqSparseLP:granularity}. By Lemma~\ref{lem:iterlowcong},
we also have that
\begin{equation*}
    \sum_{q\in Q^{(i)}\cap L_i} \frac{\textrm{cong}(q,v)}{y(q)} = \textrm{cong}(v\mid Q^{(i)}) \le 2^{11} \log^3 n \ .
\end{equation*}
Hence, there can be at most $\beta_{t+1}\cdot  2^{13} \log^5 n$ such paths $q$. 
We use Lemma~\ref{lem:p-influence} to bound the number of bad events influenced by each $q$
and obtain 
\begin{align*}
    |\Gamma_{3}(\mathcal B_1(v,t))| \le \beta_{t+1}\cdot  2^{13} \log^5 n \cdot (\log n) &\le \beta_{t+1} \cdot (\log n)^{10} \text{ and} \\
    |\Gamma_{(2,t')}(\mathcal B_1(v,t))| \le \beta_{t+1}\cdot  2^{13} \log^5 n \cdot \alpha_{t'+1} \cdot(\log n)^{3\ell} &\le \beta_{t+1}\cdot  \alpha_{t'+1} \cdot (\log n)^{4\ell} \ . \qedhere
\end{align*}
\end{proof}
\begin{lemma}
Assume that no bad event has happened until the current iteration of rounding. For any $p\in L_{i'}$ where $i - \ell - 1 \le i' \le i - 1$ and $t\ge 0$ we have
\begin{align}
    |\Gamma_{(2,t)}(\mathcal B_3(p))|&\leq \alpha_{t+1}\cdot (\log n)^{3\ell} \text{ and} \\
    |\Gamma_{3}(\mathcal B_3(p))|&\leq (k\log n)^{\ell} \ .
\end{align}
\end{lemma}
\begin{proof} The first claim trivially follows from Lemma \ref{lem:p-influence} since $\mathcal B_3(p)$ is entirely determined by the choices of its descendants in $Q^{(i)}$.
For the second, we remark that the event $\mathcal B_3(p)$ is entirely determined by the random choices made by paths $q\in Q^{(i)}\cap L_i$ that are descendants of $p$ (at distance at most $\ell$). $p$ has at most $(k/16)^{\ell}$ such descendants and we apply Lemma \ref{lem:p-influence} to each of them to obtain
\begin{align*}
    |\Gamma_{3}(\mathcal B_3(p))|&\leq (k/16)^{\ell}\cdot  (\log n) \le (k\log n)^{\ell}\ .
\end{align*}
\end{proof}
\begin{lemma}
Assume that no bad event happened until the current iteration of rounding. For any $\ell'\le \ell$, $t\ge 0$, and $s\in S$
we have
\begin{align}
    |\Gamma_{(2,t')}(\mathcal B(s,t,\ell'))| &\leq \alpha_{t+1}\cdot \alpha_{t'+1}\cdot (\log n)^{6\ell} \text{ and} \\
    |\Gamma_{3}(\mathcal B(s,t,\ell'))| &\leq \alpha_{t+1} \cdot (k\log n)^{4\ell} \ .
\end{align}
\end{lemma}
\begin{proof} For the first claim, notice that $\mathcal B(s,t,\ell')$ is entirely determined by the random choices of descendants of sources $s'\in S(s,t,\ell')$. There are at most $\alpha_{t+1}\cdot (\log n)^{3\ell}$ many such sources by Lemma \ref{lem:S_B_upperbound}. By Lemma \ref{lem:p-influence}, the choices made by descendants of each of these sources can influence at most $\alpha_{t'+1}(\log n)^{3\ell}$ bad events of type $(2,t')$. Therefore,
\begin{equation*}
      |\Gamma_{(2,t')}(\mathcal B(s,t,\ell'))| \leq (\alpha_{t+1}\cdot (\log n)^{3\ell})\cdot (\alpha_{t'+1}\cdot (\log n)^{3\ell}) \le \alpha_{t+1}\cdot \alpha_{t'+1}\cdot (\log n)^{6\ell}\ .
\end{equation*}
For the second claim, we have that $\mathcal B(s,t,\ell')$ is determined by the random choices of at most $\alpha_{t+1}\cdot (\log n)^{3\ell} \cdot (k/16)^\ell$ paths in $Q^{(i)}$ (this is because each source has at most $(k/16)^\ell$ descendants at distance $\ell'$). By Lemma \ref{lem:p-influence}, each such path influences at most $\log n$ events of type 3. Thus we can conclude by computing
\begin{equation*}
      |\Gamma_{3}(\mathcal B(s,t,\ell'))| \leq \alpha_{t+1}\cdot (\log n)^{3\ell} \cdot (k/16)^\ell \cdot \log n \le \alpha_{t+1} \cdot (k\log n)^{4\ell}\ .
\end{equation*}

\end{proof}

\paragraph{Instantiating LLL.}
For the bad events we set
\begin{align}
    x(\mathcal B_1(v,t)) &= n^{-2} \ , \\
    x(\mathcal B_{2}(s,t,\ell')) &= (\log n)^{-38\ell} \textrm{ if $t=0$}\ , \\
     x(\mathcal B_{2}(s,t,\ell')) &= (\log n)^{-10\ell}\exp\left(-\frac{\alpha_t}{(\log n)^{10\ell}} \right) \ \textrm{ if $t\ge 1$, and} \\
    x(\mathcal B_{3}(p)) &= \exp\left(-k^{1/4} \right) \ .
\end{align}
We recall here the relevant ranges of $t$ for bad events of first and second type. For a bad event of the first type, $t$ is never more than $\log n$. For bad events of the second type, $t$ is never more than $\ell$, and $\alpha_t$ never exceeds $(k\log^2 n)^{\ell}$. We compute here a few intermediate products, that will help for the final argument.
We compute for a fixed $t'\ge 0$,
\begin{equation*}
    P_{2,t'}:=(1-x(\mathcal B_{2}(s,t,\ell')))^{\alpha_{t'+1}(\log n)^{6\ell}}\ .
\end{equation*}
If $t'=0$, then 
\begin{align*}
    P_{2,t'} &=  (1-(\log n)^{-38\ell})^{\alpha_1(\log n)^{6\ell}} \\
    &\ge \exp\left(- (\log n)^{-37\ell}\cdot \alpha_1\cdot (\log n)^{6\ell}\right)\\
    &\ge \exp\left(-(\log n)^{-10\ell}\right)\ .
\end{align*}
If $t'\ge 1$, then 
\begin{align*}
    P_{2,t'} &=  \left(1-(\log n)^{-10\ell}\exp\left(-\frac{\alpha_{t'}}{(\log n)^{10\ell}} \right)\right)^{\alpha_{t'+1}(\log n)^{6\ell}}\\
    &\ge \exp\left(-(\log n)^{-10\ell}\exp\left(-\frac{\alpha_{t'}}{(\log n)^{15\ell}}\right)\cdot  \alpha_{t'+1}(\log n)^{6\ell} \right)\\
    &\ge \exp\left(- \exp\left(-(\log n)^{-\ell}\right)\right)    \ .
\end{align*}
Here we used that $\alpha_{t'+1}\le (\alpha_{t'})^3 \le \exp\left(\frac{\alpha_{t'}}{2(\log n)^{15\ell}}\right)\cdot (\log n)^{-6\ell}$ for $t'\ge 1$ (since for $t'\ge 1$, we have that $\alpha_{t'}\ge (\log n)^{20\ell}$).


Consider now a bad event $\mathcal B_1(v, t)$. Then
\begin{align*}
    \mathbb P[\mathcal B_1(v, t)] &\le n^{-10 \cdot \beta_{t}} \\
    &\le n^{-5 \cdot \beta_{t+1}}\\
    &\le n^{-2} \cdot (1 - n^{-2})^{n^2} \cdot (\prod_{t'=0}^{\ell}P_{2,t'})^{\beta_{t+1}} \cdot (1/e)^{\beta_{t+1}}\\
    &\le n^{-2} \cdot \prod_{\mathcal B \in \Gamma(\mathcal B_1(v, t))} (1-x(\mathcal B)) \ .
\end{align*}
Next, we get
\begin{align*}
    \mathbb P[\mathcal B_2(s,0,\ell')] &\le (\log n)^{-40\ell} \\
    &\le (k\log n)^{-20\ell} \cdot (1 - n^{-2})^{n^2}
    \cdot (1 - (\log n)^{-20\ell})^{(\log n)^{20\ell}}
    \cdot (1 - (k\log n)^{-20\ell})^{(k\log n)^{20\ell}} \\
    &\le x(\mathcal B') \prod_{\mathcal B\in \Gamma(\mathcal B')} (1 - x(B)) \ .
\end{align*}
Similarly, for $\mathcal B_{2B}(p, \ell')$ we have
\begin{align*}
    \mathbb P[\mathcal B_{2B}(p, \ell')] &\le (\log n)^{-30\ell} \\
    &\le (\log n)^{-20\ell} \cdot (1 - n^{-2})^{n^2}
    \cdot (1 - (k\log n)^{-20\ell})^{(k\log n)^{20\ell}}
    \cdot (1 - (\log n)^{-20\ell})^{(\log n)^{20\ell}} \\
    &\le x(\mathcal B_{2B}(p, \ell')) \prod_{\mathcal B\in \Gamma(\mathcal B_{2B}(p, \ell'))} (1 - x(B)) \ .
\end{align*}
Hence, with positive probability none of the bad events occur
and we can compute such a solution in expected quasi-polynomial time (polynomial in $P'$).
\begin{comment}
and for the source bad event, we set $x(B(s))=1/2$.
Then we can compute for any $ p \in L_{\leq i-1}\cap L_{\ge i-\ell}$ (we assume that $k\ge 10^3 (\log \log(n))^4)$ and $n$ bigger than a sufficiently large constant),
\begin{align*}
    x(\mathcal B(p) ) &\cdot \prod_{\mathcal B \in \mathcal{N}_1(\mathcal B(p))\cup \mathcal{N}_2(\mathcal B(p))}(1-x(\mathcal B)) \\
    &\ge \exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot \left(1-n^{-2^{4}}\right)^{10n^3} \cdot \left(1-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)\right)^{(k/100)^{\ell+1}} \\
    &\ge \exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot \left(1-n^{-2^{4}}\right)^{10n^3} \cdot \frac{1}{2}\cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log (n))^2}\right) \cdot (k/100)^{\ell+1}\right)\\
    &\ge \frac{\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)}{6} \cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log(n))^2} + \ell\cdot \log (k)  \right)   \right)\\
    &\ge \frac{\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)}{6} \cdot e^{-1} \ge 2\mathbb P(\mathcal B(p)).
\end{align*}

Similarly, for any $v,t$ we obtain
\begin{align*}
    x(\mathcal B(v,t) ) &\cdot \prod_{\mathcal B \in \mathcal{N}_1(\mathcal B(v,t))\cup \mathcal{N}_2(\mathcal B(v,t))}(1-x(\mathcal B))\\
    &\ge n^{-2^{4}} \cdot \left(1-n^{-2^4}\right)^{10n^3} \cdot \left(1-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \right)^{(10^4\log^6(n))\cdot 2^{t}}\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot (10^4\log^6(n))\cdot 2^{t}\right)\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-\exp\left(-2(\log \log(n))^2 \right) \cdot (10^6\log^6(n))\cdot 2^{t}\right)\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-2^{t}\right)\\
     &\ge n^{-2^{(t+3)}}\ge 2\mathbb P(\mathcal B_{\lambda,v,t}).
\end{align*}
Finally, we recall there is only one event of the third type $\mathcal B(s)$, with $x(\mathcal B(s))=1/2$. Hence, we can conclude using known results on LLL that we can round in polynomial time the layer $i+1$ without any bad event happening.
\end{comment}


\paragraph{Finishing notes.} We proved that we can round in (expected) quasi-polynomial time from layer $0$ to layer $h$ without any bad event ever happening.
Next, observe that we get that any sampled path $p\in Q \cap L_i$ has at most 
\begin{equation*}
    \bigg|\bigcup_{i'=i+1}^{i+\ell+1} M^{(i')}(p)\bigg|\le \ell \cdot \frac{1}{2\ell} \cdot \frac{k}{16} = \frac{k}{32}
\end{equation*}
marked children. We now delete from the solution all the marked paths
obtaining a solution $Q'$. Note that the sources remain as they are never marked. This means that any sampled open path retains at least $k/32$ children.
We now define a set of paths $R\subseteq Q'$, which contains all paths with high local congestion. More precisely, let $R$ contain for every path $p\in Q'\cup \{\emptyset\}$ and $\ell'\le\ell$ all paths $q\in D_{Q'}(p, \ell')$ such that $\mathrm{cong}_p(q \mid Q') > 2 \cdot 2^{10} \ell^2$.
Each such path must add $1$ to $N_S^{(i)}(p, \ell')$ or
$N_B^{(i)}(p, \ell')$ for some $i$. Since we have no more marked paths,
each $p$ has at most
\begin{equation*}
    \sum_{i'=i}^{i+\ell} N_S^{(i')}(p, \ell') + N_B^{(i')}(p, \ell') \le \ell \cdot \frac{2}{\ell^4} \cdot \left(\frac{k}{16}\right)^{\ell'} \le \frac{1}{(8\ell)^2} \left(\frac{k}{32}\right)^{\ell'}
\end{equation*}
descendants at distance $\ell'$ in $R$.
Applying Lemma~\ref{lem:loc-to-glob} we can remove $R$ and obtain a solution
$Q'' \subseteq Q' \setminus R$,
where each open path has $k / (64\ell)$ children and every source
remains in the solution. Moreover, the solution has no more paths
with $\ell$-local congestion more than $2^{11}\ell^2$ and the global congestion is at most $2^{11} \log^3 n$.
This finishes the proof of Lemma~\ref{lem:locallygood}.

\begin{comment}
Therefore we obtain a solution such that:
\begin{enumerate}
    \item One copy of the trivial path $(s)$ belongs to $Q$ for all sources $s\in S$;
    \item Every open path has $k/200$ children;
    \item No vertex has global congestion more than $1500 \log^3(n)$;
    \item No path is marked.
\end{enumerate}
Fix a distance $\ell'\le \ell$. A path that is not marked has at most 
\begin{align*}
    \ell \cdot & \frac{100(\log \log (n))^2}{\exp(100(\log \log (n))^2)}\cdot \left(k\log^2 (n)\right)^{\ell'}\\
    &\le \left(k/200 \right)^{\ell'}\cdot \frac{10^3 (\log \log(n))^3}{\exp((\log \log (n))^2)} \cdot \left(\frac{200 \log^2 (n)}{\exp(10^2(\log \log (n)))} \right)^{\ell'} \\
    &\le \frac{\left(k/200 \right)^{\ell'}}{\log^{10}(n)}
\end{align*} bad descendant paths at distance $\ell'$. Hence only a $1/(\log^{10}(n))$ fraction of descendant paths at distance $\ell'$ have congestion more than $10^3(\log \log (n))^2$. This concludes the proof of Lemma \ref{lem:locallynearlygood}.

\subsection{From locally nearly good to locally good}

In this last step, we prove Lemma \ref{lem:locallygood}, which is fairly straightforward using Lemma \ref{lem:bot-to-top} and the previously obtained locally nearly good solution. Indeed, we check that the premises of Lemma \ref{lem:bot-to-top} are satisfied by the locally nearly good solution. Using the lemma by deleting all paths that have an $\ell$-local congestion of more than $10^3(\log \log (n))^2$, we obtain a solution that has the following properties.
\begin{enumerate}
    \item One copy of the trivial path $(s)$ belongs to $Q$ for all sources $s\in S$;
    \item Every open path has $k/(400 \ell)$ children;
    \item No vertex has global congestion more than $1500 \log^3(n)$;
    \item No path has $\ell$-local congestion more than $10^3(\log \log (n))^2$.
\end{enumerate}
Thus, we obtain a $k/O(\ell)$-valid solution with $\ell$-local congestion $O(\ell^2)$ and global congestion $O(\log^3(n))$ (recall that $\ell=\Theta (\log\log (n))$). The total running time is dominated by solving the path LP which takes time $n^{O(h)}\le n^{O(\log(n))}$. This proves Lemma \ref{lem:locallygood}.
\end{comment}

==> OverleafV1/poly_time_2layers.tex <==
\section{Modified Polymatroid algorithm for polynomial time}

We will need the following definition. For any set $B$ and matroid basis $U_M$, we define $E(B,U_M)$ to be the set of elements of $B\cup U_M$ that can be exchanged in $U_M$ for an element in $B$ (it trivially contains $B$).

\begin{description}
  \item[Input: ] Matroid $M$, polymatroid $P_{|d} \subseteq [0, d]^U$ over universe $U$ and partial solution $x, y$, and some set $B_0$ of elements to be covered.
  \item[Output: ] An augmented solution $\bar{x}, \bar{y}$ that covers $U_P\cup U_M$ and at least $\epsilon |B_0|$ elements in $B_0$ or ``failure''.
\end{description}

We will define a (non-recursive) procedure running in polynomial time to solve this problem. At iteration $\ell+1$ we proceed as follows.

We build an addable set $A^{(\ell +1)}$: Assume we have already built $A^{(\leq \ell)}=\bigcup_{1\leq i\leq \ell} A^{(i)}$ and the corresponding blocking set $B^{(\leq \ell)}=\bigcup_{0\leq i\leq \ell} B^{(i)}$. Additionally we will maintain a set $I^{(\ell+1)}\subseteq A^{(\ell +1)}$ of immediately addable elements. To build $A^{(\ell +1)}$, $B^{(\ell +1)}$, and $I^{(\ell +1)}$ define the following procedure:
\begin{enumerate}
    \item $A^{(\ell +1)},B^{(\ell +1)},I^{(\ell +1)}\leftarrow \emptyset$
    \item Set $E'\leftarrow \emptyset$ ($E'$ will be the current set of elements that we can exchange in $B^{(\leq \ell)}$ for some element in $A^{(\ell + 1)}$). For each $i'\in A^{(\ell +1)}$, we will denote by $m(i')$ the element in $E'$ that was selected to be swapped with $i'$.
    \item while ($A^{(\ell + 1)}<\epsilon |B^{(\leq \ell)}|$) select some $i\in E(B^{(\leq \ell)}\setminus E',U_M)$ that can be swapped with $i'\in B^{(\leq \ell)}$ such that $f_{\mid d}(i\mid A^{(\leq \ell)}\cup B^{(\leq \ell)}\cup A^{(\ell + 1)} )\geq d$ and set $A^{(\ell + 1)}\leftarrow A^{(\ell + 1)}\cup \{i\}$, $B^{(\ell + 1)}\leftarrow B^{(\ell + 1)}\cup \mathcal C(i)$, $E'\leftarrow E'\cup \{i'\}$. If $\mathcal C(i)=\emptyset$, set $I^{(\ell+1)}\leftarrow I^{(\ell+1)}\cup \{i\}$. If no such $i$ can be found return failure. Additionnally, set $m(i)=i'$.
\end{enumerate}

(TODO: description of collapse phase)

We now describe the collapse phase that happens.

\begin{lemma}
  For any $\ell\geq 0$, and any $S\subseteq \in A^{(\ell)}$ then we have that $U_M\setminus S \cup m(S)$ is in the matroid. 
\end{lemma}
\begin{proof}
  Order the elements in $S$ in an arbitrary order $s_1,s_2,\ldots$ and we swap each $s_i$ in this order with $m(s_i)$. We can prove by an easy induction that during this process the set obtained is always a basis of the matroid. This is clear before swapping anything. Assume that we managed to swap $s_1,s_2,\ldots , s_k$ so that $U_M\setminus \{s_1,s_2,\ldots ,s_k \}\cup \{m(s_1),m(s_2),\ldots, m(s_k)\}$ is in the matroid. Recall also that by definition $m(s_{k+1})$ was selected to be swapped in $U_M$ with $s_k$. 
\end{proof}

\begin{lemma}
  For any $\ell\geq 1$, we have that $B^{(\ell)}\geq \frac{\epsilon}{1-\epsilon}|A^{(\ell)}\setminus I^{(\ell)}|$.
\end{lemma}
\begin{proof}
  Recall that we add an element to $A^{(\ell)}$ if and only if 
  
  \begin{equation*}
      f_{\mid d} (i\mid A^{(<i)}\cup B^{(\leq \ell)})\geq d. 
  \end{equation*}
  
  For ease of notation, let us consider the submodular function 
  \begin{equation*}
      g(S) = f_{\mid d} (S\mid A^{(\leq \ell)}\cup B^{(\leq \ell)}). 
  \end{equation*}
  
  After creating the set $A^{(\ell+1)}=\{i_1,\ldots ,i_k\}$, we have that
  \begin{equation*}
      g(A^{(\ell+1)})= \sum_{m = 1}^k g(i_m \mid \{i_1,\ldots ,i_{m-1} \})\geq |A^{(\ell + 1)}|d
  \end{equation*}
  
  Moreover, for each element $i$ added in $A^{(\ell+1)}$, denote by $C_i$ an arbitrary set in the blocking family $\mathcal C(i)$. 
  
  Recall that we have by submodularity of $f$ 
  
  \begin{equation*}
      g(C_i)\leq f(C_i)\leq d(1-\epsilon)|C_i|
  \end{equation*}
  
  Then by subadditivity of $g$ we obtain that
  \begin{equation*}
      g(\cup_{i\in A^{(\ell+1)}} C_i \leq g(C_i) \leq d(1-\epsilon)|A^{(\ell+1)}|+d(1-\epsilon)|B^{(ell+1)}|
  \end{equation*}
  
  Since $g$ is increasing, we also have that
  \begin{equation*}
      g(\cup_{i\in A^{(\ell+1)}} C_i\geq g(A^{(\ell+1)})\geq |A^{(\ell + 1)}|d
  \end{equation*}
  
  Putting together we obtain that 
  
  \begin{equation*}
      |A^{(\ell + 1)}|d \leq d(1-\epsilon)|A^{(\ell+1)}|+d(1-\epsilon)|B^{(ell+1)}|
  \end{equation*}
  
  which implies that $|B^{(\ell+1)}|\geq \frac{\epsilon}{1-\epsilon}|A^{(\ell+1)}|$.
\end{proof}

\begin{lemma}
  The algorithm never fails.
\end{lemma}
\begin{proof}
  Assume the algorithm fails while trying to build $A^{(\ell +1)}$, i.e. it can only build an addable set $A^{(\ell +1)}$ of size less than $\epsilon |B^{(\leq \ell)}|$. Consider this set along with the set $E'$ of elements that can be exchanged in $B^{(\leq \ell)}$ for $A^{(\ell +1)}$. Consider $E=E(B^{(\leq \ell)}\setminus E',U_M)$. Then for all $i$ in $E$ we have that $f(i\mid A^{(\leq \ell)}\cup B^{(\leq \ell)}\cup A^{(\ell + 1)})< d$. Now let $x^*,y^*$ be feasible solution to the LP with objective $\alpha\cdot d$. Then we can write that
  \begin{align*}
      d(\alpha-1)\cdot y^*(E)&<\sum_{i\in U} y_i^* \left(\alpha\cdot d -f\left(i\mid A^{(\leq \ell)}\cup B^{(\leq \ell)}\cup A^{(\ell + 1)}\right)\right)\\
      &\leq f\left( A^{(\leq \ell)}\cup B^{(\leq \ell)}\cup A^{(\ell + 1)}\right)\\
      &\leq f\left( A^{(\leq \ell)}\cup B^{(\leq \ell)}\right) + f\left(A^{(\ell + 1)}\right)
  \end{align*}
      
  where the last line comes from subadditivity of $f$. Since we have objective $\alpha d$ we can assume that $f(S)\leq \alpha d |S|$ for any set $S$. This implies that 
  \begin{equation*}
      f\left(A^{(\ell + 1)}\right)\leq (\alpha d)\cdot |A^{(\ell + 1)}|
  \end{equation*}
  
  Our next step is to bound the value of $f\left( A^{(\leq \ell)}\cup B^{(\leq \ell)}\right)$. To this end, we first recall that we assume that the algorithm is stuck which implies that $|I^{(\ell)}|<\epsilon |A^{(\ell)}|$ for all $\ell$. By subadditivity of $f$, this implies the following inequality
  \begin{align*}
      f\left( A^{(\leq \ell)}\cup B^{(\leq \ell)}\right) &\leq f\left(A^{(\leq \ell)}\cup B^{(\leq \ell)}\setminus I^{(\leq \ell)}\right) + f\left( I^{(\leq \ell)}\right) \\
      &\leq f\left(A^{(\leq \ell)}\cup B^{(\leq \ell)}\setminus I^{(\leq \ell)}\right) + \epsilon \cdot (\alpha d)\cdot  |A^{(\leq \ell)}|
  \end{align*}
  
  The last step is to bound the value of $f\left(A^{(\leq \ell)}\cup B^{(\leq \ell)}\setminus I^{(\leq \ell)}\right)$. Recall that the set $A^{( \ell)}\cup B^{( \ell)}\setminus I^{( \ell)}$ is built iteratively. At each step, a new element $i$ is added to $A^{(\ell)}$ if we have that 
  \begin{equation*}
      f_{|d}\left(i|A^{<i}\cup B^{(\ell-1)}\right)\geq d
  \end{equation*}
  
  where $A^{<i}$ denotes the set of all addable elements that were added before $i$. Then for each such added element $i$, either it is immediately addable and then $i\in I^{(\ell)}$ or a family $\mathcal C(i)$ of blocking subsets is identified and added to $B^{(\ell)}$. Each set $C\in \mathcal C(i)$ is an inclusion-wise minimal set that satisfies:
  \begin{equation*}
      f_{|d}\left(C|A^{<i}\cup B^{(\leq \ell-1)}\right)<d(1-\epsilon)|C|
  \end{equation*}
  
  By Lemma~\ref{lem:polymatroid-restriction2} we can substitute $f_{|d}$ for $f$ here.
  We enumerate all such sets $C\in \mathcal C(i)$ arbitrarily by $C_1,\dotsc, C_k$ and prove inductively that
  
  \begin{equation*}
      f\left(C_{\leq h}|A^{<i}\cup B^{(\leq \ell-1)} \right) \leq d(1-\epsilon)|C_{\leq h}|
  \end{equation*}
  for all $h\leq k$. The base case holds by definition of $C_1$. Now let h>1. If $C_h\subseteq C_{<h}$ then nothing needs to be shown. Otherwise we have that 
  
  \begin{equation*}
      d(1-\epsilon)|C_h\cap C_{<h}|\leq f\left(C_h\cap C_{<h}\right)
  \end{equation*} by minimality of $C_h$. Hence, by submodularity of $f$,
  
  \begin{equation*}
      f(C_{\leq h})\leq f(C_h)+f(C_{<h})-f(C_h\cap C_{<h})<d(1-\epsilon)\cdot \left(|C_h|+|C_{<h}|-|C_h\cap C_{<h}| \right) = d(1-\epsilon)|C_{\leq h}|
  \end{equation*}
  
  
 This proves that 
 \begin{equation*}
     f\left(\mathcal C(i)|A^{<i}\cup B^{(\leq \ell)} \right)\leq d(1-\epsilon)|\mathcal C(i)|
 \end{equation*}
  
  Finally we claim that $U_M\cap E$ is a maximal independent subset of $E$. To see this, assume this was not the case then there would exist an inclusion-wise bigger subset of $E$ that is independent. Denote this subset by $U'_M$. By the exchange property there would exist $i\in U'_M\setminus U_M\subseteq B$ and $i' \in U_M\setminus U'_M\subseteq U\setminus E$ such that $U_M - i'+i\in M$. Hence $E$ should contain $i'$ which is a contradiction.
  
  
  Hence we have 
  \begin{equation}
      x(E)\leq |U_M\cap E| \leq |E\setminus B|
  \end{equation}
\end{proof}

==> OverleafV1/polymatroid.tex <==

\section{Polymatroids}
Let $M$ be a matroid and $P$ a polymatroid over ground set $U$ of cardinality $n$. The matroid is defined by a rank function $r$, that
is, $M$ corresponds to the integer points in
\begin{equation*}
    \{ x\in\mathbb [0, 1]^U \mid x(S) \le r(S) \ \forall S\subseteq U\} .
\end{equation*}
The polymatroid $P$ is defined by a monotone, submodular function $f$,
that is, it corresponds to the integer points in
\begin{equation*}
    \{ x\in\mathbb R^U_{\ge 0} \mid x(S) \le f(S) \ \forall S\subseteq U\} .
\end{equation*}
Our goal is to find some basis $x \in M$ such that
$d \cdot x \in P$. Here $d$ is to be maximized.
This problem generalizes the two level case.

Notice that the intersection of a polymatroid $P$ with a zero anchored square
$[0, k]^U$ for some $k\in\mathbb N$ is again a polymatroid, which we denote by $P_{|k}$.
If $f$ is the submodular function corresponding to $P$, we denote by $f_{|k}$
the submodular function corresponding to $P_{|k}$.
The value $f_{|k}(S)$ is the maximum $\lVert y \rVert_1$ over all
$y\in [0, k]^S$ with $y\in P$.
We briefly explain two properties of polymatroid intersected with squares that we will use
later on.
\begin{lemma}\label{lem:polymatroid-restriction}
  Let $P$ be a polymatroid and $k \in \mathbb N$. Let $S\subseteq U$ and $i\in U\setminus S$.
  If $f_{|k}(i \mid S) < k$ then also $f(i \mid S) < k$.
\end{lemma}
\begin{proof}
  Let $x \in [0, k]^S$ with $x \in P_{|k}$ and $\lVert x \rVert_1 = f_{|k}(S)$.
  Now augment it to some $x'\in [0, k]^{S + i}$ with $x'\ge x$, $x' \in P_{|k}$ and
  $\lVert x \rVert_1 = f_{|k}(S + i)$. Since $f_{|k}(i \mid S) < k$ we have that
  $x'_i < k$.
  
  We augment $x'$ it to some $x'' \ge x'$ with $x''\in \mathbb R^{S+i}_{\ge 0}$, $x''\in P$,
  and $\lVert x'' \rVert_1 = f(S+i)$. If $x''_i \ge k$ then this would mean
  that increasing $x_i$ to $k$ would remain in $P_{|k}$. A contradiction, since
  $\lVert x \rVert_1$ is already $f(S + i)$.
  Moreover, $f(S)$ is at least $\lVert x'' \rVert_1 - x''_i$. Thus,
  \begin{equation*}
      f(i \mid S) = f(S + i) - f(S) \le \lVert x'' \rVert_1 - (\lVert x'' \rVert_1 - x''_i) < k .\qedhere
  \end{equation*}
\end{proof}
\begin{lemma}\label{lem:polymatroid-restriction2}
  Let $P$ be a polymatroid and $k' \le k$.
  Let $x\in \{0,1\}^U$ with $k' \cdot x \in P$. Then $k' \cdot x \in P_{|k}$ as well.
  In particular, if $C \subseteq U$ is an inclusion-wise minimal set with $k' \cdot |C| > f_{|k}(C)$,
  then $C$ is also an inclusion-wise minimal set with $k' \cdot |C| > f(C)$.
\end{lemma}
\begin{proof}
  The first part is by definition.
  For the second part notice that for all $C' \subsetneq C$ we have
  \begin{equation*}
      f(C') \ge f_{|k}(C') \ge k' \cdot |C'| .
  \end{equation*}
  Hence, if $k' \cdot |C| \le f(C)$, then $k' \cdot x \in P$, where $x$ is the indicator vector of $C$. Thus, by the first part of the lemma $k' \cdot x \in P_{|k}$, which is a contradiction.
  
\end{proof}

\subsection{Linear program}
Fix some $d$.
The natural linear program for this problem is as follows.
\begin{align*}
    \sum_{i\in U} x_i &= r(U) \\
    x(S) &\le r(S) &\forall S\subseteq U \\
    d \cdot x(S) &\le f(S) &\forall S\subseteq U \\
    x &\in [0, 1]^U &
\end{align*}
This relaxation has an unbounded integrality gap.
We will strengthen it by replacing the second constraint type with
\begin{equation*}
    \sum_{i\in U} x_i \cdot (d - f(i \mid S))_+ \le f(S) \quad \forall S\subseteq U.
\end{equation*}
Here $(*)_+ = \max\{0, *\}$. 
Notice that the sum is over the whole universe, not just $S$.
We can avoid the $(*)_+$ by requiring without loss of generality
that $P \subseteq [0, d]^U$ (replacing $P$ with $P_{|d}$).
The constraint is valid for all integral solutions: Let $x$ be some integer solution
and let $S'$ be the set of all $i\in U\setminus S$ with $x_i = 1$ and $f(i \mid S) \le d$. Then
\begin{equation*}
    \sum_{i\in U} x_i \cdot (d - f(i \mid S))_+
    = d \cdot y(S) + \sum_{i\in S' \setminus S} (d - f(i \mid S))
    \le f(S \cup S') - \sum_{i\in S'\setminus S} f(i \mid S) \le f(S) .
\end{equation*}
We will prove algorithmically that if the linear program above is feasible for $\alpha \cdot d$,
where $\alpha = 3$, then there exists an integral solution for $d$.

It is unclear how to solve the LP. While the constraints of the form
$x(S) \le r(S)$ are standard matroid constraints for which submodular minimization
yields a separation algorithm, the new type of constraints are more complicated.
However, We will show how to solve it by losing a constant factor.
\begin{theorem}
    Suppose there is an integer feasible for some $d^*$.
    Then we can find a feasible
    solution of the LP for $d \ge (1 - 1/e) d^*$.
\end{theorem}
\begin{proof}
  Notice that an integer solution satisfies
  $d \sum_{i\in U} x_i \le f(x)$.
  Hence, a valid convex constraint (for the integer hull) is that
  \begin{equation}\label{eq:alt-constraint}
    d \sum_{i\in U} x_i \le f^+(x).
  \end{equation}
  Here, $f^+$ is the concave closure of $f$. This is NP-hard to evaluate,
  so it is hopeless to (exactly) check this constraint.
  We will give an approximate separation algorithm for it. Namely,
  if $d^* \sum_{i\in U} x_i > (1 - 1/e)^{-1} f^+(x)$ then we find a separating
  hyperplane that cuts off $x$ from all points that satisfy~(\ref{eq:alt-constraint}).
  If the converse is true, we show that $x$ satisfies all inequalities
  with $d = (1 - 1/e) d^*$.
  
  We now take a closer look at $f^+(x)$. It is defined as the optimum
  of the following linear program.
  \begin{align*}
      \max \sum_{S\subseteq U} &f(S) y_S \\
      \sum_{S\subseteq U} \mathbb{1}_S y_S &= x \\
      \sum_{S\subseteq U} y_S &= 1 \\
      y_S &\ge 0
  \end{align*}
  Next, we construct its dual:
  \begin{align*}
      \min \lambda + \sum_{i\in U} &x_i \mu_i \\
      f(S) - \sum_{i\in S} \mu_i &\le \lambda \quad \forall S\subseteq U \\
      \lambda, \mu_i &\in \mathbb R
  \end{align*}
  Suppose that some constraint is violated a lot, that is,
  $(1 - 1/e) f(S^*) - \sum_{i\in S^*}\mu_i > \lambda$ for some $S^* \subseteq U$.
  Let us assume we know the value $\gamma = \sum_{i\in S^*} \mu_i$ by some smart
  guessing. Then we can approximate $S^*$ by maximizing $f(S)$ subject to
  the knapsack constraint $\sum_{i\in S} \mu_i \le \gamma$.
  The optimum is clearly at least $f(S^*)$. Thus
  a $(1 - 1/e)$-approximation algorithm for the problem gives us some $S$ with
  \begin{equation*}
      f(S) - \sum_{i\in S} \mu_i \ge (1 - 1/e) f(S^*) - \sum_{i\in S^*} \mu_i > \lambda .
  \end{equation*}
  This way we can approximately solve the dual which gives us a
  $(1 - 1/e)$-approximate solution to the primal.
  More precisely, it gives us a subgradient $g: [0, 1]^U \rightarrow \mathbb R$
  with $g(x) \ge (1 - 1/e) f^+(x)$ and $g(x') \le f^+(x')$ for all $x'$.
  \begin{equation*}
      d\sum_{i\in U} x_i > (1 - 1/e)^{-1} f^+(x)
  \end{equation*}
\end{proof}
\subsection{Algorithm}
We consider partial solutions $x, y \in \{0, 1\}^U$ where
$x\in M$ and $d \cdot y \in P$.
However, some elements $i\in U$ might have  $x_i = y_i = 0$.
If $x, y$ is clear from the context let $U_P$ denote those elements $i$ that have $y_i = 1$
and $U_M$ those with $x_i = 1$.
For some $S\subseteq U$ we write $d \cdot S\in P$ if $z\in P$ for the vector $z$ that
has entries $z_i = d$ if $i\in S$ and $z_i = 0$ otherwise.

We now define a recursive algorithms with the following interface.
\begin{description}
  \item[Input: ] Matroid $M$, polymatroid $P_{|d} \subseteq [0, d]^U$ over universe $U$ and partial solution $x, y$ that covers all but some $B_0 = U \setminus (U_M \cup U_P)$.
  \item[Output: ] An augmented solution $\bar{x}, \bar{y}$ that covers $U_P\cup U_M$ and at least $\epsilon^2 |B_0|$ elements in $B_0$ or ``failure''.
\end{description}
Assume without loss of generality that $U_M$ is a basis of $M$.
We construct greedily two sets set $A \subseteq B_0 \cup U_M$
and $\bar{A} \subseteq B_0$.
Intuitively, we want that the elements in $A$ are either in $B_0$
or they can be
exchanged (in the matroid $M$) for elements in $B_0$.
We iterate over all $i\in B_0 \cup U_M$.
Let $A^{(<i)}$ and $\bar{A}^{(<i)}$ denote the state of
$A$ and $\bar A$ before we consider $i$.
We add $i$ to $A$ (and $\bar i$ to $\bar A$) if
\begin{equation*}
    U_M \setminus (A^{(<i)} + i) \cup (\bar A^{(<i)} + \bar i) \in M
\end{equation*}
for some $\bar i \in B_0$ and
\begin{equation*}
    f_{|d}(i \mid A^{(<i)}) \ge d .
\end{equation*}
If the elements $i\in A$ cannot be added to $U_P$,for
this is because some elements in $U_P$
``block'' $i$, that is, we cannot add $i$ to $U_P$ 
without removing other elements first.
We will now identify those blockers.
Let $\mathcal C$ denote all $C \subseteq A \cup U_P$ such that
$|C \cap A| = 1$ and
$C$ is an inclusion-wise minimal set with
\begin{equation*}
    d \cdot |C| > f_{|d}(C) .
\end{equation*}
We set $B = \bigcup \mathcal C \setminus A$.
\bigskip

\lars{TODO: The rest needs to be adjusted to the changes above.}

\paragraph*{1)} If $|A| < \epsilon |B_0|$ we return ``failure''.

\paragraph*{2)} If $i\notin \mathcal C$ for $\epsilon^2 |B_0|$ many $i\in A$ then
we can add each $i$ to $U_P$ (Lemma~\ref{lem:add-A}),
that is, $d \cdot (U_P + i) \in P_{|d}$,
We do so, swap each $i$ for some $i'\in B_0$ in the matroid and terminate
successfully.

\paragraph*{3)} In the other case, we will use the algorithm recursively
to remove some elements in $B$ from $U_P$. To this end define
for all $S\subseteq U$:
\begin{equation*}
    f'_{|d}(S) = f_{|d}(S \mid A \cup B),
    \qquad
    r'(S) = r(S \mid B_0 \cup A) .
\end{equation*}
Let $M'$ and $P'$ be the corresponding matroid and polymatroid (they are contractions of $M$ and $P$).
Let $x'$ be equal to $x$ and let $y'$ be defined with
\begin{equation*}
    y'_i = \begin{cases}
      y_i &\text{ if } i\in U \setminus B, \\
      0 &\text{ if } i\in B .
    \end{cases}
\end{equation*}
The vectors $x', y'$ form a feasible partial solution for the contracted problem (Lemma~\ref{lem:safe-contracted-matroid} and~\ref{lem:safe-contracted-polymatroid}).
We now call the algorithm recursively with $U', f', r', x', y'$, and $B\setminus E$.
If it fails, we return ``failure'' as well.
If it succeeds, we get a new solution $\bar{x}, \bar{y}$ on the
contracted problem and $\bar{x}_{i} = 1$ for at least one $i\in B$
($\bar{y}_{i} = 1$ cannot happen because $f'(i) = 0$).
We augment $x, y$ as follows:
\begin{equation*}
    y_i \gets \begin{cases}
      \bar{y}_i &\text{ if } i\in U' \setminus B, \\
      0 &\text{ if } i\in B\setminus E \text{ and } \bar{x}_i = 1, \\
      1 &\text{ if } i\in B\setminus E \text{ and } \bar{x}_i = 0, \\
      y_i &\text{ otherwise,}
    \end{cases}
    \qquad
    x_i \gets \begin{cases}
      \bar{x}_i &\text{ if } i\in U', \\
      x_i &\text{ otherwise.}
    \end{cases}
\end{equation*}
We therefore removed at least one element in $B$ from $U_P$.
The recursive call on the contracted instance is safe with respect
to the feasibility of $x$ (Lemma~\ref{lem:safe-contracted-matroid}),
the feasibility of $y$ (Lemma~\ref{lem:safe-contracted-polymatroid}),
the invariant that every element in $A$ can be exchanged for
an element in $B_0$ (Lemma~\ref{lem:safe-contracted-matroid}) and it
cannot result in a set $C$ with the definition as above
that is not contained in $\mathcal C$ 
(Lemma~\ref{lem:safe-contracted-polymatroid}).
On the other hand, any set that
contains an element in $B$ that was removed from $U_P$ now
disappears from $\mathcal C$. We redefine $B$ with using the
smaller set $\mathcal C$. Then we remove all elements from $A$
that no longer appear in any set in $\mathcal C$.
Then we repeat the procedure at the case distinction between 1), 2) and 3).

\subsection{Analysis}
\begin{lemma}\label{lem:inc-A}
\lars{Does not hold.}
  For each $i\in E \setminus A$ it holds that $f(i \mid A \cup B) < d$.
\end{lemma}
\begin{proof}
  We notice that $f_{|d}(i\mid A_\prelim) < d$ for all $i\in E\setminus A_\prelim$.
  For each $i\in A_\prelim \setminus A$ there is some $C\subseteq B \cup \{i\}$
  with $f(C) < d / (1 + \epsilon) \cdot |C|$. Hence,
  \begin{equation*}
      f(i \mid A\cup B) \le f(i \mid C - i) = f(C) - f(C - i) < \frac{d}{1 + \epsilon} |C| - \frac{d}{1 + \epsilon} (|C| - 1) = \frac{d}{1 + \epsilon} .
  \end{equation*}
\end{proof}
\begin{lemma}\label{lem:add-A}
  For each $i\in A$ either
  $i\in \bigcup \mathcal C$ or
  \begin{equation*}
      \frac{d}{1 + \epsilon} (U_P + i) \in P_{|d} .
  \end{equation*}
\end{lemma}
\begin{proof}
  Recall that
  \begin{equation*}
      f_{|d}(i \mid B^{(<i)}) \ge f_{|d}(i \mid A^{(<i)}\cup B^{(<i)}) \ge d .
  \end{equation*}
  Assume now that $\bigcup \mathcal C(i) \setminus \{i\} \subseteq B^{(<i)}$. Together this implies that $\mathcal C(i) = \emptyset$:
  Let $C\in \mathcal C(i)$. then
  \begin{equation*}
      d \cdot |C\setminus \{i\}| > f_{|d}(C) - d
      \ge f_{|d}(C\setminus \{i\}) .
  \end{equation*}
  A contradiction, since $C\setminus\{i\} \subseteq U_P$.
  This implies that there is no set $S \subseteq U_P\cup \{i\}$ with
  \begin{equation*}
      d \cdot |S| > f_{|d}(S)
  \end{equation*}
  Hence, $d \cdot (U_P + i) \in P$.
\end{proof}

\begin{lemma}\label{lem:safe-contracted-matroid}
  Let $M'$ denote the matroid over $U' = U\setminus E$
  derived by contraction as in the algorithm. Then
  \begin{enumerate}
      \item $U_M \setminus E \in M'$,
      \item For each $S \subseteq E$ with $S\in M$ and
      each $T \in M'$ we have $S\cup T\in M$. 
  \end{enumerate}
\end{lemma}
\begin{proof}
  Consider the first claim.
  Note that $E\cap U_M$ is a maximal size independent subset of $E$.
  If not, there would be some $i\in E\setminus U_M$ and
  $i'\in U_M\setminus E$ such that $U_M + i - i' \in M$.
  Let $S\subseteq U_M \setminus E$. Then we have
  \begin{equation*}
      r'(S) = r(S \cup E) - r(E) \ge |S \cup (E \cap U_M)| - |E \cap U_M| = |S| .
  \end{equation*}
  Now consider the second claim.
  Let $S \subseteq B_0\cup A$ with $S\in M$ and
  $T \in M'$.
  Then for each $T' \subseteq U$
  \begin{equation*}
      |T \cap T'| \le r'(T') = r(T' \cup B_0 \cup A) - r(B_0 \cup A)
  \end{equation*}
  Furthermore, for each $S'\subseteq B_0\cup A$
  \begin{equation*}
      |S \cap S'| \le r(S') .
  \end{equation*}
  Thus,
  \begin{equation*}
      |T\cap T' \cup S\cap S'| \le r(T' \mid B_0\cup A) + r(S') \le r(T' \mid S') + r(S') = r(T'\cup S') .
  \end{equation*}
  Hence, $S\cup T\in M$.
\end{proof}
\begin{lemma}\label{lem:safe-contracted-polymatroid}
  Let $P'_{|d}$ denote the polymatroid over $U' = U\setminus E$
  derived by contraction as in the algorithm. Then
  \begin{enumerate}
      \item It holds that $d \cdot (U_P\setminus (E \cup B)) \in P'_{|d}$.
      \item Let $S\subseteq A\cup B$ and $T \subseteq U\setminus (E \cup B)$ with
          $d \cdot S \in P_{|d}$ and $d \cdot T \in P'_{|d}$.
      Then
      \begin{equation*}
          d \cdot (S \cup T) \in P_{|d} .
      \end{equation*}
  \end{enumerate}
\end{lemma}
\begin{proof}
  For the first claim let $S \subseteq U_P \setminus (E \cup B)$. 
  Then
  \begin{equation*}
      f'_{|d}(S) = f_{|d}(S \cup A \cup B) - f_{|d}(A \cup B)
      \ge d \cdot |S \cup B| - d \cdot |B| = d \cdot |S| .
  \end{equation*}
  Now consider the second claim.
  Let $S'\subseteq S$ and $T'\subseteq T$.
  Then
  \begin{multline*}
      d \cdot |S' \cup T'|
      \le f_{|d}(S') + f'_{|d}(T')
      = f_{|d}(S') + f_{|d}(T' \mid A \cup B) \\
      \le f_{|d}(S') + f_{|d}(T' \mid S')
      = f_{|d}(S'\cup T'). \qedhere
  \end{multline*}
\end{proof}

\begin{lemma}
  If the LP is feasible for $d\cdot \alpha$ and $\alpha \ge 3$, then the algorithm always succeeds.
\end{lemma}
\begin{proof}
  Suppose toward contradiction the algorithm fails, that is,
  at some recursive call it cannot add any elements to $A$.
  Let $A_k$ and $B_k$ denote the current sets at recursion depth $k$.
  Throughout the proof we will let $A$ denote the union of all sets $A_k$
  the same for $B$. Let $E$ denote all elements $i\in U_M$
  such that there exists some $i'\in B$ with $U_P - i + i' \in M$.
  Since the algorithm cannot add an element to $A$,
  this means for all $i\in E$ we have
  $f_{|d}(i \mid A \cup B) < d$, which by Lemma~\ref{lem:polymatroid-restriction}
  implies $f(i \mid A \cup B) < d$.
  Let $x^*, y^*$ be a feasible solution to the LP with $\alpha \cdot d$.
  We start by giving a bound on $y^*(E)$, namely
  \begin{equation}\label{eq:bound-E}
      d (\alpha - 1) \cdot y^*(E) < \sum_{i\in U} y^*_i \cdot (\alpha \cdot d - f(i \mid A \cup B))_+ \le f(A \cup B) .
  \end{equation}
  Intuitively, this means that the number of elements in $E$ that the LP solution can
  cover using the polymatroid $P$ is not much larger than what can be covered in $A\cup B$.
  Our next step is to bound $f(A \cup B)$. More precisely, we will show that $f(A\cup B) < d \cdot |A\cup B|$. This requires some tedious calculation.
  To this end, we first consider each recursion depth independently
  and show for all $k$
  \begin{equation*}
      f(A_k \cup B_k \mid A_{<k} \cup B_{<k}) \le d \cdot |A_{k} \cup B_{k}| .
  \end{equation*}
  Notice that $A_k\cup B_k$ is the union of sets $C$ which are inclusion-wise minimal
  with
  \begin{equation*}
      f_{|d}(C \mid A_{<k} \cup B_{<k}) < d \cdot |C| .
  \end{equation*}
  By Lemma~\ref{lem:polymatroid-restriction2} we can substitute $f_{|d}$ for $f$ here.
  We enumerate all such sets $C$ arbitrarily by $C_1,\dotsc, C_\ell$ and prove inductively that
  \begin{equation*}
      f(C_{\le h} \mid A_{<k} \cup B_{<k}) < d \cdot |C_{\le h}|
  \end{equation*}
  for all $h\le \ell$. The base case holds because of the definition of $C_1$.
  Now let $h>1$. If $C_h \subseteq C_{<h}$ then nothing needs to be shown. Otherwise, we have that
  \begin{equation*}
      d \cdot |C_h \cap C_{<h}| \le f(C_h \cap C_{<h}) .
  \end{equation*}
  Hence,
  \begin{equation*}
      f(C_{\le h}) \le f(C_h) + f(C_{<h}) - f(C_h \cap C_{<h}) < d \cdot |C_h| + d \cdot |C_{<h}| - d \cdot |C_h \cap C_{<h}| = d \cdot |C_{\le h}| .
  \end{equation*}
  This proves that $f(A_k \cup B_k \mid A_{<k} \cup B_{<k}) < d \cdot |A_k \cup B_k|$.
  We will now combine the inequalities of each recursion depth by showing inductively
  that for all $k$
  \begin{equation*}
      f(A_{\le k} \cup B_{\le k}) < d \cdot |A_{\le k} \cup B_{\le k}| .
  \end{equation*}
  The base case holds because of our previous bound. Let $k>1$. Then
  \begin{equation*}
      f(A_{\le k} \cup B_{\le k}) = f(A_{<k} \cup B_{<k}) + f(A_k \cup B_k \mid A_{<k} \cup B_{<k}) < d \cdot |A_{\le k} \cup B_{\le k}| .
  \end{equation*}
  We conclude that $f(A\cup B) < d \cdot |A\cup B|$. Together with (\ref{eq:bound-E})
  and Lemma~\ref{lem:add-A} this implies
  \begin{equation*}
       y^*(E) < \frac{1}{\alpha - 1}  |A\cup B| \le \frac{2}{\alpha - 1} |B| \le |B| .
  \end{equation*}
  On the other hand, since $U_M \cap E$ is a maximal independent subset of $E$, we have
  \begin{equation*}
      x^*(E) \le r(E) = |E \cap U_M| = |E \setminus B| .
  \end{equation*}
  A contradiction, since $x^*(E) + y^*(E) = |E|$.
\end{proof}
\begin{lemma}
  The algorithm terminates.
\end{lemma}
\begin{proof}
  The recursion depth is bounded by $|U|$, since each recursion reduces the size of the universe.
  On the other hand, the algorithm can make only $|U|$ recursive calls:
  After a recursion returns, $|B|$ always decreases.
  Hence, the algorithm must terminate within a time that is a polynomial times $|U|^{|U|}$.
\end{proof}



\section{Version with co matroid in polynomial time}
LP:
\begin{align*}
    \sum_{i\in U}x_i&=r(U)\\
    x(S) &\le r(S) &\forall S\subseteq U \\
    \sum_{i\in U} x_i \cdot (d - f(i \mid S))_+ &\le f(S) &\forall S\subseteq U \\
    x &\in [0, 1]^U &
\end{align*}
\begin{description}
  \item[Input: ] $\epsilon > 0$, matroid $M$, polymatroid $P_{|d} \subseteq [0, d]^U$ over universe $U$ and partial solution $x$ such that $x\in M$ (but not a basis) and $\frac{d}{1+\epsilon}\cdot x\in P$. We will denote by $\mathcal I$ the independent set of the matroid corresponding to $x$. An additional subset $i_0$ such that $x+i_0\in M$.
  \item[Output: ] An augmented solution $\bar{x}\in M$ such that $\frac{d}{1+\epsilon}\cdot \bar{x}\in P$ and $|\bar{x}|\geq |x|+1$.
\end{description}
\subsection{Description of the algorithm}
The main algorithm is made of two principal subroutines: {\sc CollapseLayer} and {\sc BuildLayer}. 
\newpage 

\begin{algorithm}
\caption{\sc BuildLayer}\label{BuildLayer}
\begin{algorithmic}[1]
\Procedure {BuildLayer}{$A$, $B$, $\ell$, $\mathcal I$, $d$, $\epsilon$}
\State Select a set $A^{\ell+1}\subseteq (U\setminus \mathcal I)\cup B^{\leq \ell}$ such that $|A^{\ell +1}|\geq \epsilon \cdot |B^{\leq \ell}|$, $(\mathcal I\setminus B^{\leq \ell})\cup A^{\ell+1}\in M$  and $f_{|d}(A^{\ell+1}\mid A^{\leq \ell}\cup B^{\leq \ell})\geq d|A^{\ell+1}|$.
\State $\mathcal{C}\leftarrow \emptyset$
\ForAll{$i\in A^{\ell+1}$} 
\State $\mathcal C \leftarrow \mathcal C\cup \mbox{\sc FindCircuits}(i,\mathcal I,d,\epsilon)$
\EndFor
\State \Return $(A^{\ell+1},\mathcal C)$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\sc FindCircuits}\label{FindCircuits}
\begin{algorithmic}[1]
\Procedure {FindCircuits}{$i$, $\mathcal I$, $d$, $\epsilon$}
\State $\mathcal C(i)\leftarrow \emptyset$
\ForAll{inclusion-wise minimal $C\subseteq \{i\}\cup \mathcal I$ such that $f_{|d}(C)<(1-\epsilon)d|C|$}
\State $\mathcal C(i) \leftarrow \mathcal C(i)\cup C$
\EndFor
\State \Return $\mathcal C(i)$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\sc CollapseLayer}\label{CollapseLayer}
\begin{algorithmic}[1]
\Procedure {CollapseLayer}{$A^{\leq \ell}$, $B^{\leq \ell}$, $\mathcal I$, $d$, $\epsilon$}
\If{$\ell=0$}
\State \Return $0$
\EndIf
\State $I\leftarrow \emptyset$
\ForAll{$i\in A^{\ell}$}
\If{{\sc FindCircuits$(i,\mathcal I,d,\epsilon)=\emptyset$}}
\State $I\leftarrow I\cup \{i\}$
\EndIf
\EndFor
\If{$|I|< (\epsilon/2) \cdot  |A^{\ell}|$}
\State \textbf{return} $\ell$
\Else 
\State Let $B'\subseteq B^{\leq \ell-1}$ be a set such that $|B'|=|I|$ and $(\mathcal I \setminus B') \cup I \in M$
\State Find $\Tilde \ell$ such that $|B'\cap B^{\Tilde \ell}|\geq \gamma |B'|$
\State $\mathcal{I}\leftarrow (\mathcal I \setminus (B'\cap B^{\Tilde \ell})) \cup I$
\ForAll{$\ell\geq \Tilde \ell$}
\State $A^{\ell},B^{\ell}\leftarrow \emptyset$
\EndFor
\State $B^{\Tilde \ell-1}\leftarrow B^{\Tilde \ell-1}\setminus B'$
\State \Return {\sc CollapseLayer}($A^{\leq \Tilde \ell-1}$, $B^{\leq \Tilde \ell -1}$, $\mathcal I$, $d$, $\epsilon$) 
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{\sc MainAlgorithm}\label{MainAlgorithm}
\begin{algorithmic}[1]
\Procedure {Main}{$\mathcal I$, $i_0$, $d$, $\epsilon$}
\State $A^0\leftarrow \emptyset$
\State $B^0\leftarrow \{i_0\}$
\State $\ell\leftarrow 0$
\While{\textbf{True}}
\State {\sc BuildLayer$(A,B,\ell,\mathcal I,d,\epsilon)$}
\State $\ell\leftarrow$ {\sc CollapseLayer}$(A^{\leq \ell+1},B^{\leq \ell+1},\mathcal{I},d,\epsilon)$
\If{$\ell=0$}
\State \textbf{Terminate}
\EndIf
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\newpage 
\begin{lemma}
  After running {\sc CollapseLayer} once, we have that $|A^{\leq \ell}\setminus I^{\leq \ell}|\leq 2\left(\frac{1-\epsilon}{\epsilon}\right)\cdot  |B^{\leq \ell}|$.
\end{lemma}
\begin{proof}
Recall that {\sc CollapseLayer} maintains the invariant that the set $I$ of immediately addable elements of $A^{\leq \ell}$ satisfies
\begin{equation*}
    |I|\leq \epsilon |A^{\leq \ell}|
\end{equation*}
All the other elements $i\in A^{\leq \ell}$ are contained in a least one circuit $C_i$ such that 
\begin{equation*}
    d(1-\epsilon)|C_i|> f_{|d}(C_i)
\end{equation*}
We prove first that this implies that 
\begin{equation*}
    f_{|d}\left(\bigcup_i C_i\right)\leq (1-\epsilon)d\left|\bigcup_i C_i\right|
\end{equation*}
Consider adding the elements one by one in any order and proceed by induction. The base case is clear. Now consider some new element $i$ to add. Either $C_i\subseteq C_{<i}$ and nothing needs to be shown. Otherwise we have that 
\begin{equation*}
    (1-\epsilon)d|C_i\cap C_{<i}|\leq f_{|d}(C_i\cap C_{<i})
\end{equation*} by minimality of $C_i$.
Hence, by submodularity
\begin{align*}
    f_{|d}(C_{\leq i})&\leq  f_{|d}(C_{i})+f_{|d}(C_{< i})-f_{|d}(C_i\cap C_{< i})\\
    &\leq (1-\epsilon)d|C_i|+(1-\epsilon)d|C_{<i}|-(1-\epsilon)d|C_i\cap C_{<i}|\\
    &\leq (1-\epsilon)d|C_{\leq i}|.
\end{align*}

Now fix $\ell'\leq \ell$. By construction of $A^{\ell'}$, we have that 
\begin{equation*}
    f_{|d}(A^{\ell'}\mid A^{\leq \ell'-1}) \geq f_{|d}(A^{\ell'}\mid A^{\leq \ell'-1}\cup B^{\leq \ell' -1})\geq d|A^{\ell'}|
\end{equation*}
Summing this inequality over all $\ell'\leq \ell$ gives that 
\begin{equation}\label{eq:lower_boundfA}
    f_{|d}(A^{\leq \ell}) \geq d|A^{\leq \ell}|
\end{equation}
Next, we recall that $C_i\subseteq A^{\leq \ell}\cup B^{\leq \ell}$ for all $i\in A^{\leq \ell}$. This gives, by submodularity and monotonicity of $f$ that
\begin{align*}
    f_{|d}(A^{\leq \ell})&\leq f_{|d}(I)+f_{|d}(A^{\leq \ell}\setminus I)\\
    &\leq (\epsilon/2)\cdot d|A^{\ell}|+f_{|d}\left(\bigcup_{i\in A^{\leq \ell}\setminus I}C_i\right)\\
    &\leq (\epsilon/2)\cdot d|A^{\ell}|+(1-\epsilon)d\left| \bigcup_{i\in A^{\leq \ell}\setminus I }C_i\right|\\
    &\leq (\epsilon/2)\cdot d|A^{\ell}|+(1-\epsilon)d|A^{\leq \ell}|+(1-\epsilon)d|B^{\leq \ell}|
\end{align*}
Putting it together with equation \eqref{eq:lower_boundfA}, we get
\begin{equation*}
   d|A^{\leq \ell}|\leq  (1-\epsilon/2)d|A^{\leq \ell}|+(1-\epsilon)d|B^{\leq \ell}|
\end{equation*}
which implies
\begin{equation*}
    |A^{\leq \ell}|\leq \frac{2-2\epsilon}{\epsilon}|B^{\leq \ell}|
\end{equation*}
\end{proof}

\begin{lemma}
  Assuming the LP is feasible with objective $(\alpha d)$ for $\alpha>6$, then the procedure {\sc BuildLayer} always succeed.
\end{lemma}
\begin{proof}
We only need to prove that line $2$ of Algorithm \ref{BuildLayer} always succeed. For this purpose, add the elements into $A^{\ell+1}$ one by one. Given the current state of $A^{\ell+1}$ (with $|A^{\ell+1}|\leq \epsilon |B^{\leq \ell}|)$ we add $i$ to $A^{\ell+1}$ if $f_{|d}(i\mid A^{\leq \ell+1}\cup B^{\leq \ell})$ and if $i$ belongs to the set 
\begin{equation*}
    E=\{i\in ((U\setminus \mathcal I)\cup B^{\leq \ell})\setminus A^{\ell + 1} \mid \mathcal I\setminus B^{\leq \ell}\cup A^{\ell+1}\cup \{i\}\in M \}
\end{equation*}
First we prove that enforcing these conditions implies that
\begin{equation*}
    f_{|d}(A^{\ell+1}\mid A^{\leq \ell}\cup B^{\leq \ell})\geq d|A^{\ell+1}|
\end{equation*}
Indeed, by defining $g(S)=f_{|d}(S\mid A^{\leq \ell}\cup B^{\leq \ell})$ we have that every element is added only if 
\begin{equation*}
    g(i\mid A^{\ell + 1})\geq d
\end{equation*}
hence by a standard telescopic sum we get the first claim. The second property that 
\begin{equation*}
    (\mathcal I\setminus B^{\leq \ell})\cup A^{\ell+1} \in M
\end{equation*} 
is clear by definition of $E$. The last property that we can always get $|A^{\ell+1}|< \epsilon |B^{\leq \ell}|$ is more difficult. For the sake of contradiction, assume that for all elements in $E$ we have $f_{|d}(i\mid A^{\leq \ell+1}\cup B^{\leq \ell})<d$ and that at the same time $|A^{\ell+1}|< \epsilon |B^{\leq \ell}|$

Denote by $x^*$ the solution to the LP with objective $(\alpha d)$ and 

By Lemma TODO (same Lemma as lemma 6 in Rothvoss paper), we note that 
\begin{equation*}
    x^*(E)\geq |B^{\leq \ell}|-|A^{\ell+1}|> (1-\epsilon)|B^{\leq \ell}|
\end{equation*}
Second, by Lemma 1, for all $i\in E$ we have 
\begin{equation*}
    f(i\mid A^{\leq \ell+1}\cup B^{\leq \ell})<d
\end{equation*} hence we can write
\begin{equation*}
    d(\alpha - 1)x^*(E)\leq \sum_{i\in U}x_i^*(\alpha\cdot d-f(i\mid A^{\leq \ell+1}\cup B^{\leq \ell}))\leq f\left(A^{\leq \ell+1}\cup B^{\leq \ell}\right)
\end{equation*}
The last step will be to bound $f\left(A^{\leq \ell+1}\cup B^{\leq \ell}\right)$.

\etienne{TODO we should get:
\begin{align*}
    f\left(A^{\leq \ell+1}\cup B^{\leq \ell}\right)&\leq f\left(A^{\ell+1}\right)+f\left(I^{\leq \ell}\right)+f\left(A^{\leq \ell}\setminus I^{\leq \ell}\cup B^{\leq \ell}\right)\\
    &\leq (\alpha d)|A^{\ell+1}|+(\alpha d)|I^{\leq \ell}|+(1-\epsilon)d\left(|A^{\leq \ell}|+|B^{\leq \ell}| \right)\\
    &\leq (\alpha d)\left((\epsilon/2)|A^{\leq \ell}|+ \epsilon |B^{\leq \ell}|\right)+(1-\epsilon)d\left(|A^{\leq \ell}|+|B^{\leq \ell}| \right)\\
\end{align*}
and then use upper bound of $|A^{\leq \ell}|\leq 2\frac{1-\epsilon}{\epsilon}|B^{\leq \ell}|$ and finish the proof with the lowerbound on $x^*(E)$.
}
\end{proof}

\begin{lemma}
{\sc FindCircuits} can be implemented to run in polynomial time.
\end{lemma}
\begin{proof}
Let $i$ be the element given as input to Algorithm \ref{FindCircuits}. We want to check for every $i_0$ in $\mathcal I$, if there is an inclusion-wise minimal set $C\subseteq \mathcal I\cup \{i\}$ containing $i_0$ such that $f_{|d}(C)<(1-\epsilon)d|C|$.
\end{proof}

\section{A relaxation for multiple layers}

We present a relaxation for many layers using polymatroids. We first introduce notation, in layer $0$ there is a set $T$ of terminal players that each want one item and are not covered by anything yet. Along with these players there are fat players and items, each of these fat player is only interested to get one item of layer $0$ and is currently assigned such an item. We denote this layer by $L_0$. 

Then each layer $L_i$ for $i>0$ is organized as follows. There are thin players, fat players, and items. Each fat player is currently covered by a item of its own layer and is only interested in items of his own layer. Each thin players either wants one item of the layer $L_{i-1}$ or $d$ many items of layer $L_i$. He is currently assigned an item from layer $L_{i-1}$. Note by creating dummy players and items in layer $L_{i-1}$ we can assume that each thin player of layer $i$ is interested in only one item of layer $L_{i-1}$ and that these items are distinct among all thin players of layer $L_{i}$. We assume that all items are currently assigned to some player except in the last layer where there are some free items. For each of these free items we create a dummy thin player that is assigned this item and wants $0$ item from the layer below.

By a slight abuse of notation, we will also note by $L_i$ the set of thin players of layer $i$.

We now describe a relaxation for this problem. In this LP, there is one variable for each sequence of thin players, $A_1,A_2,\ldots ,A_k$ with $A_i\in L_i$. This variable denoted $y(A_1,A_2,\ldots ,A_k)$ indicates if $A_k$ sends flow to the top layer ($L_0$) through players $A_{k-1},\ldots ,A_2,A_1$. We will say that such a sequence is \textit{valid} if there is a path from $A_i$ to $A_{i-1}$ in layer $L_{i-1}$ for all $A_i$ in the sequence. For every thin player $A$, we will denote by $\lambda(A)$ the set of valid sequences starting at $A$ and going to the top.

For each thin player $A$, we denote by $x_A$ the total flow he sends to the top i.e.
\begin{equation*}
    x_A=\sum_{s\in \lambda(A)} y(s)
\end{equation*}

\paragraph{Flow arriving directly to terminals.} In this part we denote by $x$ the vector $(x_A)_{A\in L_1}$, i.e. the vector whose coordinates describe how much flow thin players in $L_1$ send to the top layer. There is a natural matroid on universe $L_1$ to consider here. A set $S$ is independent if there is a perfect matching from items to players $S\cup T\cup F_0$ where $F_0$ is the set of fat players from layer 0. If we consider the co-matroid of this matroid, then we want that $x$ is a basis of the comatroid to solve our problem. Hence we just need to put matroid constraints and a basis constraint on $x=(x_A)_{A\in L_1}$ to ensure feasiblity of the solution in layer $L_0$ i.e. if $r$ is the rank function of the matroid then we want that 
\begin{align*}
    \sum_{A\in L_1} x_A = r(L_1) &\\
    \sum_{A\in S} x_A \leq r(S) &\quad \forall S\subseteq L_1
\end{align*}

\paragraph{Routing among light agents.} For a sequence $s$ of length $k$ and a thin player $A\in L_{k+1}$, we denote by $s\circ A$ the sequence $s$ where we append $A$ at the end. For a sequence $s$ and a thin player $A$, we denote by $p(s,A)$ the set of valid sequences finishing in $A$ and containing $s$ as a prefix. We can then write the following constraints.

\begin{align*}
    \forall i, \forall A\in L_i, \forall s\in \lambda (A), & \sum_{A'\in L_{i+1}} y(s\circ A') = d\cdot y(s)\\
    \forall s, \forall A, &\sum_{s'\in p(s,A)}y(s')\leq y(s)\\
    \forall A, &\sum_{s\in \lambda(A)} y(s)\leq 1
\end{align*}
The first constraint is simply stating that if a player $A$ gives away a value $y(s)$ of its big item through the sequence $s$, then he must get at least $d$ times this value from player in the next layer through the correct sequence (that should contain $s$ as a prefix). The second contraint is a capacity constraint that for any player $A$ and any sequence $s$, the total flow that $A$ can send through sequences that all contain $s$ as a prefix cannot exceed $y(s)$. The last constraint is simply stating that $A$ cannot give away its item more than once.

\paragraph{Routing inside a layer.} Recall that we define
\begin{equation*}
    x_A=\sum_{s\in \lambda(A)} y(s)
\end{equation*}
For each layer $L_i$ ($i\geq 1$) we put our polymatroid constraints that are:
\begin{equation*}
    \forall i\geq 1, \forall S\subseteq L_i\cup L_{i+1}, \sum_{A\in L_i} x_A(d-f(A\mid S)) + \sum_{A\in L_{i+1}} (1-x_A)(1-f(A\mid S)) \leq f(S)
\end{equation*}
Here $f$ can be thought of the submodular function that is equal to the maximum flow we can send to players in $S$ assuming the fat items currently assigned to thin players of $L_{i+1}$ are free.

\subsection{A useful example}

This extension is inspired by the example of Bansal and Srividenko. In $L_0$ we have one terminal and $d$ items. The terminal is interested in any of these items. Each of these items is currently assigned to a thin player in $L_1$ (so there are $d$ players in $L_1$). For each player of $L_1$ we create a tree containing $d$ items in $L_1$. Each of these items are assigned to a thin player in $L_2$ (hence $d$ thin players in $L_2$ per tree so $d^2$ in total). In the last layer of the tree there are $d$ items and the players of $L_2$ in the corresponding tree are interested in any of these items. See picture below for $d=3$.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{example.pdf}
    \caption{Example for $d=3$}
    \label{fig:example}
\end{figure}




It is clear that if any of the thin player in $L_1$ gives up his big item (which is necessary to satisfy the terminal) then if this player takes $d/\alpha$ items from $L_1$ then at least $d/\alpha$ corresponding players in $L_2$ must share $d$ items in $L_2$ together. Each one of them wants $d$ items and one of them has to get less than $d/(d/\alpha)=\alpha$. So $\OPT$ is at most $\min (\alpha/d, 1/\alpha) \leq 1/\sqrt{d}$. 


==> OverleafV1/proofs_with_flow.tex <==

\section{Fat and thin players}
We are considering a setting which generalizes the (non-trivial)
$1, \epsilon$ case of restricted Santa Claus,
but also covers the integrality gap example.

There are fat items $R_f$ (value $v_j = k$) and thin items $R_t$ ($v_j = 1$);
fat players $P_f$ (demand $d_i = k$) and thin players $P_t$ ($d_i = 1$).
Each player $i$ is interested in a set of items $R(i)$.
We restrict ourselves to the case where thin player are only interested
in thin items.

We assume there exists a solution that assigns to each player
items of total value at least their demand.
In other words, each fat player gets either one fat item or $k$ thin items, and
to each thin player gets one thin item.

We will prove that a generalization of the local search algorithm 
is able to assign each thin player one thin item and
each fat player either one fat item or $k/4$ thin items
(assume for simplicity $k/4$ is integer).

\subsection{Algorithm}
We first calculate a feasible solution for only the thin players
(this is the unit size problem, which is easy)
and then augment the solution to cover one additional
fat player $i_0$ in each iteration.

We need to define a certain flow network to handle finding thin addable edges
for fat players.
This is essential the residual graph of bipartite matching.
Consider some previously computed assignment of thin resources.
We want every thin player to maintain a thin item
(but they can swap theirs for another).
Fat players may act as sources or sinks, i.e., we
may steal from fat players or give them more thin items.
We write the following flow network $G^t$ with integral capacities:
There is a node for each player and each thin item.
There is an arc from each player to each thin item they currently have
with capacity $1$. There is an arc from each
thin item to each player that is interested in it (but does not currently have it)
of capacity $\infty$.
Moreover, define a network $G^t(Q)$ for $Q\subseteq P_f$,
where we delete the outgoing arcs of the fat players $Q$.
Network $G^t(Q)$ does not allow to steal items from players $Q$.

We run a generalization of the local search.
As before we have addable edges and blocking edges.
There are three types of edges
\begin{itemize}
\item A unit edge, which contains one thin player and one thin item
 he is interested in;
\item A fat edge, which contains one fat player and one fat item;
\item A thin edge, which contains one fat player and $k/4$ thin items. 
\end{itemize}
We write $B^u, B^f, B^t$ ($B = B^u\cup B^f\cup B^t$)
for the blocking edges of these types and
$A^u, A^f, A^t$ for the addable edges.
The general approach of the algorithm is as follows:
When there is an edge $e$ disjoint from $(A\cup B)_R$ (the items in
$A$ and $B$, where $e_P$, the player in $e$, is in
$B_P \cup \{i_0\}$ (the players in the blocking edges and the new player),
we might add this as an addable edge. 
When some edge in the current matching intersects with the items
in this addable edge, we add it to the blocking edges.

We constraint this algorithm slightly.
Firstly, we always prioritize unit edges when adding new addable edges.
Secondly, we only add thin addable edges in the following way.
When considering an edge for player $i$,
we require that there are $k/4$ item-disjoint paths in $G^t(P_f\cap B_P)$
that start in some non-blocking fat player $i'\in P_f\setminus B_P$
and end in $i$.
Such paths can be found by computing a maximum flow from $P_f\setminus B_P$
to $i$.
These paths correspond to a thin edge for player $i$,
which we use as an addable edge (take the last item in each path).

Note that the constraint for the paths
(together with prioritization of the unit edges)
implies that thin addable edge are disjoint from the
previous addable or blocking edges:
Consider one of the
paths $i_1,j_1,\dotsc,i_\ell,j_\ell,i$ and suppose some $j_k$ is in
a blocking or addable edge. Choose $k$ minimal.
If $j_k$ is in a blocking thin edge,
this means $i_k\in P_f \cap B_P$.
However, by construction $G^t(P_f\cap B_P)$ does not have outgoing
edges for $i_k$. If it is in a unit blocking edge, then it is also in
an addable edge.
Hence, consider only the case that $j_k$ is in an addable edge.
Player $i_k$ is currently assigned item $j_k$. Hence, $i_k\in B_P$.
Since players in $P_f\cap B_P$ have no outgoing arcs, $i_k$ must
be a thin player. In particular, $k > 1$ (player $i_1$ is fat).
Player $i_k$ is interested in item $j_{k-1}$. Since $k$ is chosen
minimal, $j_{k-1}$ is not in an addable or blocking edge.
Thus, the unit addable edge $(i_k, j_{k-1})$ would have been chosen
over the thin addable edge by priority. A contradiction.

Adding this thin addable edge will result in adding at least one
thin blocking edge (the players from where the paths come) or
the addable edge will immediately collapse, if all paths come from
unassigned resources.

\subsection{Analysis}
By the same arguments as in the original variant this algorithm terminates
(or gets stuck).
We now show that it does not get stuck.

Suppose toward contradiction no addable edge exists.
Recall $B^t$ denotes the thin blocking edges and $B^f$ the fat blocking edges.
Let $T^f\subseteq B^f$ be those edges $e$
where $e_P$ has a fat item in the optimal solution
and let $F^f = B^f\setminus T^f$.
Let $T^t\subseteq B^t$ be those edges $e$
where $e_P$ does not have a fat item in the optimal solution
and let $F^t = B^t\setminus T^t$.

The notation reads as 'true fat', 'false fat', 'true thin', 'false thin'.
\bigskip

\begin{tabular}{l|l|l}
  
  & & player has \\
  & & fat item in \\
  & & current solution \\\hline
  player has fat item in OPT & $F^t$ & $T^f$ \\\hline
                             & $T^t$ & $F^f$
\end{tabular}
\bigskip
\begin{lemma}
  If the algorithm is stuck, $|F^f| \le |B^t|$.
\end{lemma}
\begin{proof}
Suppose toward contradiction $|F^f| \ge |B^t|$.
We consider the flow in $G^t$ that is derived from augmenting the current solution
(of small items) to the optimal one.
In this flow every player in $F^t$ loses at most $k / 2$ items (in sum).
Every player in $T^t$ gains at least $k/2$ items (in sum).
Every player in $F^f$ gains at least $k$ items (in sum).
Every player in $T^f$ does not lose thin items, since he has none.
We can decompose the flow into paths, where each path corresponds
to a sequence of item moves and each path starts with a player
that loses items and ends with a player that gains items.
Moreover, the paths are disjoint on the items.

Now take all $|F^f| k \ge |F^f| k/4 + |B^t| \cdot 3/4 \cdot k$ paths
that end in players in $F^f$.
At most $|F^t| k/2 \le |B^t| k/2$ of these paths begin in a player in $F^t$.
We forget about these and we are left with at least
$|F^f\cup B^t| k/4$ paths that
start in a player not in $B_P$ and end in a player in
$F^f$. Stop each path at the first player in $P_f\cap B_P$.
Now these are also valid paths in network $G^t(P_f\cap B_P)$.
Since the paths cannot cross $T^f$ (those player have no outgoing arcs
in $G^t$ because they have no thin items),
we have $|F^f\cup B^t| k/4$ paths starting
in $P_f\setminus B_P$ and ending in $F^f\cup B^t$.
By pidgeon-hole principle there is one player in $B^t\cup F^f$
where least $k/4$ paths end.
Hence, this player has an addable edge. A contradiction.
\end{proof}

\subsection{Proof fixed with correct network}
We consider the network where each thin item has an incoming edge of capacity $1$ from the player that currently has it or from the source $s$ if the item is not assigned yet. Each player has incoming edges of capacity $1$ from every thin item he is interested in but that he does not have yet. We remark that the indegree of every item in this network is exactly $1$.
\begin{lemma}
  If the algorithm gets stuck, then there is no feasible solution.
\end{lemma}
\begin{proof}
  Consider the network above, except that each non blocking player has an incoming edge from the source of capacity $\infty$ and each player in $B_t\cup F_f\cup \{i_0\}$ has an outgoing edge of capacity $\infty$ to the sink $t$. Since the algorithm is stuck, it must be that the maximum flow in this network is at most $(|B_t\cup F_f|+1)\frac{k}{4}$. Hence the minimum $s$-$t$ cut is of value at most $(|B_t\cup F_f|+1)\frac{k}{4}$. Note that all the non blocking players are on the $s$ side of the cut while all the players in $B_t\cup F_f\cup \{i_0\}$ are on the $t$ side of the cut. We claim the following.
  
  \begin{claim}
    All the edges in the minimum cut are from a player to an item he is currently assigned or from the source to an unassigned item.
  \end{claim}
  \begin{proof}
    There are three types of edges, from item to player, from player to item, and from source to unassigned item. Assume an edge from item to player is in the minimum cut. Then by moving this item to the $t$ side of the cut, we do not increase the size of the cut since items have indegree at most $1$.
  \end{proof}
  
  We then set the dual variables as follows.
  \begin{enumerate}
      \item For every fat player in a blocking edge, $y_i=k$
      \item For every fat item in a blocking edge, $z_j=k$
      \item For every thin player on the $t$ side of the cut and also in a blocking edge we set $y_i=1$.
      \item For every thin item that a blocking player (or $i_0$) on the $t$ side of the cut is interested in, we set $z_j=1$.
      \item We set $y_{i_0}=k$.
  \end{enumerate}
  
  We check the dual is feasible. If $i$ is a fat player with $y_i>0$, then $i$ is in a blocking edge. If $i\in T_f$, then all fat items he is interested in also have value $k$ by point 2 (if a fat item he was interested had value zero, it would mean the item is not in a blocking edge and the algorithm cannot be stuck). If $i\notin T_f$, then $i\in B_t\cup F_f\cup \{i_0\}$. By point $2$ again, all fat items $i$ is interested in are in a blocking edge. Since $i$ must be on the $t$ side of the cut, all thin items he is interested in have value $1$. If $i$ is a thin player with $y_i>0$, then $i$ is a blocking player on the $t$ side of the cut. By point $4$, all items he is interested in have value $1$. Overall the dual is feasible.
  
  We now proceed to the final counting. We note that in the sum $\sum_i z_i$, we account for both fat items and thin items. For fat items, the only items with non zero value are also in a blocking edge hence there is a injective mapping from these items to the set $B_f$ and we have
  \begin{equation*}
      \sum_{i,\mbox{ $i$ is fat}} z_j \leq |B_f|k
  \end{equation*}
  
  For thin items, we decompose the sum into several cases: if an item is in a thin addable or blocking edge, if it is in a unit blocking edge, if it is neither of the previous cases but a blocking player on the $t$ side of the cut is interested in it. 
  
  The first case accounts for a total of at most $|A_t\cup B_t|\frac{k}{4}$. The second case accounts for a total of at most $|P'|$ where $P'$ is the set of thin players on the $t$ side of the cut that are blocking. The last case accounts for a total of at most $(|B_t\cup F_f|+1)\frac{k}{4}$. To see this, notice that if the item is not in a blocking or addable edge it must be that the player $i$ with $y_i>0$ interested in it is a fat player (otherwise the algorithm is not stuck). This item is either unassigned or is assigned to some non blocking player. Hence in both cases this item counts for $1$ in the minimum cut. Therefore there are at most $(|B_t\cup F_f|+1)\frac{k}{4}$ may of these. 
  
  We can now compute 
  \begin{multline*}
      \sum_i y_i - \sum_j z_j = \left(|B_t|k + |B_f|k + |P'| + k\right)-\left(|A_t\cup B_t|\frac{k}{4} + |B_f|k + |P'| + (|B_t\cup F_f|+1)\frac{k}{4}\right) \\
      \geq \left(|B_t|k + |B_f|k + |P'| + k\right)-\left(|B_t|\frac{k}{2} + |B_f|k + |P'| + (|B_t|+|F_f|+1)\frac{k}{4}\right)\\
      \geq |B_t|\frac{k}{4} + \frac{3k}{4} - |F_f|\frac{k}{4} >(|B_t|-|F_f|)\frac{k}{4}>0
  \end{multline*}
\end{proof}

\subsection{$O(\log n)$ layers}
In this section, we assume we have $O(\log (n))$ layers and that the algorithm is stuck in all the layers to reach a contradiction. We will note all the sets with a superscript $\ell$ to indicate in which layer it is. For instance $B_t^\ell$ denotes the blocking thin edges on layer $\ell$. The bottom layer is layer $1$. We take the convention that superscript $0$ means an emptyset. 

We run the algorithm to reach a $\alpha$-approximation, i.e. we want to assign either a big item or $k/\alpha$ thin items to big players.

We first generalize the first lemma.

\begin{lemma}
  If the algorithm is stuck, then for all $\ell\geq 1$
  \begin{equation*}
      |F_f^\ell| \leq \frac{|B_t^\ell|}{\alpha-1}+\frac{\alpha}{\alpha-1}\frac{|F_f^{(\ell-1)}|}{k}
  \end{equation*}
\end{lemma}
\begin{proof}
  Consider as in the first lemma when we augment our current solution to the optimal one. First consider the flow coming from unassigned resources or non blocking players. For each blocking player, this incoming flow cannot be more than $k/\alpha$ otherwise the algorithm is not stuck. Hence by ignoring this flow, we ignore an incoming flow of at most $k/\alpha$. We can now enumerate the cases in layer $\ell$.
  
  \begin{enumerate}
      \item Players in $T_f^\ell\cup T_f^{(\ell-1)}$ do not receive nor send flow.
      \item Players in $F_f^\ell$ receive a flow of $k-k/\alpha$.
      \item Players in $F_t^\ell$ send a flow of $k/\alpha$.
      \item Players in $T_t^{\ell}$ receive a flow of $k-2k/\alpha$.
      \item Players in $F_f^{(\ell-1)}$ send a flow of $1$.
      \item Players in $F_t^{(\ell-1)}$ receive a flow of $1$.
      \item Players in $T_t^{(\ell-1)}$ do not send nor receive flow in this layer. 
  \end{enumerate}
  
  Hence by flow conservation, it must be that 
  \begin{equation*}
      |F_f^\ell|k(1-1/\alpha)+|T_t^\ell|k(1-2/\alpha)+|F_t^{(\ell-1)}|\leq |F_t^\ell|k/\alpha + |F_f^{(\ell-1)}|
  \end{equation*}
  which implies our claim.
\end{proof}

We finish the proof as follows.
\begin{lemma}
  Assume the algorithm is stuck in all layer, then there is no feasible solution.
\end{lemma}
\begin{proof}
  We argue separately as in the case with only one layer. With the same arguments, we can set a feasible dual solution so that we get
  \begin{equation*}
      \sum_{i, \mbox{\footnotesize $i$ is in layer $\ell$}} y_i - \sum_{j, \mbox{\footnotesize $j$ is in layer $\ell$}} z_j > (|B_t^{\ell}|(1-3/\alpha)-|F_f^{\ell}|/\alpha)k^\ell
  \end{equation*}
  
  Then summing over all the layers we get:
  
  \begin{equation*}
      \sum_i y_i - \sum_j z_j > \sum_\ell (|B_t^{\ell}|(1-3/\alpha)-|F_f^{\ell}|/\alpha)k^\ell
  \end{equation*}
  Choose $\alpha>6$ so that $1-3/\alpha>1/2$. We then want to prove that
  \begin{equation*}
      \frac{1}{2}\sum_{\ell} |B_t^\ell|k^\ell > \sum_{\ell} |F_f^\ell|k^\ell/\alpha
  \end{equation*}
  Using the recursion formula in the previous lemma, we get that on the right hand side, each $|B_t^\ell|$ is counted at most
  \begin{equation*}
      \frac{k^\ell}{\alpha(\alpha-1)}\left(1 +  \frac{\alpha}{\alpha-1} + \left(\frac{\alpha}{\alpha-1}\right)^2 + \ldots + \left(\frac{\alpha}{\alpha-1}\right)^{O(\log n)}\right)
  \end{equation*}
  which is less than 
  \begin{equation*}
      \frac{k^\ell}{\alpha}\left(\frac{\alpha}{\alpha-1}\right)^{O(\log n)}
  \end{equation*}
  which for $\alpha=\Theta (\log n)$ is indeed smaller that $\frac{k^\ell}{2}$.
\end{proof}


\subsection{Old proof}
\begin{lemma}
  If the algorithm gets stuck, then there is no feasible solution.
\end{lemma}
\begin{proof}
  We consider the configuration LP, but for all players in $T^f$
  we allow only configurations that contain a fat item.
  Since players in $T^f$ have a fat resource in the integral solution,
  we know that the LP is still feasible with this restriction.
  The advantage here is that the dual has fewer constraints;
  hence, it is easier to get a contradiction.

  Take the flow network $G^t(B_f\cap B_P)$. We add a source $s$ and sink $t$.
  From the source $s$ to every fat player not in $B_P \cup \{i_0\}$
  we add an arc of capacity $\infty$. From every fat player in
  $(B^t \cup F^f)_P \cup \{i_0\}$ we add an arc of capacity $\infty$ to the sink.
  Since there is no addable edge, we know that this network has
  a maximum flow of less than $(|B^t \cup F^f| + 1) k / 4$.
  In particular, there is a cut of size less than $(|B^t \cup F^f| + 1) k / 4$.
  Let $P'$ be the set of players that are on the side of the sink in this
  cut. Clearly, all fat players in $P'$ are also in $B_P\cup\{i_0\}$,
  since otherwise an infinite arc would be in the cut.
  Moreover, $(B^t \cup F^f)_P \cup \{i_0\} \subseteq P'$.
  Every finite arc in the network goes from a player to a thin item that
  he is interested in (and has capacity $1$). Let $R'$ be the thin items
  that are not assigned to players in $P'$, but that some player in $P'$
  is interested in. These resources and players form all arcs in the minimum cut.
  Hence, $|R'| < (|B^t \cup F^f| + 1) k / 4$.
  
  \begin{enumerate}
    \item For every (fat) player $i\in B^t_P$ set $y_i = k$;
    \item For every (fat) player $i\in B^f_P$ set $y_i = k$;
    \item For every (fat) item $j\in B^f_R$
          set $z_j = k$;
    \item For every (thin) item $j\in (A^t\cup B^t)_R$ set $z_j = 1$;
    \item For every thin player $i\in P'$ we set $y_i = 1$;
    \item For every (thin) item that is assigned to a thin player in
          $P'$ we set $z_j = 1$;
    \item For (thin) every item in $R'$ we set $z_j = 1$.
    \item We set $y_{i_0} = k$;
  \end{enumerate}
  All other players and items get value $0$.

  Let $i$ be a player and $C$ a configuration for $i$.
  If $y_i = 0$, then trivially $z(C) \ge y_i$.
  If $y_i > 0$ and $i$ is thin, then $i\in P'$.
  Thus $z(C) = v(C) \ge 1 = y_i$ (here we use that all items $i$ is interested
  in have $z_j = 1 = v_j$).
  If $y_i > 0$ and $i$ is fat, then $i$ is either the new player or in some
  blocking edge.
  First suppose that $i$ is in some edge of $T^f$. Recall, here we
  require that $C$ contains a fat item. Thus, $z(C) \ge k = y_i$.
  Otherwise, $i\in B^t \cup F^f \cup \{i_0\}$. Hence $i\in P'$.
  This means all items that $i$ is interested in have $z_j = v_j$ and
  therefore $z(C) = v(C) \ge k = y_i$.

  Finally, we calculate
  \begin{multline*}
    \sum_{j} z_j \le \underbrace{|A^t \cup B^t| k/4}_{(4)} + \underbrace{|B^f| k}_{(3)} + \underbrace{|P'|}_{(6)} + \underbrace{(|B^t \cup F^f| + 1) k/4}_{(7)} \\
    \le |B^t| k/2 + |B^f| k + |P'| + |B^t| k/2 + k/4 \\
    < \underbrace{|B^t| k}_{(1)} + \underbrace{|B^f| k}_{(2)} + \underbrace{|P'|}_{(5)} + \underbrace{k}_{(8)} \le \sum_{i} y_i .
  \end{multline*}
\end{proof}

\section{Iterative rounding idea (Refuted)}
It seems this does not work.
\paragraph{Setting.}
There are $\ell$ layers.
Each layer $h$ consists of a set of thin players $P^t_h$
and a network of resources $R_h$ and fat players $P^f_h$.
With the exception of the first layer
each thin player is connected to a single private
resource of the previous layer. In addition, it
is connected to $k$ private resources of its layer
below. Here private means that no other thin player
is connected to this resource.
However, there is a network of fat players and other resources
that connects the $k$ resources of each thin players
to the single resource of thin players
in the next layer.

Next we introduce the following abstraction of the networks
and fat players in a layer.
Of each layer $h$ let $R^f_h\subseteq R_h$ denote the resources in this layer
of which a thin player has a single private one.
Likewise, let $R^t_h\subseteq R_h$ denote those resources in layer $h$
of which thin players have $k$ private ones.
Recall that $R^t_h$ and $R^f_h$ are connected by a network
of fat players and additional resources.
We define a matroid $(R^{ft}_h, I_h)$
on the universe $R^{ft}_h = R^t_h \cup R^f_h$.
A set $S\subseteq R^{ft}_h$ is independent, i.e., $S\in I_h$,
if there is an allocation of $R_h\setminus S$ to
to fat players. It can be seen that this is a matroid,
because it is a minor of the transversal matroid.
We can assume w.l.o.g.\ that for a thin player $i$ all
his private items are symmetric in this matroid, i.e.,
they behave the same.

\paragraph*{Linear program.}
Let $i\in P^t_h$ and $0 \le z \le 1$.
We define $\chi_h^t(i, z) \in [0,1]^{R^{ft}_h}$ as the
vector $x$ that has $x_j = 0$ for all resources $j$
that are not private to $i$ and $x_j = z$ for all that
are.
Similarly, for $i\in P^t_{h+1}$ we define
We define $\chi_h^f(i, z) \in [0,1]^{R^{ft}_h}$ as the
vector $x$ that has $x_j = 0$ for all resources $j$
that are not the single private item of $i$
and $x_j = z$ for the private item.

We abuse notation by using $I_h$ also to refer
to the polytope of the matroid $(R^{ft}_h, I_h)$.
Our linear program has one variable $y_i$ for each
thin player. A value $y_i = 0$ describes that
the player takes his single unique resource from the previous
layer and a value $y_1 = 1$ describes that
he takes the $k$ resources from its own layer.
\begin{align*}
    y_i &= 1 &\text{for each thin player $i$ in layer $1$} \\ 
    \sum_{i\in P^t_h} \chi_h^t(i, y_i) + \sum_{i\in P^t_{h+1}} \chi_h^f(i, 1 - y_i) &\in I_h &\text{for all layers $h$} \\
    0 \le y_i &\le 1 &\text{for each thin player $i$}
\end{align*}

\paragraph*{Iterative rounding.}
Our plan is to round the LP solution starting with the
thin players in the second layer. More precisely,
we fix the values $y_i$ for the thin players in the third layer
(even though fractional).
Then we restrict the LP to the variables $y_i$ of players in
the second layer, i.e., $i\in P^t_2$.
The $y_i$ values of the third layer are hardcoded constants
and so are those of the first (as they must be $1$).
Constraints of layers $3,4,\dotsc$ are removed.

For thin players in the second layer we round
the values $y_i$ to $0$ or $1$ maintaining feasibility
of the linear program
and assuring that we can give $k/\log(n)$
resources to each thin player in the first two layers.
Then we delete the topmost layer from the instance
and repeat.
This step is implemented by a local search procedure.

\section{Polynomial time algorithm}
In this section we will describe a polynomial time local search.
For now only the algorithm (and perhaps running time analysis).

\paragraph*{Setting and notation.}
There are $h$ distance levels $D_1,\dotsc,D_h$. Each level $D_d$ is a tuple $(T(d), F(d), R(d))$.
We call $T(d)$ the complex players, $F(d)$ the simple players, and $R(d)$ the resources.
Define for convenience $T(h+1) = \emptyset$.
There is a bipartite graph on $(T(d) \cup T(d+1) \cup F(d), R(d))$
describing which player is interested in which resources.
A player in $T(d)$ is interested in exactly $k$ resources, a player in $T(d+1)$
is interested in exactly one resource.
A feasible solution is an integral flow in the bipartite graph of each level
with the resources as sources and the player as sinks.
It satisfies the following.
Each simple player receives a flow of $1$. Each complex player in $T(d)$ either receives
a flow of $1$ in level $d-1$ or a flow of
\begin{equation*}
  \frac{k}{\alpha} \cdot \frac{h + 1 - d}{h}
\end{equation*}
in level $d$ (or both). We call a complex player \emph{double-covered} if he
has flow from both levels.

A partial solution is one where some of the complex players in $T(1)$ receive no flow.
We start with a partial solution where no complex player in $T(1)$ receives flow
(we can assume there is a trivial partial solution that satisfies this).
Then we change the solution so that one more complex player in $T(1)$ receives a flow
of $k/\alpha$.

We also consider the residual network derived from these flows.

\paragraph*{Local search data structure.}
The local search maintains a sequence of layers $L_1,L_2,\dotsc$
(not to be confused with levels).
Each Layer is a tuple $(d_i, \Delta^+_i, \Delta^-_i, A_i, B_i, I_i)$.
The number $d_i\in\{1,2,\dotsc,h\}$ describes
the level of the residual network that this layer is involved in.
The values $\Delta^+_i, \Delta^-_i \in \{0, 1\}$ determine that the
layer tries to give resources to the complex players $T(d_i + \Delta^+_i)$
and takes away resources from $T(d_i + \Delta^-_i)$.
The addable players $A_i$ are a subset of $T(d_i + \Delta^+_i)$ and
all of them do not currently have resources in $d_i$.
The blocking players $B_i$ are a subset of $T(d_i + \Delta^-_i)$ and
they all have resources in level $d_i$.
We write  $A_{\le j} = \bigcup_{i\le j} A_i$ and $B_{\le j} = \bigcup_{i\le j} B_i$.
Furthermore, we denote by $A_{\le j}(d)$ and $B_{\le j}(d)$ the addable players and
blocking players of layers $i \le j$ with $d_i = d$.
The set $I_i \subseteq R(d_i)$ consists of
resources currently assigned to double covered players.

Intuitively, the algorithm tries to double-cover addable players.
For that, it tries to take resources (or flow) away from the blocking players.
Later layers will try to double-cover the blocking players. If this succeeds,
they can give up their resources in level $d_i$ to give flow to the addable players.

We let $L_\ell$ denote the maximum layer at some state ($\ell$ changes during the algorithm's execution).

\paragraph*{Local search invariants.}
We ensure that $A_i \subseteq B_{\le i-1}(d_i)$ and for each layer $i$.

TODO: More.

\paragraph*{Collapsing a layer.}
TODO: This all needs adjustments.

Suppose for a layer $L_i$ we have that $|B_i|/100$ of the blocking players
are double-covered. Then we release the resources in $R(d_i)$ that these players
currently have. 

Oversimplified:
We augment the current partial solution along the flow from $B_i$ to $A_i$,
thereby double-covering a significant portion of players in $A_{i}$.
Then we remove all layers after $L_{i}$.

Reality:
We need to ensure that this flow does not interact with the flows in lower layers.
To do this we proceed like in [Annamalai??] with the $I_i$.
We iterate over all layers $i'$ with $d_{i'} = d_i$.
We start with $X = I_{\le i}$ and $Y = \emptyset$
maintaining a maximum flow from $X$ to $Y$.
We augment the flow to a maximum flow from
$X$ to $Y \cup A_{i'}$;
then from $X\cup B_{i'}$ to $Y \cup A_{i'}$.
Finally we add $B_{i'}$ to $X$ and
$A_{i'}$ to $Y$.

\paragraph*{Building a new layer.}
If there is no layer that can be collapsed, we build a new one.
We iterate over $(d, \Delta^+, \Delta^-)$ in lexicographically decreasing order until we succeed.
Our goal is to construct a layer $(d,\Delta^+, \Delta^-, A, B, I)$.

\begin{description}
\item[Case:  $\Delta^+ = \Delta^- = 1$.]
We consider the flow network in the residual graph of level $d$.
We build $A$ and $B$ greedily maintaining that $|B| = |A|$ and there is a flow of $|B| = |A|$ from $B$ to $A$. Let $i\in B_{\le \ell} \cap T(d+1), i'\in T(d+1) \setminus B_{\le \ell}$ such that $i$ does not have a resource in $R(d)$ and $i'$ has one. We add $i$ to $A$ and $i'$ to $B$
if: The flow from $B\cup\{i'\}$ to $A\cup\{i\}$ is greater (by one) that the flow from $B$ to $A$; and the LP is feasible (TODO: formalize) for $B\cup\{i\}$.

\item[Case:  $\Delta^+ = 1, \Delta^- = 0$.]
We consider the flow network in the residual graph of level $d$.
We compute a maximum flow from $T(d) \setminus B_{\le \ell}$ to $B_{\le \ell} \cap T(d+1)$.
We set $A$ to all sinks that receive a flow (of one) and $B$ to all sources that
give away any flow.

\item[Case:  $\Delta^+ = 0, \Delta^- = 1$.]
We consider the flow network in the residual graph of level $d$.
We build $A$ and $B$ greedily starting with the empty set.
We maintain that there is a flow from $B$ to $A$ sending a large flow to each
player in $A$ (TODO: formalize).
Let $i\in B_{\le \ell} \cap T(d)$. We now build a temporary set $S$.
Let $i'\in T(d+1)\setminus B_{\le\ell}$. We add $i'$ to $S$ if the flow
from $B\cup S \cup \{i'\}$ to $A\cup \{i\}$ is larger (by one) than the flow from
$B\cup S$ to $A\cup \{i\}$; and the LP is feasible for $B\cup S \cup \{i'\}$ (TODO: formalize).
If no player can be added to $S$ and $S$ is very big (TODO: formalize) we
add $i$ to $A$ and $S$ to $B$. Otherwise, we discard $i$ and $S$.

\item[Case:  $\Delta^+ = 0, \Delta^- = 0$.]
We consider the flow network in the residual graph of level $d$.
We build $A$ and $B$ greedily starting with the empty set.
We maintain that there is a flow from $B$ to $A$ sending a large flow to each
player in $A$ (TODO: formalize).
Let $i\in B_{\le \ell} \cap T(d)$.
We compute a maximum flow from $T(d) \setminus B_{\le \ell}$ to $A\cup\{i\}$.
If the flow is much larger (TODO: formalize) than that from $T(d) \setminus B_{\le \ell}$
to $A$, then we add $i$ to $A$.
Once no more player can be added to $A$ we set $B$ to be the sources of the flow
that give away any flow.
\end{description}

If the new layer is small (TODO: formalize) this combination of $d,\Delta^+,\Delta^-$ has failed and is discarded.
\newpage
\section{Poly time 2 levels}

\paragraph*{Setting and notation.}
There are $2$ distance levels $D_1,D_2$.
There are complex players $T(2)$ and simple players $F(2)$ in the second level
and resources $R(1), R(2)$ in both levels.
There is a bipartite graph $G(1)$ on $(T(2), R(1))$
and a bipartite graph $G(2)$ on $(F(2) \cup T(2), R(2))$
describing which player is interested in which resources.
A player in $T(2)$ is interested in exactly $k$ resources of $R(2)$
and one resource in $R(1)$. A player in $F(2)$ is interested in exactly one resource in $R(2)$.
A feasible solution is an integral flow in each bipartite graph $G(1)$ and $G(2)$
with the resources as sources and the player as sinks.
It satisfies the following.
Each simple player in $F(2)$ receives a flow of $1$. Each complex player in $T(2)$ either receives
a flow of $1$ in level $G(1)$ or a flow of $k/\alpha$
in $G(2)$ (or both). We call a complex player \emph{double-covered} if he
has flow from both levels.

A partial solution is one where some of the complex player in $T(2)$ receive no flow.
We start with a partial solution where no complex player in $T(2)$ receives flow in $G(2)$
and a maximal number of them receive flow in $G(1)$
(we can assume there is a trivial partial solution that satisfies this).
Then we change the solution so that one more complex player in $T(2)$ receives a flow
of $k/\alpha$.

We also consider the residual network derived from these flows.

We define the weight of a player $w(i)$ as $1$ if $i\in T(2)$ and $1/k$ if $i\in F(2)$.
For some set $A\subseteq T(2)\cup F(2)$ we write $w(A)$ for the sum of weights.

\paragraph*{Local search data structure.}
The local search maintains a sequence of layers $L_1,L_2,\dotsc$
(not to be confused with levels).
Each Layer is a tuple $(d_i, A_i, B_i, I_i)$.
The number $d_i\in\{1,2\}$ describes
the residual network that this layer is involved in, i.e, that of $G(d_i)$.
The addable players $A_i$ are a subset of $T(2)$ and
all of them do not currently receive flow in $G(d_i)$.
The blocking players $B_i$ are also a subset of $T(2)$ and
all of them receive flow in $G(d_i)$.
We write  $A_{\le j} = \bigcup_{i\le j} A_i$ and $B_{\le j} = \bigcup_{i\le j} B_i$.
The set $I_i \subseteq R(d_i)$ consists of
resources currently not assigned or assigned to double covered players.

Intuitively, the algorithm tries to double-cover the addable players.
For that, it tries to take resources (or flow) away from the blocking players.
Later layers will try to double-cover the blocking players. If this succeeds,
they can give up their resources in level $d_i$ to give flow to the addable players.

We let $L_\ell$ denote the maximum layer at some state ($\ell$ changes during the algorithm's execution).

\subsection{first layer}
Perform actions in the second layer whenever possible.
\paragraph*{Invariants.}
We maintain that for each layer $i$ with $d_i = 1$ there is a flow in the residual graph of $G(1)$
from $I_{\le i}\cup B_i$ to $A_i$ of value at least $|A_i|$.

\paragraph*{Collapsing a layer.}
Suppose for a layer $L_i$ with $d_i = 1$ we have that the number of blocking players in $B_i$ that are
double-covered and $|I_{\le i}|$ together are at least $|A_i|/100$.
Let $I$ denote the resources assigned to these double-covered players.
Intuitively we would like to augment the current flow to reroute flow from $I_{\le i} \cup I$ to $A_i$
and double-cover a significant fraction of them. However, this will change the residual graph of $G(1)$ and
it could destroy the structure of previous layers (in particular, the invariant on the flow).
The following is similar to [Annamalai??].

Let $h_1,h_2,\dotsc$ denote the indices of layers with $d_{h_j} = 1$.
We compute a maximum flow in the residual graph of $G(1)$ from $I_{\le i} \cup I$
to $A_{h_1}$.
For $j=2,3,4,\dotsc$ we augment this to a maximum flow from $I_{\le i} \cup I$
to $A_{h_1}\cup\cdots\cup A_{h_j}$.
Let $X$ be the decomposition of the last flow into resource disjoint paths.
For each $j$ we set $I'_{h_j}$ to the the sources of paths in $X$ ending in $A_{h_j}$.

Notice (this is not trivial):
The maximum flow in the residual graph from $I'_{\le j}\cup B_j$ to $A_j$ is at least $|A_j|$ for each
$j\le i$. Moreover, there is also such a flow and a corresponding decomposition into paths $Y$ such
that $Y$ does not intersect with the resources of paths of $X$ that end in $A_{h_{j'}}$ for any $h_{j'} < h_j$.

Because $|B_j|$ is growing exponentially (TODO) there must be a $j$ such
that $|I'_{h_j}| \ge |A_{h_j}| / 1000$.
We augment along these paths, set $I_{h_1} = I'_{h_1},\dotsc,I_{h_{j-1}} = I'_{h_{j-1}}$
and remove all layers $> h_j$.
It needs to be verified that the invariant on the flows still holds, i.e.,
the flow from $I_{\le i}\cup B_i$ to $A_i$ is of value at least $|A_i|$.

\paragraph*{Building a layer.}
If no layer can be collapsed, we build a new one.
Let $I$ denote the free resources not in $I_{\le \ell}$.
We will greedily construct a flow in the residual graph of $G(1)$ from $T(1) \setminus B_{\le \ell}$ to
$I \cup B_{\le \ell}$.
We start with $B = \emptyset$ and a maximal flow from $I$ to $B_{\le \ell}$. Then, for each player $i \in T(1) \setminus B_{\le \ell}$
we check if the maximum flow from $|I \cup B\cup i|$ to $|B_{\le \ell}|$ is greater than that from $|I \cup B|$.
Further, we perform the following test. We let every player in $T(1) \setminus B_{\le \ell}$ release
his resources in $R(2)$; we add $B\cup \{i\}$ to the blocking players; and we check if the algorithm manages
to reroute the resources to $B\cup \{i\}$ or if it gets stuck. If it succeeds, we add $i$ to $B$.

After finalizing $B$ we let $A$ be the sinks in the flow constructed.
If $w(A) \ge w(B_{\le \ell}) / 100$ we succeed and 
add $(1, A, B)$ to the layers.
If not, we fail.

\subsection{second layer}

\paragraph*{Invariants.}
For each layer $L_i$ with $d_i = 2$ there is a flow from $I_{\le i}\cup B_i$ to $A_i$ such that each player
in $A_i$ receives a flow of $1000 k / \alpha$.

\paragraph*{Collapsing a layer.}
Collapse 1:
Suppose for a layer $L_i$ with $d_i = 2$ we have that $|B_i|/100$ of the blocking players are double-covered.
Let $B'_i$ denote these players.
We compute a flow from $I_{\le i} \cup B_i$ to $A_i$ that sends a flow of $k / \alpha$ to each player in $A_i$.
We set $I'_i$ to be the sources (resources) in this flow that are in $I_i$ or assigned to a double-covered player in $B_i$.
We release the resources in $I_i$ from double-covered players. Then we remove from $B_i$ all double-covered players
and players that do not send flow.

Collapse 2:
Suppose for a layer $L_i$ with $d_i = 2$ we have that $|I_i| \ge |A_i| \cdot 100 k/\alpha$.
We construct like in the procedure of the first layer new sets $I'_1,I'_2,\dotsc,I'_i$
and get $|I'_j| \ge |A_j| \cdot 2 k/\alpha$ for some $j$. In particular, a constant fraction of $A_j$
receives a flow of $k / \alpha$ from $I'_j$. We augment along these paths and double-cover these addable players.

\paragraph*{Building a layer.}
Let $I$ denote the resources assigned to these double-covered players.
We greedily construct a flow in the residual graph of $G(2)$ from $I \cup T(2)\setminus B_{\le \ell}$
to $B_{\le \ell}$. We start with $A = \emptyset$ and a maximum flow from $I$ to $B_{\le \ell}$.
For each player $i\in B_{\le \ell}$ we check if there is a flow from $I \cup T(2) \setminus B_{\le \ell}$
to $A\cup\{i\}$ such that every player in $A\cup\{i\}$ receives a flow of $k/\alpha$.
If so, we add $i$ to $A$ and continue.

After finalizing $A$, we check if $w(A) \ge w(B_{\le \ell}) / 100$. If not, we fail.
If it holds, we add $(2, A, B)$ as a new layer where $B$ are the sources in the flow.

\newpage
\section{Flow LP and its dual}

\subsection{2 layers}
We consider the following flow linear program. Complex players are partitioned into two sets $C$ and $T$ (terminals). Each complex player $A\in C$ is associated with a variable $x_A\in [0,1]$ which describes how much this player is satisfied as a thin player. Complex players in $T$ already got their fat item stolen (i.e. $x_A=1$). Note that terminals might want more than $1$ item here in contrast with CCK09. Note that all complex players in the top layer are terminals. 

For the complex player $A_1$ e denote $\mathcal P(A_1)$ the set of all paths starting at a free resource or a private item of a complex player one layer below and ending at $A_1$.


For any path $p$ and complex player we have a variable $f_A(p)$. We denote by $s(p)$ the starting point of $p$ which is either a complex player or a free resource. 

We denote by $I_1$ the set of item on the top layer and $I_2$ the set of items at the bottom layer. We describe next the linear program:

\paragraph{Primal:} 

minimize $0^T \cdot (x,f)$ subject to:
 
\begin{tabular}{|c|c|c|}
  \hline
  set & constraint & dual variable \\
  \hline
  $\forall A\in T$ &  $\sum_{p\in \mathcal P(A)} f_A(p) = N_A$  & $d_A$\\
  $\forall A\in C$ &  $\sum_{p\in \mathcal P(A)} f_A(p) = N_A\cdot x_A$  & $d_A$ \\
  $\forall A\in C$, $\forall i\in I_2$ &  $\sum_{p\in \mathcal P(A):i\in p} f_A(p) \leq x_A$  & $c_{A,i}$ \\
  $\forall i\in I_1\cup I_2$ &  $\sum_{A\in T\cup C} \sum_{p\in \mathcal P(A):i\in p} f_A(p) \leq \beta(i)$  & $c_i$ \\
  $\forall A\in C$ &  $\sum_{A'\in T\cup C} \sum_{p \in \mathcal P(A'):A\in p} f_{A'}(p) = x_A$  & $o_A$ \\
  $\forall A,p$ &  $x_A, f_A(p)\geq 0$  & $\emptyset$ \\
  
  \hline 
\end{tabular}

\paragraph{Dual:} 

maximize $-\left(\sum_{A\in T}N_A d_A + \sum_{i\in I_1\cup I_2} \beta(i)c_i \right)$ 

\begin{tabular}{|c|c|c|}
  \hline
  set & constraint & primal variable\\
  \hline
  $\forall A\in C$ & $N_Ad_A + o_A + \sum_{i\in I_2} c_{A,i} \leq 0$ & $x_A$ \\
  $\forall A\in C$ and $p\in \mathcal P(A)$ & $d_A + \sum_{i\in p} (c_{A,i}+c_i)\geq 0$ & $f_A(p)$\\
  $\forall A\in T$ and $p\in \mathcal P(A)$ that starts at a free resource & $d_A + \sum_{i\in p} c_i\geq 0$ & $f_A(p)$\\
  $\forall A\in T$ and $p\in \mathcal P(A)$ that starts at a complex player $A'$ & $d_A+o_{A'}+\sum_{i\in p}c_i\geq 0$ & $f_A(p)$ \\
  $\forall A,i$ &  $c_{A,i}, c_i\geq 0$  & $\emptyset$\\
  
  \hline 
\end{tabular}

==> OverleafV1/reduction_proof.tex <==
\section{A simple reduction
\lars{(Needs adjustments)}}

In this section we want to give a proof similar to [??] showing that
if we have a polynomial time $\alpha$-approximation algorithm for
certain level instances of the
Santa Claus problem, then we can get also a polynomial time
$O(\alpha \cdot \mathrm{polylog}(n))$-approximation algorithm for the general problem.

\paragraph{Level instance.} The level instances are defined as follows.
There are $\ell = O(\log(n))$ levels $L_1,\dotsc,L_\ell$. Each level $L_j$ has a set of players $P(j)$
and resources $R(j)$.
The optimum is $1$ and for each level $j$ the resources $R(j)$ have
value $1$ or $0$ for players in $P(j)$ and value either $1 / d_i$ or $0$
for players $i\in P(j - 1)$. Here $d_i \gg \mathrm{polylog}(n)$ is a player specific
value, his \emph{demand}.
\bigskip

Furthermore, we reduce level instances to even more structured \emph{volume level instances}.
Such that a polynomial time $\alpha$-approximation algorithm for volume level instances
implies a polynomial time $O(\alpha \log^2(n))$-approximation algorithm for level instances.

\paragraph{Volume level instance.}
In addition to the structure of a level instance each player $i$ and each resource $j$ are given a volume
$w(i)$ and $w(j)$. If a resource $j$ has a value $1$ for a player in the same layer, the
volume of the player is the same as that of the resource.
If a resource $j'$ in the next layer has a non-zero value, i.e., a value of $1/d_i$, for player $i$
then $w(i) = d_i \cdot w(j')$.
\bigskip

By straight-forward constructions we reduce a general instance of Santa Claus
to one where each player has a demand $d_i \gg \mathrm{polylog}(n)$
and each resource has value $1$, $1/d_i$, or $0$ for him.
We call players \emph{fat} if they do not have resources of the second kind
and thin if they do. By adding some dummy items and dummy fat players we can
ensure that every thin player has exactly one resource that has value $1$ to
him and he is also the only thin player that has a value of $1$ for it.

We start with a solution that satisfies only the thin players by assigning
the unique resource, which he has value $1$ for, to him.
Intuitively, we want to augment the solution so as to decrease the number
of fat players, which are not covered, by a significant fraction, i.e.,
by $1 - 1/\mathrm{polylog(n)}$. This step is repeated until all fat players
are covered, which happens after $\mathrm{polylog(n)}$ iterations, if the decrease
is as above.
Let $\alpha$ be the approximation ratio of the algorithm for the level instance.
In the $k$'th iteration we want that every thin player either has his resource
of value $1$ or at least $d_i / (k\alpha)$ of the resources he values
with $1/d_i$.
With a polylogarithmic bound on the number of iterations, this yields an
approximation rate of $\alpha \cdot \mathrm{polylog}(n)$.

Consider the following construction for an improving step of iteration $k$.
We duplicate all resources $\ell$ times for some $\ell \in \mathbb N$.
Further, we create $\ell$ sets of player copies.
The first set contains all players that currently have no resource (must be fat) or
which currently have a resource of value $1$.
In all other sets we take only copies of players that currently have a value $1$ resource.
We denote the copies by $P(1), R(1), P(2), R(2),\dotsc, P(\ell - 1), R(\ell - 1), P(\ell), R(\ell)$.
Players $i\in P(j)$ get a value of $1$ for the resources in $R(j)$ that
in the original instance has a value of $1$ for him.
The resources in $R(j + 1)$ (for $j < \ell$) corresponding to those that have a value of $1/d_i$
in the original instance will get a value of $1/d_i$ in this construction.
All other combinations of resources and players will get a value of $0$.

Consider the assignment of resources to players copies as in the previous iteration.
This assignment will only leave some of the players in level $1$ uncovered. Every
other player copy will get one value $1$ resource.
A solution in the level instance can be viewed as an augmentation to the assignment above.
In other words, in the residual graph of $P(j) \cup R(j)$ it is a flow where the sources
are unassigned resources or players $i\in P(j)$ that receive $d_i$ resource of the next level and the sinks
are either players in $P(j - 1)$ or if $j = 1$ they are players not covered by the assignment above.
Furthermore, this flow can be viewed as a collection of resource disjoint paths.
We now argue that for $\ell > \log(n)$ the level instance has a solution of value $1/2$.
To this end, consider a feasible solution for the original instance
and derive a partial solution to the level instance as follows.

Assign the resources in each
copy the same as in the original instance assigning resources to the appropriate
player of the same level if the value is $1$ and the next level if it is $1/d_i$.
This will cover all players except for those in the last level which would have
received resources of the next level.
We will fix this now. For every player that is not covered (in the last level)
we let him steal his value $1$ item by reverting along the path that took it away
initially.
Now some of the players in level $\ell - 1$ might not be covered anymore.
For each player $i$ that receives no value $1$ resource and less than
$d_i / 2$ resources of the next level we let him steal back his resource from
the player in level $\ell - 2$. Notice that
because he has less than $d_i / 2$ resources, there must be at least $d_i / 2 \ge 2$
players in level $\ell$ of which the reverted paths ended in $i$.
We associate two of these players with $i$.
In the same way we continue in level $\ell - 2, \ell - 3, \dotsc, 1$.
Notice that the association between players that steal back their resource and
those that stole their resources forms a forest of full binary trees whose leafs
are in layer $\ell$.
We argue that in layer $1$ there is no player $i$ that is stolen more than
$d_i / 2$ of his resources. This is because otherwise the forest of associated
players would contain a full binary tree of height $\ell$, in particular,
there would be at least $2^\ell$ players in level $\ell$. This is a contradition
since $2^\ell > \log(n)$.

Now suppose we have an $\alpha/2$-approximate solution for the level instance,
i.e., each player $i$ receives either a value $1$ resource or $d_i / \alpha$
value $1/d_i$ resources.
We add together the flows corresponding to each level.
This means a fat player who was not covered in the previous iteration receives a flow of
$1$. A player $i$ who receives flow from the next level in some copy
sends at most a flow of $h$ through his value $1$ resource
and receives at least a flow of $d_i / \alpha$ over his value $1/d_i$ resources.
A player who does not receive flow from the next level at any copy
preserves the flow. Finally, a player $i$ that did not appear in the level
instance because he was covered with $d_i / ((k-1)\alpha)$ 
resources of value $1/d_i$ in the previous iteration
send out a flow of at most $h d_i / ((k - 1) \alpha)$;
an unassigned resource sends out a flow of at most $h$.
We divide this flow by $h \cdot k$ and make it integral.
For simplicity we ignore the error due to rounding for now (TODO fix later).
That way we can obtain a flow such that:
\begin{itemize}
    \item each player $i$ who had $d_i / ((k - 1) \alpha)$ resources in the previous
    iteration sends a flow of at most $d_i / (k (k - 1) \alpha)$, i.e., he retains at least
    \begin{equation*}
        \frac{d_i}{\alpha} \left(\frac{1}{(k - 1)} - \frac{1}{k(k - 1)} \right)
        = \frac{d_i}{k\alpha}
    \end{equation*}
    resources
    \item each player $i$ who had one value $1$ resource in the previous iteration
    now either still has one value $1$ resource or he has $d_i / (k\alpha)$
    value $1/d_i$ resources.
    \item of the players $i$ that were not covered in the previous iteration at
    least a fraction of $1/(k\alpha)$ receive a value $1$ resource.
\end{itemize}

==> deleted/ImprovedRounding.tex <==
\section{Computing a locally good solution for small $k$}
The goal of this section is to prove Lemma \ref{lem:lowk_localsol}. We recall that we are in a layered graph. The root $r$ (or the source) belong to layer $L_0$ and edges can only go inbetween vertices of consecutive layers. Denote by $\lambda$ a path from the root to some vertex $v$. $\lambda$ can thought of as a tuple of vertices $(r,v_1,\ldots, v_\ell)$ where $r$ is the root, $v_1$ a vertex in layer $L_1$ that is connected to $r$, and more generally $v_\ell$ is a vertex in layer $L_\ell$ that is connected to $v_{\ell-1}\in L_{\ell-1}$. Note that consecutive vertices in a tuple have to be connected by an edge in the graph. Finally we say that $\lambda$ is a \textit{closed} path if its last vertex is a sink.
\larstodo{Can we find a better term for these paths than sink? Maybe ``closed''?}

We will denote by $\lambda \circ v$ the path $\lambda$ in which we add the extra vertex $v$ at the end. A path $\lambda'$ is said to the a \textit{descendant} of $\lambda$ if it contains $\lambda$ as a prefix. We say that $\lambda$ is an \textit{ancestor} of $\lambda'$. We also say that $\lambda \circ v$ is a \textit{child} of $\lambda$ (who is then a \textit{parent} of $\lambda \circ v$).\larstodo{I prefer the term parent}

\lars{Based on the paths described above, we will now describe
a linear programming relaxation.
We have a variable $y(\lambda)$ for each $\lambda$ that in an integral solution takes value 1 if the path $\lambda$ is used entirely and 0 otherwise. With this in mind, it is easy to see that the following linear program is a relaxation of the problem.}

\begin{align}
    \sum_{\substack{\lambda':\\ \lambda'\textrm{ is child of } \lambda}} y(\lambda') &= k \cdot y(\lambda) &\textrm{for all } \lambda \textrm{ that is not closed} \label{eqLP:flowLPdemand}\\
     \sum_{\substack{\lambda': \lambda' \textrm{ ends in vertex }v,\\ \lambda'\textrm{ is descendant of } \lambda}} y(\lambda') &\leq y(\lambda) &\forall \lambda,v \label{eqLP:flowLPcapacity}\\
    y((r)) &= 1 & \label{eqLP:flowLPdemandroot}\\
    y &\ge 0 & 
\end{align}
If the graph has $h$ many layers, then this linear program has $n^{O(h)}$ variables and constraints and therefore can be solved in time $n^{O(h)}$. In order to prove Lemma \ref{lem:lowk_localsol}, we will design a rounding scheme. Before getting to the heart of the proof, we will first preprocess the fractional solution to ``sparsify'' the support.

\subsection{Preprocessing the LP solution}
A configuration at level 0 denoted $R$ as the singleton $\{r\}$. Then we define inductively a \textit{configuration} (denoted $C$) at level $\ell\geq 1$ as a set $S_C$ of $k/2$ vertices that belong to the layer $L_\ell$, and an ancestor tuple $(R(=C_0),C_1,\ldots ,C_{\ell-1})$ of configurations where $C_i$ is at level $i$. As a shorthand we will write $C=(S_C,(R,C_1,\ldots ,C_{\ell-1}))$. We say that $C_i$ is an \textit{ancestor} of $C$ and that $C$ is a \textit{descendant} of $C_i$. Furthermore $C_{\ell-1}$ is the \textit{father} of its \textit{child} $C$. We write $\mathrm{des}(C)$ for all descendants of $C$, $\mathrm{child}(C)$ for all children of $C$.

For all vertices $v$ at layer $L_\ell$ that appear in the definition of a configuration $C$ at level $\ell$, we will say that $v$ \textit{belongs} to $C$ (that we will often write $v\in C$). For some $C$ and $v$ we denote by $\mathrm{dist}(C, v)$ the number of layers between configuration $C$ and vertex $v$.

We have one variable $x_C$ per configuration $C$ (again with the intuition that $x_C=1$ if the integral solution uses this exact set of $k/2$ vertices as descendants of the ancestors of $C$). Our goal is to obtain a solution to the following linear program.
\larstodo{At the moment there seems to be a problem with the definition of configurations when selecting the same set twice.}
\begin{align}
    \sum_{\substack{C' \in \mathrm{des}(C): \\ v\in C'}} x_{C'} &\le 2 x_C &\forall C, v \label{eqLP:configLPcapacity}\\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &= \frac{k}{2} x_C &\forall C, \text{ where $C$ is not a terminal} \label{eqLP:configLPdemand}\\
    x_{C'} &= \frac{x_C}{\log n} &\forall C, C'\in \mathrm{child}(C) \label{eqLP:configLPsparsity}\\
    x_R &= 1 & \label{eqLP:configLPdemandroot}
\end{align}
It is easy to obtain such a solution from the fractional solution $y^*$ of the original LP. We proceed layer by layer (from top to bottom) as follows. We start with the trivial configuration $R$ at level 0 and set $x_R=1$. Then assume we sampled configurations until level $\ell$. For each configuration $C=(S_C,(R,C_1,\ldots ,C_{\ell-1}))$ at level $\ell$, we choose its children as follows. For each $v\in S_C$, we let $\lambda_v$ be the path ending at $v$ and going through all vertices $v_i\in C_i$ that sampled the configuration $C_{i+1}$. Each vertex $v\in S_C$ (that is not a sink) then samples $\log n$ sets of $k/2$ vertices in $L_{\ell+1}$ ensuring that each vertex $w\in L_{\ell+1}$ appears independently in each set with probability at most $y^*(\lambda_v \circ w)/(2y^*(\lambda_v))$.


We note that this is possible since constraint \eqref{eqLP:flowLPdemand} ensures that 
\begin{equation*}
   \sum_{w\in L_{\ell+1}} \frac{y^*(\lambda_v \circ w)}{2y^*(\lambda_v)} \geq \frac{k}{2}.
\end{equation*}

For each set $S'$ that was sampled in this manner, we add the configuration $C'=(S',(R,C_1,\ldots ,C_{\ell-1},C))$ as a children of the configuration $C$. We set $x_{C'}=x_C/\log n$. Since we sample exactly $\log n$ children of $C$, it is clear that constraints \eqref{eqLP:configLPdemand} and \eqref{eqLP:configLPsparsity} are automatically satisfied. We then turn our attention to constraint \eqref{eqLP:configLPcapacity}. Fix a configuration $C$ at some level $L_\ell$ and a vertex $v\in L_{\ell'}$ with $\ell'\ge \ell$. Assume we selected configurations up to level $i\le \ell'$. For each vertex $w\in L_i$ that belongs to $S_{C'}$ for $C'$ a descendant of $C$ we consider the path $\lambda_w$ that goes through the ancestor configurations of $C'$ from the root to $w$. When selecting configurations at level $i+1$, each of these vertices $w$ will select $\log n$ sets of $k/2$ vertices at level $L_{i+1}$ where each vertex $x\in L_{i+1}$ belongs to each set with probability $y^*(\lambda_w\circ x)/(2y^*(\lambda_w))$. 

In the following, we define
\begin{equation*}
    X_j(C',w, x)
\end{equation*}
to be the random variable that is 1 if the vertex $x$ is selected by the vertex $w$ in its $j$th set ($j\in [1,\log n]$) to be part of a child configuration of $C'$. If it is not then $X_j(C',w, x)=0$.

We define for a path $\lambda$ its \textit{expected load} on vertex $v$ as the quantity
\begin{equation*}
    L(\lambda,v)=   \left[\sum_{\substack{\lambda': \lambda' \textrm{ ends at vertex }v,\\ \lambda'\textrm{ is a descendant of } \lambda}} y(\lambda')\right]/y(\lambda).
\end{equation*}

Recall that by constraint \eqref{eqLP:flowLPcapacity}, we have that $L(\lambda,v)\leq 1$. Using these definitions, we will keep track of the fractional load induced on $v$ by descendants of $C$ at level $i$ denoted by 

\begin{equation*}
    Y^{(i)}(C,v) := \sum_{C' \in \mathrm{des}(C)\cap L_i} x_{C'}\cdot L(\lambda (C'),v)
\end{equation*}

Note that in the end we want to bound the quantity 
\begin{equation*}
    \sum_{\substack{C' \in \mathrm{des}(C): \\ v\in C'}} x_{C'}
\end{equation*}
which is precisely equal to $Y^{(\ell')}(C,v)$ (where $v\in L_{\ell'}$). We will prove the following lemma. Moreover, note that if $C$ is at level $\ell$, then
\begin{equation*}
    Y^{(\ell)}(C,v)\leq x_C.
\end{equation*}
\begin{lemma}
\begin{equation*}
    probability blabla
\end{equation*}
\end{lemma}
\begin{proof}
We note that 
\begin{equation*}
    Y^{(i+1)}(C,v) := \sum_{C' \in \mathrm{des}(C)\cap L_{i+1}} \left[x_{C'}\cdot \sum_{x\in S_{C'}} \sum_{x\in S_C} L(\lambda (C') \circ x,v)  \right]
\end{equation*}
\end{proof}











\newpage
The root $r$ chooses $\log n$ sets of $k/2$ children each in layer 1 where each vertex $v$ belongs to each set independently with probability $y^*((r,v))/2$. Each of these sets will give a configuration $C$ at level 1. And we will set $x_C=1/\log n$. 

Then each configuration $C$ that was selected samples its children as follows. For each $v\in C$, if $v$ is a sink do nothing, else select $\log n$ set of $k/2$ vertices each (vertices at layer 2) where each vertex $w$ in $L_2$ is selected in each set with probability $y^*((r,v,w))/(2y(r,v))$. Each set selected will give the configuration $C'$ associated to the set of vertices and the ancestors tuple $(R,C)$. We set $x_{C'}=x_C/\log n=1/\log^2 n$ for those configurations and $x_{C'}=0$ for the other configurations of the same level. Note that is it possible that we select 2 identical configurations in which case we will implicitly treat them as distinct objects.

We continue iteratively until the last layer. Each configuration $C$ at level $\ell$ that was selected selects $\log n$ set of $k/2$ vertices each (vertices at layer $\ell+1$). If $\lambda$ is the path that leads until configuration $C$ then each vertex $w\in L_{\ell+1}$ is selected in each set with probability



And for all configurations t
\subsection{Computing locally consistent solution}

Perform sparsification as described above.
Let $L_1,\dotsc,L_h$ be the configurations is layers $1,\dotsc,h$.
We write $\mathrm{des}(C)$ for all descendants of $C$, $\mathrm{child}(C)$ for all children.
We assume that in layer $1$ there is a ``pseudo-configuration'' $R$ corresponding to the root.
For some $C$ and $v$ we denote by $\mathrm{dist}(C, v)$ the number of layers between configuration $C$ and vertex $v$.
With high probability, we get a solution for the following system.
\etienne{TODO put ref to each line}
\begin{align}
    \sum_{\substack{C' \in \mathrm{des}(C): \\ v\in C'}} x_{C'} &\le 2 x_C &\forall C, v \\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &\ge \frac{k}{2} x_C &\forall C, \text{ where $C$ is not a terminal} \\
    x_{C'} &= \frac{x_C}{\log n} &\forall C, C'\in \mathrm{child}(C) \\
    x_R &= 1 &
\end{align}
We want to round now layer by layer, maintaining
the following set of constraints after iteration $\ell$.
\begin{align}
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 10^3 \cdot \log k \cdot \log^3\log n \cdot x_C &\forall C\in L_{1}\cup\cdots\cup L_{\ell} \text{ and } v \text{ with } \mathrm{dist}(C, v) \le \log\log n \label{eqLP:capacitycloserange}\\
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 10^3\cdot \log^3 n \cdot x_C &\forall C\in L_{1}\cup\cdots\cup L_{\ell} \text{ and } v \text{ with } \mathrm{dist}(C, v) > \log\log n \label{eqLP:capacitylongrange}\\
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 2 x_C &\forall C\in L_{\ell+1}\cup\cdots\cup L_h, v \label{eqLP:capacityfractional}\\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &= \frac{k}{24} \cdot x_C &\forall C, \text{ where $C\in L_{1}\cup\cdots\cup L_{\ell}$ is not a terminal} \label{eqLP:demandintegral}\\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &= \frac{k}{2} x_C &\forall C, \text{ where $C\in L_{\ell+1}\cup\cdots\cup L_h$ is not a terminal} \label{eqLP:demandfractional} \\
    x_{C'} &\in \left\lbrace 0,\frac{x_C}{\log n} \right\rbrace&\forall C, C'\in \mathrm{child}(C), C'\in L_{\ell+1}\cup\cdots\cup L_h \label{eqLP:fractionality}\\
    x_{C} &\in \{0, 1\} &\forall C\in L_1\cup \cdots \cup L_\ell \label{eqLP:integrality}\\
    x_R &= 1 &
\end{align}
\larstodo{There is some error in (16). A configuration cannot be a terminal right?}
We perform the following rounding to round $L_{\ell+1}$:
for each $C\in L_{\ell}$, pick a set of $k/24$ configurations $C'\in \mathrm{child}(C)$ uniformly among all such sets. Since we have that $x_{C'}=1/\log (n)$ for all $C'\in \mathrm{child}(C)$ and that 
\begin{equation*}
    \sum_{C'\in \mathrm{child}(C)}x_{C'}\ge \frac{k}{2},
\end{equation*}
it implies that any such configuration $C'$ is selected with probability exactly $x_{C'} / 12$.
For any $C'\in \mathrm{child}(C)$ that was selected we scale up the descendants of $C'$ by $1/x_{C'}=\log n$. For all $C'$ that was not selected, we set $x_{C''}$ to 0 for all descendants $C''$ of $C'$ (i.e. we delete the configuration $C'$ along with all its descendants).

We will show with LLL that with positive probability the constraints remain valid.

For all configurations $C\in L_{\ge \ell+1}$, we call the new rounded variables $x'_C$. Note that this is a random variable that takes value either 0 or $x_C \cdot \log n$ with probability $1/(12 \log n)$.


Consider the constraint for $C, v$. If $C$ is below layer $L_{\ell+1}$,
it must remain valid. Otherwise, $x_C$ was rounded to $1$ before and
\larstodo{I would remove the braces here (and in the next equations).}
\begin{equation*}
    \mathbb E[ \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x'_{C'} ] = \frac{1}{12}\cdot \left( \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} \right)
\end{equation*}
By the capacity constraints satisfied before rounding, we have that
\begin{equation*}
    \frac{1}{12}\cdot \left( \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} \right) \le 10^2 \cdot \log k \cdot \log^3\log n,
\end{equation*}
\larstodo{$10^3$ instead?}
if $\textrm{dist}(C,v)\le \log \log n$ and 
\begin{equation*}
    \frac{1}{12}\cdot \left( \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} \right) \le 10^2 \cdot \log^3n
\end{equation*} otherwise.
Hence in order to violate the capacity constraint after rounding one more layer, this expectation has to be exceeded by at least
\begin{equation*}
    500 \cdot \log k \cdot \log^3\log n \quad \text{or} \quad 500 \cdot \log^3 n ,
\end{equation*}
depending on the distance between $C$ and $v$.

\etienne{TODO write some intuition for LLLL}

For fixed $C, v$ and $C' \in \mathrm{desc}(C) \cap L_{\ell+1}$ we denote by $S_{C',v}$ the random variable equal to
\begin{equation*}
    S_{C',v}:=\sum_{\substack{C'' \in \mathrm{des}(C'):\\ v\in C''}} x'_{C''}.
\end{equation*}
Intuitively, the value $S_{C',v}$ corresponds to the expected congestion that the descendants of $C'$ will put on $v$ if we were not scaling down the probabilities after rounding $x_{C'}$.

Note that $S_{C',v}$ can take value either 0 or 
\begin{equation*}
    \log(n) \cdot \left( \sum_{\substack{C'' \in \mathrm{des}(C'):\\ v\in C''}} x_{C''}\right).
\end{equation*}
The latter case happens with probability $1/(\log n \log\log n)$.\larstodo{Why this probability?}



Then we split those random variables $S_{C',v}$ depending on how big a value they can take. More precisely, let $G_{C,v,t}$
be the set of all random variables $S_{C',v}$ that take value either 0 or a positive real number in the interval $[2^{-(t+1)},2^{-t})$.

Note that any variable $x'_{C'}$ with $C'\in L_{\ell+1}$ belongs to the first layer that is not rounded yet. Hence we have that $x_{C'}\in \{0,\frac{1}{\log(n)}\}$. Also the capacity constraint 
\begin{equation*}
    \sum_{\substack{C'' \in \mathrm{des}(C'):\\ v\in C''}} x_{C''} \le 2 x_{C'}
\end{equation*}
is satisfied. This implies that 
\begin{equation*}
   \log(n) \cdot \left( \sum_{\substack{C'' \in \mathrm{des}(C'):\\ v\in C''}} x_{C''}\right) \le \log(n)\cdot (2x_{C'}) \leq 2 
\end{equation*} for all $C'\in \mathrm{desc}(C) \cap L_\ell$. Moreover, we have that
\begin{equation*}
    x_{C''}\in \left\lbrace 0,\frac{1}{\log(n)^{\textrm{dist}(C',C'')+1}}\right\rbrace.
\end{equation*} for all $C''$ that is a descendant of $C'$.
Hence the partitioning or random variables $S_{C',v}$ is only relevant for 
\begin{equation*}
    t\in [-1,\textrm{dist}(C',C'')\cdot \log\log(n)].
\end{equation*}

Next, we define as a bad event $B_{C,v,t}$ that
\begin{equation}
\label{eq:badeventdef}
     \sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}>
     \begin{cases}
        3\mathbb E[\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}] + 250 \cdot \log k \cdot \log\log n &\text{ if } \mathrm{dist}(C, v) \le \log\log n \\
        3 \mathbb E[\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}] + 250\cdot \log n &\text{ if } \mathrm{dist}(C, v) > \log\log n \\
     \end{cases}
\end{equation}
We finish this part by a simple proof to upper bound the probability of a bad event happening.
\begin{lemma}
\label{lem:bad_event_proba}
For any $C,v,t$, we have that 
\begin{equation*}
    \mathbb P [B_{C,v,t}]\leq k^{-2^{t+7} \log \log n}
\end{equation*} if $B_{C,v,t}$ is of type 1. If $B_{C,v,t}$ is of type 2 then
\begin{equation*}
    \mathbb P [B_{C,v,t}]\leq n^{-2^{t+7}}.
\end{equation*}
\end{lemma}
\begin{proof}
We consider the first case. Let $B_{C,v,t}$ be a bad event of the first type. The variables $S_{C',v}\in G_{C,v,t}$ are not independent but satisfy the \textit{negative regression} condition of \cite{negativedependence} (see Definition 21). To see this, notice that two random variables $S_{C',v}, S_{C'',v}\in G_{C,v,t}$ are either such that the configurations $C',C''$ do not have the same father, in which case they are independent. On the contrary, if $C',C''$ have the same father then conditioning by $x_{C'}=1$ cannot decrease the property that $x_{C''}$ is equal to 1. By Proposition 29 in \cite{negativedependence}, the standard Chernoff-Hoeffding bounds apply to the sum of random variables in negative regression.
By Chernoff-Hoeffding (see Theorem \ref{chernoff} in appendix), we have that 
\begin{equation*}
    \mathbb P [B_{C,v,t}] \leq \exp\left(-125 \log k \log \log n \cdot 2^{t}\right) \leq k^{-2^{t+7}\log \log n}.
\end{equation*}
Similarly, if $B_{C,v,t}$ is a bad event of the second type, we can apply standard Chernoff-Hoeffding bounds and obtain 
\begin{equation*}
    \mathbb P [B_{C,v,t}] \leq \exp\left(-125 \log n \cdot 2^{t}\right) \leq n^{-2^{t+7}}.
\end{equation*}
\end{proof}

\subsection{Applying the Lov\'asz Local Lemma}
For a bad event $B_{C,v,t}$, we denote by $\mathcal N^{(1,t')}(B_{C,v,t}),\mathcal N^{(2,t')}(B_{C,v,t})$ the set of bad events $B_{C,v,t'}$ of first type (or second type respectively) that depend on $B_{C,v,t}$. For any bad event $B_{C,v,t}$ we denote by $\mathcal N (B_{C,v,t})$ the set of all bad events it depends on. Let us now bound the dependencies with the following lemmas. 
\begin{lemma}
\label{lem:variable_dependency}
For any $C\in L_{\ell+1}$, the corresponding random variable $x'_{C}$ influences at most $(k/2)\log(n)$ other random variables $x'_{C'}$ with $C'\in L_{\ell+1}$.
\end{lemma}
\begin{proof}
Clearly, if the configurations $C$ and $C'$ do not have the same father then the corresponding random variables are independent. If they share a common father $C"$, note that $x_{C"}=1$ and that $x_C=x_{C'}=1/\log n$. By the constraint \eqref{eqLP:demandfractional}, we know that $C''$ can have only $(k/2)\log n$ relevant children, which concludes the proof.
\end{proof}
\begin{lemma}
\label{lem:variable_influence}
For any $C\in L_{\ell+1}$ and any $t\geq 0$, the corresponding random variable $x'_{C}$ influences at most 
\begin{equation*}
    (2^{t+1} (k/2)^{\log\log n})\cdot  \log\log(n)
\end{equation*} bad events $B_{C,v,t}$ of the first type, and at most $n\log n$ bad events of the second type.
\end{lemma}
\begin{proof}
    We first count the number of vertices $v$ at distance $d$ from $C$ such that a descendant $C'$ of $C$ contains $v$ and $x_{C'}\neq 0$, i.e. we consider all the vertices $v$ such that some descendant of $C$ is expected to put a strictly positive congestion on $v$. It is clear that $x'_C$ can only influence bad events $B_{C,v,t}$ for such vertices. Note that, by constraint \eqref{eqLP:demandfractional}, the total demand of $C$ is equal to $k/2$ vertices on the layer $L_{\ell+2}$, $(k/2)^2$ vertices on layer $L_{\ell+3}$ and so on. Hence at distance $d$, the total volume of vertices taken by descendants of $C$ is equal to $(k/2)^d$.
    
    Hence if $x'_C$ influences a bad event $B_{C,v,t}$, it must be that the total fractional demand of the descendants of $C$ on vertex $v$ is at least $2^{-(t+1)}$. Since the total demand on all vertices is upper bounded by $(k/2)^{\textrm{dist}(C,v)}$, there can be only $2^{t+1}\cdot (k/2)^{\textrm{dist}(C,v)}$ such events for a fixed $t$ and $\textrm{dist}(C,v)$. If we consider only bad events on the first type, then $\textrm{dist}(C,v)$ can be at most $\log \log n$ hence $x'_C$ can influence in total at most 
    \begin{equation*}
        (2^{t+1} (k/2)^{\log\log n})\cdot  \log\log(n)
    \end{equation*} such events for a fixed $t$. The bound on bad event of the second type is easier to obtain. There are at most $n$ choices of vertices and $\log n$ choices of an ancestor $C'$ of $C$ such that $x'_C$ can influence $B_{C',v,t}$.
\end{proof}

\begin{lemma}
\label{lem:bad_event_influence}
Any bad event $B_{C,v,t}$ of the first type depends on at most \begin{equation*}
    2^{t+11} \log k \cdot \log^3\log n
\end{equation*} random variables $x'_{C'}$ with $C'\in L_{\ell+1}$.
Any bad event $B_{C,v,t}$ of the second type depends on at most \begin{equation*}
    2^{t+11}  \log^3 n
\end{equation*} random variables $x'_{C'}$ with $C'\in L_{\ell+1}$.
\end{lemma}
\begin{proof}
We consider the first case. By constraint \eqref{eqLP:capacitycloserange}, we have that 
\begin{equation*}
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} \le 10^3 \cdot \log k \cdot \log^3\log n 
\end{equation*} since $x_C$ was rounded to 1 previously. This implies that there can only be at most $2^{t+1}\cdot (10^3 \cdot \log k \cdot \log^3\log n )$ descendants $ C'\in L_{\ell + 1}$ of $C$ that induce a fractional load of at least $2^{-(t+1)}$. This concludes the first case. The same argument with constraint \eqref{eqLP:capacitylongrange} proves the second case.
\end{proof}

The previous three lemmas allow us to upper bound easily the size of the neighborhoods $\mathcal N^{(1,t')}(B_{C,v,t}),\mathcal N^{(2,t')}(B_{C,v,t})$.

\begin{lemma}
\label{lem:neighborhood}
For any bad event $B_{C,v,t}$ (either of the first or second type) and for $n,k$ bigger than some big enough constant, we have that 
\begin{align*}
    \left|\mathcal N^{(1,t')}(B_{C,v,t})\right| \le & 2^{t+t'}\cdot (k/2)^{5\log\log n}\quad \forall t' \in [-1,\log^2 \log n], \textrm{ and}\\
    \left|\mathcal N^{(2,t')}(B_{C,v,t})\right| \le & 2^t\cdot n^3\quad \forall t'\in [-1,\log (n) \log \log (n)].
\end{align*}
\end{lemma}
\begin{proof}
A bad event $B_{C,v,t}$ of the first type can depend on at most 
\begin{equation*}
    2^{t+11} \log k \cdot \log^3\log n
\end{equation*} random variables by Lemma \ref{lem:bad_event_influence}. By Lemma \ref{lem:variable_dependency}, each of these variables can influence at most $(k/2)\log n$ other variables. Finally, by Lemma \ref{lem:variable_influence} each of these variables can influence at most 
\begin{equation*}
    (2^{t'+1} (k/2)^{\log\log n})\cdot  \log\log(n)
\end{equation*} bad events $B_{C,v,t'}$ of the first type. Hence we can compute that 
\begin{align*}
     \left|\mathcal N^{(1,t')}(B_{C,v,t})\right| &\le (2^{t+11} \log k \cdot \log^3\log n)\cdot  ((k/2)\log n)\cdot  (2^{t'+1} (k/2)^{\log\log n})\cdot  \log\log(n))\\
     &\le 2^{t+t'}(k/2)^{4\log \log n}
\end{align*} (for $n,k$ big enough). The same arguments show that 
\begin{align*}
     \left|\mathcal N^{(2,t')}(B_{C,v,t})\right| &\leq (2^{t+11} \log k \cdot \log^3\log n)\cdot  ((k/2)\log n)\cdot (n\log n) \\
     &\le 2^{t}\cdot n^3
\end{align*} (for $n,k$ big enough). Similarly, if $B_{C,v,t}$ is a bad even of the second type, then
\begin{align*}
    \left|\mathcal N^{(1,t')}(B_{C,v,t})\right| &\le (2^{t+11}  \log^3 n)\cdot ((k/2)\log n) \cdot (2^{t'+1} (k/2)^{\log\log n})\cdot  \log\log(n)) \\
    &\le 2^{t+t'}\cdot (k/2)^{5\log \log n}
\end{align*} (for $n,k$ big enough). Finally, we obtain
\begin{align*}
    \left|\mathcal N^{(1,t')}(B_{C,v,t})\right| &\le (2^{t+11}  \log^3 n)\cdot ((k/2)\log n) \cdot (n\log n) \\
    &\le 2^{t}\cdot n^3
\end{align*} (for $n,k$ big enough).
\end{proof}

With Lemmas \ref{lem:bad_event_proba} and \ref{lem:neighborhood}, we are ready to apply the non-uniform LLL. We will set 
\begin{equation*}
    x(B_{C,v,t})=(\mathbb P(B_{C,v,t}))^{1/2}
\end{equation*} for all bad events. If $B_{C,v,t}$ is a bad event of the first type, we obtain that 
\begin{align*}
    \prod_{t'=-1}^{\log^2 \log n} \prod_{B_{C,v,t}\in N^{(1,t')}(B'_{C,v,t})} (1-x(B'_{C,v,t})) &\ge  \prod_{t'=-1}^{\infty} (1-k^{-2^{t'+6}\log \log n})^ {\left|\mathcal N^{(1,t')}(B_{C,v,t})\right|}\\
    &\ge \prod_{t'=-1}^{\infty}(1-k^{-2^{t'+6}\log \log n})^ {2^{t+t'}\cdot (k/2)^{5\log \log n}}\\
    &\ge \prod_{t'=-1}^{\infty}\exp\left( -k^{-2^{t'+5}\log \log n}\cdot  2^{t+t'}\cdot (k/2)^{5\log \log n}\right)\\
    &\ge \prod_{t'=-1}^{\infty}\exp\left( -k^{-2^{t'+2}\log \log n}\cdot  2^{t+t'}\right)\\
    &\ge  \prod_{t'=-1}^{\infty}\exp\left( -(k^{-2^2-\log \log n})^{2^{t'}}\cdot  2^{t'}\cdot 2^{t}\right)\\
    &\ge  \prod_{t'=-1}^{\infty}\exp\left( -(k^{-\log \log n})^{2^{t'}}\cdot 2^{t}\right)\\
    &\ge  \prod_{t'=-1}^{\infty}\exp\left( -2^{-t'}\cdot 2^{t}\right) = \exp\left(-2^t\sum_{t'=-1}^{\log^2\log n} 2^{-t'} \right) \ge \exp\left(-2^{t+2} \right).
\end{align*}

We obtain in the same way that
\begin{align*}
    \prod_{t'=-1}^{\log(n)\log \log (n)} \prod_{B_{C,v,t}\in N^{(2,t')}(B'_{C,v,t})} (1-x(B'_{C,v,t})) &\ge  \prod_{t'=-1}^{\infty}(1-n^{-2^{t'+6}})^ {2^t\cdot n^3}\\
    &\ge \prod_{t'=-1}^{\infty} \exp \left(-n^{-2^{t'+5}}\cdot 2^t \cdot n^3 \right)\\
    &\ge \prod_{t'=-1}^{\infty} \exp \left(-n^{-2^{t'+3}}\cdot 2^t \right)\\
    &\ge \prod_{t'=-1}^{\infty} \exp \left(-n^{-(t'+3)}\cdot 2^t \right)\\
    &\ge \exp\left(-2^t \sum_{t'=2}^{\infty}n^{-t'}\right)\ge \exp\left(-2^{t+1} \right).
\end{align*}

Hence we can verify the condition to apply LLL as follows:
\begin{align*}
     x(B_{C,v,t})\prod_{B'_{C,v,t}} (1-  x(B'_{C,v,t}))&\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot \exp\left(-(2^{t+2}+2^{t+1}) \right)\\
     &\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot \exp\left(-2^{t+3} \right)\\
     &\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot k^{-2^{t+3}\log \log n}\\
     &\ge \mathbb P(B_{C,v,t}).
\end{align*}
If $B_{C,v,t}$ is a bad event of the second type, we conclude similarly
\begin{align*}
     x(B_{C,v,t})\prod_{B'_{C,v,t}} (1-  x(B'_{C,v,t}))&\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot \exp\left(-(2^{t+2}+2^{t+1}) \right)\\
     &\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot \exp\left(-2^{t+3} \right)\\
     &\ge (\mathbb P(B_{C,v,t}))^{1/2} \cdot n^{-2^{t+3}}\\
     &\ge \mathbb P(B_{C,v,t}).
\end{align*}

We can therefore apply the constructive version of the Lov\'asz Local Lemma by Moser and Tardos \cite{moser2010constructive} to obtain in polynomial time a set of $k/24$ children configurations such that no bad event happens for each $C\in L_\ell$ (such that $x_C=1$).

\subsection{Wrapping Up}
We showed that by applying LLL, we can round one more layer of configuration such that no bad events happen. By the definition of a bad event in Equation \eqref{eq:badeventdef}, this means that 
\begin{equation}
     \sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}\leq 
     \begin{cases}
        3\mathbb E[\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}] + 250 \cdot \log k \cdot \log\log n &\text{ if } \mathrm{dist}(C, v) \le \log\log n \\
        3 \mathbb E[\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}] + 250\cdot \log n &\text{ if } \mathrm{dist}(C, v) > \log\log n \\
     \end{cases}
\end{equation} for all $C,v,t$. We can now verify that the constraints \eqref{eqLP:capacitycloserange} and \eqref{eqLP:capacitylongrange} are maintained after rounding one more layer. Indeed for $C,v$ such that $\textrm{dist}(C,v)\leq \log \log n$ we have that 
\begin{align*}
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x'_{C'} &= \sum_{t=-1}^{\log^2 \log n} \sum_{S_{C',v}\in G_{C,v,t}} S_{C',v} \\
    &\le \sum_{t=-1}^{\log^2 \log n}3\mathbb E[\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}] + 250 \cdot \log k \cdot \log\log n\\
    &= 3\mathbb E[\sum_{t=-1}^{\log^2 \log n}\sum_{S_{C',v}\in G_{C,v,t}} S_{C',v}]+250 \cdot \log k \cdot \log^3 \log n\\
    &= \frac{3}{12}\sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'}+250 \cdot \log k \cdot \log^3 \log n\\
    &\le \frac{3}{12}\cdot  10^3 \cdot \log k \cdot \log^3 \log n+250 \cdot \log k \cdot \log^3 \log n \\
    &\le 10^3\log k \cdot \log^3 \log n.
\end{align*}
The constraint \eqref{eqLP:capacitylongrange} is verified with the same argument. Hence after rounding all the layers from top to bottom, we obtain the following integral system.
\begin{align}
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 10^3 \cdot \log k \cdot \log^3\log n \cdot x_C &\forall C \text{ and } v \text{ with } \mathrm{dist}(C, v) \le \log\log n \label{eqLPintegral:capacitycloserange}\\
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 10^3\cdot \log^3 n \cdot x_C &\forall C \text{ and } v \text{ with } \mathrm{dist}(C, v) > \log\log n \label{eqLPintegral:capacitylongrange}\\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &= \frac{k}{24} \cdot x_C &\forall C, \text{ where $C$ is not a terminal} \label{eqLPintegral:demandintegral}\\
    x_{C} &\in \{0, 1\} &\forall C \label{eqLPintegral:integrality}\\
    x_R &= 1 &
\end{align}
From these integral configuration variables it is straightforward to build a pseudo flow where each vertex obtains $k/24$ children, the maximum congestion is no more than $10^3\cdot \log n$ and every subflow of depth $\log \log n$ has congestion no more than $10^3\cdot  \log k \cdot  \log \log n$. This ends the proof of Theorem \ref{thm:}.

\newpage

==> deleted/LocallyGood.tex <==
\section{Computing a locally good solution}
The goal of this section is to prove Lemma~\ref{lem:locallygood}. We recall that we are in a layered graph with vertices partitioned into layers $L_0, L_1,\dotsc, L_{h}$ where $h = \log n$. The sources $S$ belong to layer $L_0$ and edges can only go from vertices in some layer $L_i$ to
the next layer $L_{i+1}$. 

In the following we will extensively argue about
paths that start in one of the sources. For the
remainder of the section every path $p$ that
we consider is implicitly assumed to start at one of the sources and then traverse (a prefix of)
the layers one by one.
Slightly abusing notation, we sometimes
use $L_i$ also to denote the set of paths
ending in a vertex of $L_i$, that is,
\begin{equation*}
    \bigcup_{v\in L_i} I(v) \ ,
\end{equation*} 
and $T$ to describe the set of closed paths (recall that those are the paths that end at a sink). Let $P$ refer to the set of all possible paths and notice that by virtue of the layers
we have that $|P| \le n^{h} \le n^{\log n}$.
We will now describe
a linear programming relaxation, which goes back to
Bateni et al.~\cite{bateni2009maxmin}. The intuition behind the linear program is to select paths similarly to the way we describe solutions,
see Section~\ref{sec:prelim}.
We have a variable $x(p)$ for each path $p$ that in an integral solution takes value $1$ if the path $p$ is contained in an arborescence and $0$ otherwise.
\begin{align}
    \sum_{q\in C(p)} x(q) &= k \cdot x(p) &\forall p\in P\setminus T \label{eqLP:flowLPdemand}\\
     \sum_{q\in I(v)\cap D(p)} x(q) &\leq x(p) &\forall p\in P,v\in V \label{eqLP:flowLPcapacity}\\
    x((s)) &= 1 &\forall s\in S \label{eqLP:flowLPdemandroot}\\
    x &\ge 0 & 
\end{align}

Constraint~\eqref{eqLP:flowLPcapacity} deserves
further elaboration: it would be natural to state only the simpler constraint $\sum_{q\in I(v)} x(q) \le 1$ for all $v$, which describes that $v$ has congestion at most one. Instead,~\eqref{eqLP:flowLPcapacity} is a strengthening of this constraint. Without it, there
could be situations, where for example we take a path $p$ with only value $1/k$ and then a single child of $q$ with value $1$. Such situations easily lead to large integrality gaps, which we can avoid by this strengthening.

Since the graph has $h+1$ many layers, this linear program has $n^{O(h)}$ variables and constraints and therefore can be solved in time $n^{O(h)}$. We refer to this relaxation as the \textit{path LP}. In order to prove Lemma \ref{lem:locallygood}, we will design a rounding scheme. Before getting to the main part of the proof, we will first preprocess the fractional solution to sparsify its support.

\subsection{Preprocessing the LP solution}
The goal of this part is to sparsify the path LP solution $x$ to get another sparser solution $y$ (i.e., with a limited number of non-zero entries). For ease of notation, we might need to take several times a copy of the same path $p\in P$. We emphasise here that two copies of the same path are different objects. To make this clear, we will now have a \textbf{multiset} $P'$ of paths but we will slightly change the parent/child relationship between paths. Precisely, for any path $q'\in P'$ is assigned as child to a \textbf{unique} copy $p'\in P'$ such that $q$ was a child of $p$ in the set $P$. With this slight twist, all the ancestors/descendants relationships extend to multisets in the natural way. For instance, we will denote by $D_{P'}(p)$ the set of descendants of $p$ in the multiset $P'$. Again, the set of closed path in $P'$ will be denoted by $T'$ and $S'$ refers to the sources. We assume that there is a unique copy of the trivial path $(s)\in P'$ for any source $s\in S$.

The preprocessing of the LP will allow us to obtain a multiset of path $P'$ as above and a fractional solution $y$ such that 
\begin{align}
    \sum_{q\in C_{P'}(p)} y(q) &= \frac{k}{4} \cdot y(p) &\forall p\in P'\setminus T'\label{eqSparseLP:demand}\\
     \sum_{ q\in I_{P'}(v)\cap D_{P'}( p)} y( q) &\leq 2y( p) &\forall p\in P',v \in V\label{eqSparseLP:capacity}\\
     y(p) &=  \frac{1}{(4\log^2 (n))^i}  & \forall i\leq h, \forall  p\in L_i\label{eqSparseLP:granularity}\\
     y((s))&=1 &\forall s\in S \label{eqSparseLP:root}
\end{align}
We obtain such a solution $y$ in a similar way as the randomized rounding in~\cite{bateni2009maxmin, chakrabarty2009allocating}, which achieves polylogarithmic congestion. Instead of polylogarithmic congestion we obtain constant congestion at the cost of getting variables that are not integers, but fractional variables with a certain granularity. For completeness we give
the proof in Appendix~\ref{sec:Sparsify}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sampling a locally nearly good solution}
We start this part with the sparse solution $y$ and the multiset of paths $P'$ that we computed above. We will proceed to round this fractional solution to an integral solution that is \textit{locally nearly good}. We define here a few concepts before moving to the definition of locally nearly good solutions. $D_{Q}(p, \ell')$ will denote the set of descendants of $p$ at distance $\ell'$ of $p$ in multiset $Q$. $\textrm{cong}_{Q}(p)$ is the total congestion induced by $Q$ on the endpoint of $p$. $\textrm{cong}_{Q,p}(q)$ will denote the \textit{local congestion} induced on the endpoint of $q$ by all descendants of $p$ in the solution $Q$. Finally, we set $\ell=10 \log \log (n)$ in the rest of the section.


A locally nearly good solution is a multiset of paths $Q$ (where again every path has a \textbf{unique} parent among the relevant copies of the same path) that has the following properties:
\begin{enumerate}
    \item One copy of the trivial path $(s)$ belongs to $Q$ for all sources $s\in S$;
    \item Every open path has $k/200$ children;
    \item No vertex has global congestion more than $1500 \log^3(n)$;
    \item For every path $p\in Q$ and $\ell' \le \ell$ we have that
    \begin{equation*}
        \left| \{q\in D_{Q}(p, \ell') \mid \textrm{cong}_{Q,p}(q)\ge 10^3(\log \log (n))^2 \}\right|\le \frac{|D_Q(p, \ell')|}{\log^{10} (n)} \ .
    \end{equation*}
\end{enumerate}

We elaborate here on those conditions. The first two conditions are fairly intuitive. The third condition states that the maximum global congestion is at most poly-logarithmic. The fourth condition states that any selected path has few close descendants that have a high local congestion. The goal is to obtain this locally nearly good solution, then for every $p\in Q$ we remove its descendants that have a too high $p$-induced congestion and apply the bottom-to-top pruning technique (see Lemma \ref{lem:bot-to-top}) to argue that we obtain a locally good solution.



The goal of this subsection is to prove the following lemma.
\begin{lemma}
\label{lem:locallynearlygood} We can compute in expected polynomial time a locally nearly good solution.
\end{lemma}

To obtain such a nearly good solution, we will proceed layer by layer, where the top layers are already rounded integrally and the bottom layers are still fractional. However, unlike the case of the preprocessing, we cannot argue with high probability and union bounds, since some properties we want only deviate from expectation by $\textrm{poly}(\log\log) (n)$ factors. To obtain a locally nearly good solution, we will use the Lov\'asz Local Lemma (LLL) in every iteration, where one iteration rounds one more layer. In the following, we describe the rounding procedure, the bad events and an analysis of their dependencies and finally we apply LLL.

\paragraph{The randomized rounding procedure.} We proceed layer by layer to round the solution $y$ to an integral solution $Q$. We start by adding a single copy the trivial path $(s)$ for each source $s\in S$. Assume we rounded until layer $i$, that is we defined a multiset of paths $Q^{(i)}$ for all paths that end in $L_{\le i}$. 

To round until layer $i+1$ we proceed as follows. Every open path $p\in Q^{(i)}\cap L_i$ selects exactly $k/200$ children where the $i$-th child equals $q\in L_{i+1}$ probability equal to 
\begin{equation*}
    \frac{y(q)}{\sum_{q'\in C_{P'}(p)}y(q')}\ .
\end{equation*}
The selection of each child is independent of the choices made for other children. We define by $Q'_p$ the multiset of children that are chosen by $p$ in this way. For any path $q\in Q'_p$, we set its parent to $p$ (note that this parent is indeed unique) and we add the set $Q'_p$ to our solution $Q^{(i)}$ to obtain $Q^{(i+1)}$. That is, we set
\begin{equation*}
    Q^{(i+1)} \leftarrow Q^{(i)} \cup (\cup_{p\in Q^{(i)}\cap L_i} Q'_p).
\end{equation*}
We will repeat this procedure until reaching the last layer $h$. We will analyze this procedure using LLL.





\paragraph{The bad events for global congestion.}

\paragraph{The bad events for local congestion.} The second type of bad events will deal with local congestion. We need a few more definitions. For any $p \in L_{\leq i}\cap L_{\ge i-\ell}$ (recall that $\ell=10 \log \log (n)$) we define the set of \textit{bad} descendants with respect to $p$ and step $i$ as the set of paths $q\in L_{|p|+\ell}\cap P'$ such that
\begin{equation*}
    \textrm{cong}^{(i)}(p,v_q) \ge 10^3 (\log \log (n))^2.
\end{equation*} Intuitively, this is the set of descendant paths $q$ at a fixed distance from $p$ that have a high conditional congestion at their endpoint $v_q$. This set of bad paths is denoted $B_p^{(i)}$. We say that a path $p \in L_{\leq i}\cap L_{\ge i-\ell}$ is \textit{marked} at step $i+1$ if \begin{equation*}
    \left| B_p^{(i+1)}\setminus B_p^{(i)} \right| \ge \frac{100(\log \log (n))^2}{\exp(10^3(\log \log (n)^2)}\cdot \left(\frac{(100 \log^2 (n))\cdot k}{10}\right)^{\ell},
\end{equation*} that is a lot of descendant paths become marked. We denote this set of marked paths by $M_{i+1}$. We choose this particular threshold because of the granularity of the solution $y$. Indeed, in the solution $y$, each path has $(k/10)\cdot (100\log^2(n))$ children paths. Hence at distance $\ell$, a path has at most $((k/10)\cdot (100\log^2(n)))^{\ell}$ descendants.

We are now ready to state the second type of bad event. We define the bad event $\mathcal B_p$ for any $p \in L_{\leq i}\cap L_{\ge i-\ell}$ as the fact that 
\begin{equation*}
    |C_{Q^{(i+1)}}(p) \cap M_{i+1}|\ge \frac{k}{200(\log \log (n))^2},
\end{equation*}
which intuitively means that a lot of children of $p$ become marked at step $i+1$, counting only children that are actually included in the partial solution $Q^{(i+1)}$.

















%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\etienne{To be continued...}



\paragraph{The probabilities and dependencies of the bad events.} In this part, we upper bound the probability of each bad event happening with the following lemma. Note that we assume that no bad events happened in previous iterations of the rounding (we will show in particular that this implies that Equation \eqref{eq:lowcongestion_partialrounding} was maintained so far).
\begin{lemma}
\label{lem:badevent_proba}
Assume that no bad events happened until layer $\ell$. Then for any $v\in V$ and integer $t$, we have that
\begin{equation*}
    \mathbb P(\mathcal B_{v,t})\leq n^{-2^{t+5}}.
\end{equation*}
For any $p \in L_{\leq i}\cap L_{\ge i-\ell}$, we have that
\begin{equation*}
    \mathbb P(\mathcal B_p)\le \exp\left(-\frac{k}{220 (\log \log(n))^2} \right).
\end{equation*}
\end{lemma}
\begin{proof}
As remarked above, $C_{\lambda, v, t}$ is the sum of independent random variables that take value in the set $\{0\}\cup (2^{-(t+1)},2^{-t}]$. By a standard Chernoff bound, we obtain that the probability the bad event $\mathcal B_{\lambda,v,t}$ happens is at most 
\begin{equation*}
    \exp\left( \frac{-100 \log(n)}{3 \cdot 2^{-t}}\right)\le n^{-2^{t+5}}.
\end{equation*}
For the second claim, we first note that for a fixed path $\lambda'$, any vertex $v$ that does not belong to $B_{\lambda'}^{(\ell)}$ must satisfy 
\begin{equation*}
    \sum_{\lambda'' \in D(\lambda')\cap L_{\ell}} \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y_{\mid \lambda''}(\lambda''') \le 10^3 (\log \log (n))^2,
\end{equation*} by definition. Furthermore, the value (note the change in the first index of the sum)
\begin{equation*}
    \sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}} \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y_{\mid \lambda''}(\lambda''')
\end{equation*} is sum of independent random variables that can take value at most 
\begin{equation*}
    \max_{\lambda'' \in L_{\ell+1}} \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y_{\mid \lambda''}(\lambda''') =   \max_{\lambda'' \in L_{\ell+1}} \frac{\sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y(\lambda''')}{\tilde y (\lambda'')} \le 2.
\end{equation*} (using Constraint \eqref{eqSparseLP:capacity}). Moreover, when a sampled path $\lambda''\in L_\ell$ chooses its children in $L_{\ell+1}$, each such path $\lambda'''\in L_{\ell+1}$ is chosen in expectation
\begin{equation*}
    \frac{k}{100} \cdot \frac{\tilde y_{\mid \lambda''}(\lambda''')}{\sum_{\lambda''''\in C(\lambda'')}\tilde y_{\mid \lambda''}(\lambda'''')} = \frac{k}{100} \cdot \frac{\tilde y(\lambda''')}{\sum_{\lambda'''' \in C(\lambda'')}\tilde y(\lambda'''')} = \frac{\tilde y(\lambda''')}{10\cdot \tilde y(\lambda'')}.
\end{equation*} times (using constraint \eqref{eqSparseLP:demand}). Let us call $N_{\lambda'''}$ the number of times a path $\lambda'''\in L_{\ell+1}$ is taken in the process. Putting everything together, we can compute by linearity of expectation that
\begin{align*}
    \mathbb E[\sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}} \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y_{\mid \lambda''}(\lambda''')] &= \sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}} \mathbb E[N_{\lambda''}] \cdot \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \frac{\tilde y(\lambda''')}{\tilde y(\lambda'')}\\
    &= \sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}} \frac{\tilde y(\lambda'')}{10\cdot \tilde y(P(\lambda''))} \cdot \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \frac{\tilde y(\lambda''')}{\tilde y(\lambda'')}\\
    &=\sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}}  \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \frac{\tilde y(\lambda''')}{10 \tilde y(P(\lambda''))}\\
    &\leq 10^2 (\log \log (n))^2.
\end{align*}
Hence the random variable 
\begin{equation*}
    \sum_{\lambda'' \in D(\lambda')\cap L_{\ell+1}} \sum_{\lambda''' \in D(\lambda'')\cap A(v)} \tilde y_{\mid \lambda''}(\lambda''')
\end{equation*} has expectation at most $10^2 (\log \log (n))^2$ and is written as a sum of independent random variables that take value at most $2$. By a standard Chernoff bound, the probability that a vertex $v$ belongs to $B_{\lambda'}^{(\ell+1)}\setminus B_{\lambda'}^{(\ell)}$ is at most 
\begin{equation*}
    \exp(-300 (\log \log(n)^2).
\end{equation*}
Now fix a $\lambda'\in C(\lambda)$. To be marked at step $\ell+1$, it must be (by definition) that 
\begin{equation*}
    \left| B_{\lambda'}^{(\ell+1)}\setminus B_{\lambda'}^{(\ell)} \right| \ge \frac{100(\log \log (n))^2}{\exp(300(\log \log (n)^2)}\cdot \left(\frac{(100 \log^2 (n))\cdot k}{10}\right)^{10\log \log n}.
\end{equation*} 
However, $\lambda'$ has only at most $\left(\frac{(100 \log^2 (n))\cdot k}{10}\right)^{10\log \log n}$ descendants $\lambda''$ that are at distance $10\log \log (n)$, end at $v$, and are such that $\tilde y(\lambda'')\neq 0$. Hence, for $\lambda'$ to be marked at step $\ell+1$, it must be that the value $\left| B_{\lambda'}^{(\ell+1)}\setminus B_{\lambda'}^{(\ell)} \right|$ exceeds its expectation by a multiplicative factor of at least $100(\log \log (n))^2$. By Markov's inequality, this can happen only with probability at most 
\begin{equation*}
    \frac{1}{100 (\log \log (n))^2}.
\end{equation*}
To finish the proof, we notice for any fixed $\lambda\in L_{\le \ell-1}\cap L_{\ell-10 \log \log (n)}$, $\lambda'\in C(\lambda)\cap M_{\ell+1}$ and $\lambda''\in C(\lambda)\cap M_{\ell+1}$ are independent events for $\lambda'\neq \lambda''$. Indeed, these events depend only on random choices made by descendants of $\lambda'$ or $\lambda''$ respectively. Hence the number of children of $\lambda$ that are marked at step $\ell+1$ is a sum of boolean random variables that are independent. Since $\lambda$ has $k/100$ children by construction, each of them being marked at step $\ell+1$ independently with probability $\frac{1}{100 (\log \log (n))^2}$. We conclude that the probability that more than $\frac{k}{200 (\log \log (n))^2}$ are marked happens with probability at most 
\begin{equation*}
    \exp\left(-\frac{k}{220(\log \log (n))^2} \right).
\end{equation*}
\end{proof}


To bound the dependencies between bad events, for any bad event of first or second type $\mathcal B$ we define $\mathcal N_1(\mathcal B)$ to be the set of bat events of the first type $\mathcal B_{v,t}$ that depend on the bad event $\mathcal B$. Similarly, $\mathcal N_2(\mathcal B)$ is the set of bad events of the second type that are not independent of $\mathcal B$. We prove the following lemma.
\begin{lemma}
\label{lem:badevents_dependencies}
Assume that no bad events happened until layer $\ell$. Then for any bad event $\mathcal B$, we have that
\begin{equation*}
    |\mathcal N_1(\mathcal B)|\leq 10n^3.
\end{equation*}
Furthermore, for any $\lambda$, $v\in V$ and integer $t$, we have 
\begin{equation*}
    |\mathcal N_2(\mathcal B_{\lambda,v,t})|\leq (10^6 \log^6(n))\cdot 2^{(t+1)},
\end{equation*}
and for any $\lambda \in L_{\leq \ell}\cap L_{\ge \ell-10\log \log (n)}$, we have
\begin{equation*}
    |\mathcal N_2(\mathcal B_{\lambda})|\leq (k/100)^{11\log \log (n)}.
\end{equation*}
\end{lemma}
\begin{proof}
The first statement is easy to prove. There are at most $(k/100)^\ell \cdot n\cdot (10\log^2(n))\le 10n^{3}$ bad events of the first type in total ($(k/100)^\ell$ options for the choice of $\lambda\in L_{\le \ell}$ such that $\hat m_\lambda\neq 0$, $n$ possibilities of the choice of vertex $v$ and $10\log^2(n)$ possibilities for the choice of $t$).

For the second statement, we first notice that the bad event $\mathcal B_{\lambda,v,t}$ depends only on selecting paths $\lambda' \in L_{\ell+1}$ such that 
\begin{equation*}
    \frac{\sum_{\lambda''\in D(\lambda')\cap A(v)}\tilde y(\lambda'')}{\tilde y(\lambda')} \ge 2^{-(t+1)}.
\end{equation*}
Call this set of paths $\Lambda_t$. We can now count how many sampled paths $\lambda''' \in L_\ell$ have at least one child in $\Lambda_t$. For each such sampled path $\lambda''' \in L_\ell$, we have that 
\begin{align*}
    \sum_{\lambda'\in C(\lambda''')} \sum_{\lambda''\in D(\lambda')\cap A(v)} \tilde y (\lambda'') &\ge \sum_{\lambda'\in C(\lambda''')\cap \Lambda_t} \sum_{\lambda''\in D(\lambda')\cap A(v)} \tilde y (\lambda'')\\
    &\ge \sum_{\lambda'\in C(\lambda''')\cap \Lambda_t} 2^{-(t+1)}\tilde y (\lambda')\\
    &\ge \frac{ 2^{-(t+1)}}{(100\log^2(n))^{\ell+1}}.
\end{align*}
(in the last step we used the granularity of $\tilde y$, see constraint \eqref{eqSparseLP:granularity}). By Equation \eqref{eq:lowcongestion_partialrounding}, we also have that 
\begin{equation*}
    \sum_{\lambda''\in D(\lambda''')\cap A(v)} \frac{\tilde y(\lambda'')}{\tilde y(\lambda''')} \le (1500\log^3(n)) \cdot \frac{\tilde y(\lambda''')}{\tilde y(\lambda''')},
\end{equation*}
which is equivalent to 
\begin{equation*}
    \sum_{\lambda''\in D(\lambda''')\cap A(v)} \tilde y(\lambda'') \le (1500\log^3(n)) \cdot \tilde y(\lambda''').
\end{equation*}
By the calculation above, we saw that for each path $\lambda'''$ that has at least one child in $\Lambda_t$ we obtain
\begin{equation*}
    \sum_{\lambda''\in D(\lambda''')\cap A(v)} \tilde y(\lambda'') \ge \frac{2^{-(t+1)}}{(100\log^2(n))^{\ell+1}}.
\end{equation*}
Hence the number of such paths $\lambda'''$ can be at most 
\begin{equation*}
    \frac{(1500\log^3(n)) \cdot \tilde y(\lambda''')}{\frac{2^{-(t+1)}}{(100\log^2(n))^{\ell+1}}} \le (10^6 \log^5(n))\cdot 2^{(t+1)}.
\end{equation*} (note that here we assume that $y(\lambda''')$ is equal to $1/(100\log^2(n))^\ell$ by simply making copies of the same path if it was taken more than once in the preprocessing).

Each such path $\lambda'''$ can in turn only influence bad events $\mathcal B_{\lambda'}$ only if $\lambda'''$ is a descendant of $\lambda'$, and it is clear that any path has at most $h\le \log n$ ancestors. Hence we obtain 
\begin{equation*}
    |\mathcal N_2(\mathcal B_{\lambda,v,t})|\leq (10^6 \log^6(n))\cdot 2^{(t+1)}.
\end{equation*}

Finally, for the last statement fix a bad event $\mathcal B_\lambda$. Such a bad event depends only on the sampling done by descendant sampled paths $\lambda'\in L_\ell$. There are only $(k/100)^{\ell-|\lambda|}\le (k/100)^{10\log \log (n)} $ such paths.\larstodo{This is wrong. It depends also on paths being not sampled.} Each such sampled path $\lambda'\in L_\ell$ can only influence a bad event $\mathcal B_{\lambda''}$ if $\lambda'\in D(\lambda'')$. Hence we obtain in total
\begin{equation*}
    (\log (n))\cdot (k/100)^{10\log \log (n)} \le (k/100)^{11\log \log (n)},
\end{equation*} which ends the proof of the lemma.
\end{proof}

\paragraph{Rounding layer $\ell+1$ using LLL.} Using Lemma \ref{lem:badevent_proba} and \ref{lem:badevents_dependencies}, we are ready to set up LLL. We will set for any bad event $\mathcal B_\lambda$
\begin{equation*}
    x(\mathcal B_\lambda) := \exp\left(-\frac{k}{440 (\log \log (n))^2} \right),
\end{equation*}
and for any bad event $\mathcal B_{\lambda, v,t}$
\begin{equation*}
    x(\mathcal B_\lambda) = n^{-2^4}.
\end{equation*}
Then we can compute for any $ \lambda \in L_{\leq \ell-1}\cap L_{\ge \ell-10\log \log (n)}$ (we assume that $k\ge 10^3 (\log \log(n))^4)$ and $n$ bigger than a sufficiently large constant),
\begin{align*}
    x(\mathcal B_\lambda ) &\cdot \prod_{\mathcal B \in \mathcal{N}_1(\mathcal B_\lambda)\cup \mathcal{N}_2(\mathcal B_\lambda)}(1-x(\mathcal B)) \\
    &\ge \exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot \left(1-n^{-2^{4}}\right)^{10n^3} \cdot \left(1-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)\right)^{(k/100)^{11 \log \log (n)}} \\
    &\ge \exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot \left(1-n^{-2^{4}}\right)^{10n^3} \cdot \frac{1}{2}\cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log (n))^2}\right) \cdot (k/100)^{11 \log \log (n)}\right)\\
    &\ge \frac{\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)}{6} \cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log(n))^2} + (100\log \log (n))\cdot \log (k)  \right)   \right)\\
    &\ge \frac{\exp\left(-\frac{k}{440 (\log \log (n))^2} \right)}{6} \cdot e^{-1} \ge \mathbb P(\mathcal B_\lambda).
\end{align*}

Similarly, for any $\lambda,v,t$ we obtain
\begin{align*}
    x(\mathcal B_{\lambda,v,t} ) &\cdot \prod_{\mathcal B \in \mathcal{N}_1(\mathcal B_\lambda)\cup \mathcal{N}_2(\mathcal B_\lambda)}(1-x(\mathcal B))\\
    &\ge n^{-2^{4}} \cdot \left(1-n^{-2^4}\right)^{10n^3} \cdot \left(1-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \right)^{(10^6\log^6(n))\cdot 2^{(t+1)}}\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-\exp\left(-\frac{k}{440 (\log \log (n))^2} \right) \cdot (10^6\log^6(n))\cdot 2^{(t+1)}\right)\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-\exp\left(-2(\log \log(n))^2 \right) \cdot (10^6\log^6(n))\cdot 2^{(t+1)}\right)\\
     &\ge \frac{n^{-2^{4}}}{6}\cdot \exp\left(-2^{(t+1)}\right)\\
     &\ge n^{-2^{(t+5)}}\ge \mathbb P(\mathcal B_{\lambda,v,t}).
\end{align*}
We can conclude using known results on LLL that we can round in polynomial time the layer $\ell+1$ without any bad event happening. We show in particular that Equation \eqref{eq:lowcongestion_partialrounding} is maintained with $\tilde Y_{\ell+1}$. No bad event implies that for any fixed $\lambda\in L_{\le \ell},v\in V$
\begin{equation*}
    \sum_{t=-1}^{10 \log^2 (n)} C_{\lambda,v,t} \le 2\mathbb E[\sum_{t=-1}^{10 \log^2 (n)} C_{\lambda,v,t}] + 1000\log^3(n).
\end{equation*}
To compute $\mathbb E[\sum_{t=-1}^{10 \log^2 (n)} C_{\lambda,v,t}]$ denote by $N_{\lambda'}$ the number of times a path $\lambda' \in L_{\ell+1}$ is selected by its parent. Notice that 
\begin{align*}
   \mathbb E[ \sum_{t=-1}^{10 \log^2 (n)} C_{\lambda,v,t}] &= \sum_{\lambda' \in D(\lambda)\cap L_{\ell+1}} \mathbb E[ N_{\lambda'}] \cdot \sum_{\lambda''\in D(\lambda')\cap A(v) } \frac{\tilde y (\lambda'')}{\tilde y(\lambda')}\\
   &= \sum_{\lambda' \in D(\lambda)\cap L_{\ell+1}} \frac{\tilde y(\lambda')}{10 \cdot \tilde y(P(\lambda'))} \cdot \sum_{\lambda''\in D(\lambda')\cap A(v) } \frac{\tilde y (\lambda'')}{\tilde y(\lambda')}\\
   &= \frac{1}{10} \cdot \sum_{\lambda' \in D(\lambda)\cap L_{\ell}} \sum_{\lambda''\in D(\lambda')\cap A(v) } \frac{\tilde y (\lambda'')}{\tilde y(\lambda')}
\end{align*}
Hence we see that
\begin{equation*}
    \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{\ell+1}(\lambda') = \frac{1}{10}\cdot  \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{\ell}(\lambda'),
\end{equation*}

and if Equation \eqref{eq:lowcongestion_partialrounding} holds before step $\ell+1$ and no bad event happens then we obtain 
\begin{equation*}
    \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{\ell+1}(\lambda') \leq \frac{1}{10}\cdot  \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{\ell}(\lambda') + 1000\log^3(n) \le 1500 \log^3(n)
\end{equation*} for each distinct sampled copy of $\lambda$. Hence when summing over all copies of $\lambda$, we indeed obtain
\begin{equation*}
    \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{\ell+1}(\lambda') \leq  (1500 \log^3(n))\cdot \tilde Y_{\ell+1}(\lambda).
\end{equation*}

\paragraph{Wrapping-up.} We proved that we can round in polynomial time from layer 0 to layer $h$ without any bad event ever happening. In particular, by applying Equation \eqref{eq:lowcongestion_partialrounding} with $\lambda=(r)$, we obtain that for any $v$
\begin{equation*}
    \sum_{\lambda' \in D(\lambda)\cap A(v)} \tilde Y_{h}(\lambda') \le 1500 \log^3(n).
\end{equation*} We indeed get poly-logarithmic congestion on all vertices. Furthermore, we obtain that for any sampled path $\lambda$ has at most 
\begin{equation*}
    |\cup_{\ell} M_\ell \cap C(\lambda)|\le (10 \log \log (n)) \cdot \frac{k}{200 (\log \log (n))^2} \le \frac{k}{20 \log \log (n)}
\end{equation*} marked children. We now delete from the solution all the marked paths. This means that any sampled path retains at least
\begin{equation*}
    \frac{k}{100}-\frac{k}{20 \log \log (n)} \ge  \frac{k}{200}
\end{equation*} children (assuming $n$ big enough). Therefore we obtain a solution of global congestion such that:
\begin{itemize}
    \item Every selected path has at least $k/200$ children,
    \item The global congestion is at most $1500 \log^3(n)$, and 
    \item No path is marked.
\end{itemize}
A path that is not marked has at most 
\begin{align*}
    (10 \log \log n) \cdot & \frac{100(\log \log (n))^2}{\exp(10^3(\log \log (n))^2)}\cdot \left(\frac{(100 \log^2 (n))\cdot k}{10}\right)^{10\log \log n}\\
    &\le \left(k/200 \right)^{10\log \log (n)}\cdot \frac{10^3 (\log \log(n))^3}{\exp((\log \log (n))^2)} \cdot \left(\frac{2000 \log^2 (n)}{\exp(10^2(\log \log (n)))} \right)^{10\log \log (n)} \\
    &\le \frac{\left(k/200 \right)^{10\log \log (n)}}{2^{10\log \log (n)}} = \frac{\left(k/200 \right)^{10\log \log (n)}}{\log^{10}(n)}.
\end{align*} bad descendant vertices at distance $10 \log \log (n)$. Hence only a $1/(\log^{10}(n))$ fraction of descendant vertices at distance $10 \log \log (n)$ have congestion more than $10^3(\log \log (n))^2$. This concludes the proof of Lemma \ref{lem:locallynearlygood}.
\subsection{From locally nearly good to locally good}
TODO
\newpage
















%%%%%%%%%%%%%%%%%%%%%

\subsection{Sampling a locally nearly good solution v2}

We start this part with the sparse solution $y$ and the multiset of paths $P'$ that we computed above. We will proceed to round this fractional solution to an integral solution that is \textit{locally nearly good}. We recall or define here a few concepts before moving to the definition of locally nearly good solutions. $D_{Q}(p, \ell')$ will denote the set of descendant paths of $p$ at distance $\ell'$ of $p$ in a multiset $Q$. If $q\in D_{Q}(p, \ell')$, we will say that $q$ is an $\ell'$-descendant of $p$. In the whole proof, we set $\ell=10\log \log (n)$. We will say that two paths $p$ and $p'$ are \textit{globally equivalent} if
\begin{enumerate}
    \item $p,p'\in Q$,
    \item $|p|=|p'|$, and
    \item $p$ and $p'$ traverse the same tuple of vertices until layer $|p|-\ell$. That is, they follow the same path in the graph $G$ except maybe for the last $\ell$ vertices.
\end{enumerate}
We will write $p\sim p'$ if $p$ and $p'$ are globally equivalent. Note for instance that all the paths containing only a source are globally equivalent. Using this, several important quantities will keep track of the congestion in various senses. 

\begin{definition}[Global congestion on a vertex]
The \textit{total congestion} on vertex $v$ is simply the total number of paths in $Q$ that end at $v$. This is denoted by $|I_Q(v)|$.
\end{definition}
\begin{definition}[$p$-induced congestion on a path $q$]
The \textit{$p$-induced congestion} on path $q$ is the total number of paths $q'$ that are an $\ell'$-descendant of a path $p'\sim p$ and end at the endpoint of $q$. Formally, this is defined as follows.
\begin{equation*}
    \textrm{cong}_{Q,p}(q) = \sum_{p'\sim p} |D_Q(p',\ell')\cap I_Q(q)|.
\end{equation*}
\end{definition}
For intuition, the reader might ignore that we are summing up to global equivalence assuming there is a single source. If there are several sources, we need this more involved definition in the first $\Theta(\ell)=\Theta (\log \log (n))$ layers of the rounding.
\begin{definition}[$\ell'$-local congestion on a path $p$]
The \textit{$\ell'$-local congestion} on path $p$ is the sum over all paths $q$ that are $\ell'$-descendants of $p$ of the $p$-induced congestion on $q$. This is denoted as follows.
\begin{equation*}
    \textrm{cong}_Q(p,\ell'):=\sum_{q\in D_{Q}(p, \ell')} \textrm{cong}_{Q,p}(q)\ .
\end{equation*}
\end{definition}
Intuitively, the $\ell'$-local congestion is counting the number of pairs of $\ell'$-descendants of $p$ that overlap (up to global equivalence). This quantity will be used to measure the average congestion, in a similar spirit as in Section \ref{sec:loc-to-glob}.

We are now ready to define the notion of locally nearly good solution. A \textit{locally nearly good solution} is a multiset of paths $Q$ (where again every path has a \textbf{unique} parent among the relevant copies of the same path) that has the following properties:
\begin{enumerate}
    \item One copy of the trivial path $(s)$ belongs to $Q$ for all sources $s\in S$;
    \item Every open path has $k/200$ children;
    \item No vertex has global congestion more than $1500 \log^3(n)$;
    \item For every path $p\in Q$ and any $1\le \ell'\le \ell$ we have that
    \begin{equation*}
        \textrm{cong}_Q(p,\ell')\le   k^{\ell'}\cdot (10^3 \log \log (n))^2 \ .
    \end{equation*}
\end{enumerate}

The goal of this subsection is to prove the following lemma.
\begin{lemma}
\label{lem:locallynearlygood} We can compute in expected polynomial time a locally nearly good solution.
\end{lemma}

To obtain such a nearly good solution, we will proceed layer by layer, where the top layers are already rounded integrally and the bottom layers are still fractional. However, unlike the case of the preprocessing, we cannot argue with high probability and union bounds, since some properties we want only deviate from expectation by $\textrm{poly}(\log\log) (n)$ factors. To obtain a locally nearly good solution, we will use the Lov\'asz Local Lemma (LLL) in every iteration, where one iteration rounds one more layer. In the following, we describe the rounding procedure, the bad events and an analysis of their dependencies and finally we apply LLL.

\paragraph{A few more definitions: Conditional congestion.} Before defining our bad events, we define here a few useful quantities that we will need to keep track of. We define here various notion notions of \textit{conditional} congestion in the sense that we will condition by all the sampling that was done until step $i$ included. This can be seen as generalizations of notions that appear in Appendix \ref{sec:Sparsify} for the preprocessing step. First of all, we define the fractional congestion induced by some path $p\in P'\cap L_{\ge i}$ on a vertex $v\in V$ as follows.
\begin{equation*}
      \textrm{cong}(p,v) := \sum_{q\in D_{P'}(p)\cap I_{P'}(v)} y(q).
\end{equation*}
Using this definition, we will define the conditional fractional congestion at step $i$ induced by $p$ on path $q$ as follows.
\begin{equation*}
    \textrm{cong}_p(q \mid Q^{(i)}) := \begin{cases}
    \sum_{p'\sim p} |\{q' \in D_{Q^{(i)}}(p')\cap I_{Q^{(i)}}(q) \}| & \textrm{if }
    v\in L_{\le i}\\
    \sum_{p'\sim p} \sum_{q'\in D_{Q^{(i)}}(p')\cap L_i} \frac{1}{y(q)}\cdot \textrm{cong}(q',v_q)  & \textrm{otherwise.}
    \end{cases}
\end{equation*}
We will use this definition only for $p\in Q^{(i)}\cup L_{\ge i+1}$. If $v$ belongs to one of the first $i$ layers (i.e. $v$ is in the integral part corresponding to the partial solution), this is simply the number of paths descendants of $p\in Q^{(i)}$ in our partial solution that end at $v$. Otherwise, this is the total fractional congestion induced by all the paths that we actually selected in our partial solution $q\in Q^{(i)}$ and that are descendants of $p$. The name \textit{conditional} comes from the term $\frac{1}{y(q)}$ which is simply the fact that we condition on having already selected the path $q$.

The global congestion at step $i$ on a vertex $v\in V$ is also straightforward to define.
\begin{equation*}
    \textrm{cong}(v\mid Q^{(i)}) := \begin{cases}
     |\{q \in Q^{(i)}\cap I(v)\}| & \textrm{if }
    v\in L_{\le i}\\
    \sum_{q\in Q^{(i)}\cap L_i} \frac{1}{y(q)}\cdot \textrm{cong}(q,v)  & \textrm{otherwise.}
    \end{cases}
\end{equation*}


\paragraph{The first bad event: Global congestion.} Before moving to the definition of bad events for global congestion, we emphasize that if no such bad event happened before rounding layer $i$ and during the rounding of layer $i+1$, it will be easy to show that the following low congestion property is maintained.
\begin{equation}
\label{eq:lowcongestion_partialrounding}
      \textrm{cong}(v\mid Q^{(i)}) \le  1500 \log^3(n), \ \forall v\in V
\end{equation}

Indeed, the first type of bad events will deal with maintaining this global congestion property for every vertex $v\in V$. However, for some technical reasons we will first partition the multiset $P'\cap L_{i+1}$ of candidate paths according to the conditional fractional congestion that they induce on $v$. More precisely, fix an integer $t\ge 0$, then we denote by $P'_{v,t}$ the multiset of all paths $p\in P'\cap L_{i+1}$ such that 
\begin{equation*}
      \frac{\textrm{cong}(p,v)}{y(q)}  \in (2^{-t},2^{-(t-1)}].
\end{equation*}

We are now ready to define our first type of bad event. We fix a vertex $v\in V$ and an integer $t\ge 0$ and for any path $p\in P'\cap L_{i+1}$ we denote by $N_p$ the random variable that is the number of copies of this path $p$ that are selected by its parent. Then the bad event $\mathcal B_{v,t}$ is defined as the event that
\begin{equation*}
   Z_{v,t}:= \sum_{q\in P'_{v,t}} N_q \cdot \frac{\textrm{cong}(q,v)}{y(q)} \ge 2\mathbb E[Z_{v,t}] + 100 \log(n).
\end{equation*}

At this point, it is worthwhile to mention that because of the low granularity of the starting fractional solution $y$, $t$ can only take values in the interval $[0,10\log^2(n))$. Indeed, simply rewriting Constraint \eqref{eqSparseLP:capacity}, we obtain that 
\begin{equation*}
    \textrm{cong}(q,v) \le 2,
\end{equation*} for any $q\in P'$ and any $v\in V$. Moreover, by Constraint \eqref{eqSparseLP:granularity}, we have that the smallest non-zero value that $\textrm{cong}(q,v)$ can take is at least
\begin{equation*}
    \frac{1}{(4\log^2 (n))^{h-|q|}} \ge \frac{1}{(4\log^2 (n))^{h}} \ge \frac{1}{(4\log^2 (n))^{\log (n)}}\ .
\end{equation*}
Hence our bad events $\mathcal B_{v,t}$ will only be instantiated for $t\in [0,10\log^2 (n))$. 



\paragraph{The second bad event: Local congestion.} The second type of bad event will deal exactly with the local congestion. We fix a path $p\in Q^{(i)}$ and some $1\le \ell'\le \ell$. Recall that we want to obtain an upper bound on the quantity
\begin{equation*}
    \textrm{cong}_Q(p,\ell')=\sum_{q\in D_{Q}(p, \ell')} \textrm{cong}_{Q,p}(q) = \sum_{q\in D_{Q}(p, \ell')}\sum_{p'\sim p} |D_Q(p',\ell')\cap I_Q(q)|\ .
\end{equation*}
For this we will use the quantity $ \textrm{cong}_p(q \mid Q^{(i)})$ previously defined. We define 
\begin{equation*}
    \textrm{cong}(p,\ell' \mid Q^{(i)}) = \sum_{q\in D_{}}
\end{equation*}



==> deleted/deletedLABELEDPATH.tex <==
In the rest of Section \ref{sec:locallygood}, it can happen that we sample several times the same path $\lambda$. Hence to avoid confusion, we will denote by $\tilde \lambda$ a path from the root to some vertex $v\in L_{\ell}$ associated with integers $i_1,i_2,\ldots, i_\ell$ that indicate that this path is a descendant the path $\tilde \lambda_1$ which is the $i_1$-th children of the root, as well as a descendant of $\tilde \lambda_2$ which is the $i_2$-th children $\tilde \lambda_1$, and so on. We call such a path a \textit{labeled path.} It might be that two labeled paths are not formally equal but that the corresponding paths in the graph $G$ are in fact identical. 

Apart from this technicality, all the previous definitions for paths without integer IDs extend in the natural way to paths with integer IDs. With a slight abuse of notation, we will also denote by $\tilde \lambda$ the corresponding path in the graph $G$. This will be clear from context when this is the case.

To obtain this, consider the very simple following algorithm, that proceeds layer by layer starting from the root. We define for the root $\tilde y(\tilde{(r)})=1$. Then the root path $\tilde{(r)}$ samples $k/10 \cdot (100 \log n)$ children paths ending at layer 1 independently at random where the $i$-th children is going through the path $\lambda \in L_1$ with probability equal to
\begin{equation*}
    \frac{y^*(\lambda)}{\sum_{\lambda' \in L_1} y^*(\lambda')}.
\end{equation*}
After this sampling we set 
\begin{equation*}
    \tilde y(\tilde \lambda)=\frac{1}{100 \log (n)},
\end{equation*}
for each labeled path $\tilde \lambda$ that was sampled. Assume now that we sampled until layer $\ell$, that is we defined $\tilde y(\tilde \lambda)$ for all $\tilde \lambda \in L_{\leq \ell}$. Then for each labeled path $\tilde \lambda \in L_{\ell}$ that was sampled, we define the truncated flow LP solution $y^*_{\mid \tilde \lambda}$ as follows:
\begin{equation*}
    y^*_{\mid \tilde \lambda}(\lambda'):=
    \begin{cases}
    \frac{1}{(100\log (n))^j} & \textrm{if } j\leq \ell \textrm{ and }\lambda'\in L_j\cap A(\tilde \lambda)\\
    \frac{y^*(\lambda')}{\tilde y(\tilde \lambda)} & \textrm{if }
    \lambda' \in D(\tilde \lambda)\\
    0 & \textrm{otherwise.}
    \end{cases}
\end{equation*}
Intuitively, we are conditioning the flow LP solution $y^*$ by the fact that we already sampled the specific path $\tilde \lambda$.

Then, every labeled path $\tilde \lambda$ samples $k/10 \cdot (100 \log n)$ children paths independently in the same way as the root. That is, the $i$-th child corresponds to the path $\lambda' \in L_{\ell+1}$ with probability equal to
\begin{equation*}
    \frac{y^*_{\mid \tilde \lambda}(\lambda')}{\sum_{\lambda'' \in L_{\ell+1}} y^*_{\mid \tilde \lambda}(\lambda'')}.
\end{equation*}

After any iteration $\ell$ of the above process, we define the following object
\begin{equation*}
    Y^*_\ell:=\sum_{\tilde \lambda \in L_\ell}y^*_{\mid \tilde \lambda}.
\end{equation*}
Note that $Y_0^*$ is simply equal to $y^*$ while $Y_h^*$ is equal to the final $\tilde y$.


\begin{lemma}
With high probability, we have the following properties after step $\ell$ of the above process.
\begin{align}
    \sum_{\lambda'\in C(\lambda)} y(\lambda') &= k \cdot y(\lambda) &\textrm{for all } \lambda \textrm{ that is not closed} \label{eqLP:flowLPdemand}\\
     \sum_{\tilde \lambda'\in A(v)\cap D(\tilde \lambda)} y(\lambda') &\leq y(\lambda) &\forall \lambda,v \label{eqLP:flowLPcapacity}\\
    y((r)) &= 1 & \label{eqLP:flowLPdemandroot}\\
    y &\ge 0 & 
\end{align}
\end{lemma}


==> deleted/deletedPREPROCESSING.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%
. For each path $ \lambda \in L_{\ell}$ that was sampled (i.e. such that $m_\lambda \neq 0$), we define the truncated solution $y^*_{\mid \lambda}$ as follows:
\begin{equation*}
    y^*_{\mid  \lambda}(\lambda'):=
    \begin{cases}
    \frac{\tilde y( \lambda)}{(k/10)^{\ell-j}} & \textrm{if } j\leq \ell \textrm{ and }\lambda'\in L_j\cap A( \lambda)\\
    y^*(\lambda') \cdot \frac{\tilde y( \lambda) }{ y^*( \lambda)} & \textrm{if }
    \lambda' \in D( \lambda)\\
    0 & \textrm{otherwise.}
    \end{cases}
\end{equation*}
\larstodo{what about Layer $L_{\ell}$?}
Then, every path $\lambda$ that is not closed samples $m_\lambda\cdot (k/10) \cdot (100 \log n)$ children paths independently in the same way as the root. That is, the $i$-th child goes through the path $\lambda' \in L_{\ell+1}$ with probability equal to
\begin{equation*}
    \frac{y^*_{\mid  \lambda}(\lambda')}{\sum_{\lambda'' \in C(\lambda)} y^*_{\mid \lambda}(\lambda'')}.
\end{equation*}
After this process, each path $\lambda' \in L_{\ell+1}$ is taken some $m_{\lambda'}$ times and we set
\begin{equation*}
    \tilde y( \lambda')=\frac{m_{\lambda'}}{(100 \log^2 (n))^{\ell+1}}.
\end{equation*}
We claim that after $h$ iterations, we get with high probability the desired solution $\tilde y$ that satisfies constraint  \eqref{eqSparseLP:demand}, \eqref{eqSparseLP:capacity}, \eqref{eqSparseLP:granularity}, and \eqref{eqSparseLP:root}. To help the formal proof, it will be useful to define the following quantity after $\ell$ iterations.
\begin{equation*}
    Y^*_\ell:=\sum_{ \lambda \in L_\ell}y^*_{\mid  \lambda}+\sum_{ \lambda \in L_{\ell-1}\cap E}y^*_{\mid  \lambda}.
\end{equation*}
Note that $Y_0^*$ is simply equal to $y^*$ while $Y_h^*$ is equal to the final $\tilde y$.

\begin{lemma}
\label{lem:sparsify}
With high probability, we have the following properties after step $\ell$ of the process above.
\begin{align}
    \sum_{\lambda'\in C(\lambda)} Y^*_\ell(\lambda') &= k \cdot Y^*_\ell(\lambda) &\textrm{for all } \lambda\in L_{\geq \ell} \textrm{ that are not closed} \label{eqAggregateLP:demandbottom}\\
    \sum_{\lambda'\in C(\lambda)} Y^*_\ell(\lambda') &= \frac{k}{10} \cdot Y^*_\ell(\lambda) &\textrm{for all } \lambda\in L_{\le \ell-1} \textrm{ that are not closed}\label{eqAggregateLP:demandtop}\\
     \sum_{ \lambda'\in A(v)\cap D( \lambda)} Y^*_\ell(\lambda') &\leq Y^*_\ell(\lambda) &\forall \lambda\in L_{\ge \ell},\forall v\in V\label{eqAggregateLP:capacitybottom}\\
     \sum_{ \lambda'\in A(v)\cap D( \lambda)} Y^*_\ell(\lambda') &\leq 2Y^*_\ell(\lambda) &\forall \lambda\in L_{\le \ell-1},\forall v\in V\label{eqAggregateLP:capacitytop}\\
     Y^*_\ell(\lambda)\cdot (100\log^2 (n))^\ell &\in \mathbb N&\forall \lambda\in L_{\le \ell}\label{eqAggregateLP:granularity}\\
    Y^*_\ell((r)) &= 1 & \label{eqAggregateLP:root}\\
    Y^*_\ell &\ge 0 & 
\end{align}
\end{lemma}
\begin{proof}
We prove this lemma by induction on $\ell\ge 0$. Clearly, for $\ell=0$, we have that $Y_0^*=y^*$ hence $Y_0^*$ satisfies all the constraints \eqref{eqLP:flowLPdemand}, \eqref{eqLP:flowLPcapacity}, and \eqref{eqLP:flowLPdemandroot}. This implies that constraints \eqref{eqAggregateLP:demandbottom}, \eqref{eqAggregateLP:root}, and \eqref{eqAggregateLP:capacitybottom}, \eqref{eqAggregateLP:granularity} are satisfied. Constraints \eqref{eqAggregateLP:capacitytop} and \eqref{eqAggregateLP:demandtop} are vacuously satisfied. 

Next, we assume that $Y_\ell^*$ satisfies the above constraints after step $\ell$. Then we proceed to round one more layer. We verify below the constraints one by one.
\paragraph{Constraint \eqref{eqAggregateLP:demandbottom}.}
Fix a non-closed path $\lambda' \in L_{\ge \ell+1}$ and let $\lambda \in L_{\ell+1}$ be its ancestor. Note that by definition we have that
\begin{equation*}
    y^*_{\mid  \lambda}(\lambda')=\frac{y^*(\lambda')}{\tilde y(\lambda)},
\end{equation*} for any $\lambda'\in D(\lambda)$. By definition, we also note that $Y^*_{\ell+1}(\lambda')=y^*_{\mid  \lambda}(\lambda')$ for any $\lambda'\in D(\lambda)$. Hence we can compute 
\begin{align*}
     \sum_{\lambda''\in C(\lambda')} Y^*_{\ell+1}(\lambda'')&= \sum_{\lambda''\in C(\lambda')} y^*_{\mid  \lambda}(\lambda'')\\
     &=\sum_{\lambda''\in C(\lambda')} y^*(\lambda'') \cdot \frac{\tilde y( \lambda) }{ y^*( \lambda)}\\
     &= \frac{\tilde y( \lambda) }{ y^*( \lambda)} \cdot \sum_{\lambda''\in C(\lambda')} y^*(\lambda'')\\
     &= \frac{\tilde y( \lambda) }{ y^*( \lambda)} \cdot (k\cdot y^*(\lambda')) \\
     &=k\cdot y^*_{\mid  \lambda}(\lambda')\\
     &=k\cdot Y^*_{\ell+1}(\lambda').
\end{align*}
(note that we used the fact that $y^*$ satisfies constraint \eqref{eqLP:flowLPdemand} from the third to the fourth line).
\paragraph{Constraint \eqref{eqAggregateLP:demandtop}.} We first claim that $Y^*_\ell(\lambda')=Y_{\ell+1}^*(\lambda')$ for any $\lambda'\in L_{j}$ with $j\leq \ell$. To see this, note that 
\begin{align*}
    Y^*_\ell(\lambda')&=\sum_{\lambda''\in D(\lambda')\cap L_\ell}y^*_{\mid  \lambda''}(\lambda')\\
    &=  \frac{\sum_{\lambda''\in D(\lambda')\cap L_\ell} \tilde y( \lambda'')}{(k/10)^{\ell-j}}.
\end{align*}
By the definition of the sampling process, each path $\lambda''\in L_\ell$ will sample exactly $(k/10)\cdot (100 \log^2 (n))$ children path $\lambda'''$ and set the value
\begin{equation*}
     \tilde y( \lambda''')=\frac{m_{\lambda'''}}{(100 \log^2 (n))^{\ell+1}}.
\end{equation*}
Hence it is clear that 
\begin{equation*}
    \sum_{\lambda''' \in C(\lambda'')} \tilde y( \lambda''') = (k/10)\cdot \tilde y(\lambda'').
\end{equation*}
By a simple calculation, we can conclude that 
\begin{align*}
    Y^*_{\ell+1}(\lambda')&=\sum_{\lambda''\in D(\lambda')\cap L_{\ell+1}}y^*_{\mid  \lambda''}(\lambda')\\
    &=  \frac{\sum_{\lambda''\in D(\lambda')\cap L_{\ell+1}} \tilde y( \lambda'')}{(k/10)^{\ell+1-j}}\\
    &=\frac{\sum_{\lambda''\in D(\lambda')\cap L_{\ell}} \tilde y( \lambda'')}{(k/10)^{\ell-j}}\\
    &= Y^*_{\ell}(\lambda').
\end{align*}
By induction hypothesis we already had that $Y^*_{\ell}$ satisfies constraint \eqref{eqAggregateLP:demandbottom} for all $\lambda \in L_{\leq \ell-1}$ and $Y^*_{\ell}(\lambda)=Y^*_{\ell+1}(\lambda)$ in that case so the constraint remains verified. It is easy to verify with the same arguments as above that the constraint is now verified also for $\lambda \in L_\ell$.

\paragraph{Constraint \eqref{eqAggregateLP:capacitybottom}.} Fix a $\lambda' \in L_{\ge \ell+1}$ and some $v\in V$. We define $\lambda\in L_{\ell+1}$ to be the ancestor of $\lambda'$. We can compute 
\begin{align*}
     \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'') &=  \sum_{ \lambda''\in A(v)\cap D( \lambda')} y^*_{\mid  \lambda}(\lambda'')\\
     &= \sum_{ \lambda''\in A(v)\cap D( \lambda')} y^*(\lambda'') \cdot \frac{\tilde y( \lambda) }{ y^*( \lambda)}\\
     &\le y^*(\lambda') \cdot \frac{\tilde y( \lambda) }{ y^*( \lambda)}\\
     &= y^*_{\mid  \lambda}(\lambda')\\
     &= Y^*_{\ell+1}(\lambda'),
\end{align*}
where we use constraint \eqref{eqLP:flowLPcapacity} in the third line.

\paragraph{Constraint \eqref{eqAggregateLP:capacitytop}.} Fix a $\lambda' \in L_{\le \ell}$ and some $v\in V$. First note that $Y_\ell^*(\lambda')=Y_{\ell+1}^*(\lambda')$ as proved above. Hence it suffices to prove that with high probability, 
\begin{equation*}
    \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'') \leq 2Y^*_\ell(\lambda').
\end{equation*} 
If $v\in L_{\le \ell}$ then this is true with probability 1 as $ \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'') =  \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell}(\lambda'')$ and by induction we had constraint \eqref{eqAggregateLP:capacitytop} for $Y_\ell^*$. Hence assume $v\in L_{\ge \ell+1}$. Notice that for any $\lambda'' \in A(v)\cap D( \lambda')$ and $\lambda\in A(\lambda'')\cap L_{\ell+1}$ its ancestor in layer $\ell+1$, we have that
\begin{equation*}
    Y^*_{\ell+1}(\lambda'') = y^*_{\mid  \lambda}(\lambda'') = y^*(\lambda'') \cdot \frac{\tilde y( \lambda) }{ y^*( \lambda)}.
\end{equation*}
Hence we can decompose the sum
\begin{equation}
\label{eq:sparsificationCongestion}
      \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'') = \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}} \sum_{\lambda '' \in D(\lambda)\cap A(v)} Y^*_{\ell+1}(\lambda'') = \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}} \left[\frac{\tilde y( \lambda) }{ y^*( \lambda)} \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'')\right].
\end{equation}
During the sampling of the $(\ell+1)$th layer, each sampled path $\lambda \in L_{\ell}$ samples in exactly $m_\lambda \cdot (k/10) \cdot (100\log^2 (n))$ children paths. Using Equation \eqref{eq:sparsificationCongestion}, we can see the fractional congestion $\sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'')$ as a sum of independent random variables that take value between 0 and 
\begin{equation*}
    \frac{\tilde y( \lambda) }{ y^*( \lambda)} \cdot \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'') \leq \tilde y( \lambda)=\frac{m_\lambda}{(100 \log^2 (n))^{\ell+1}}.
\end{equation*} (note that we the fact that $y^*$ satisfies constraint \eqref{eqLP:flowLPcapacity}). We can even assume that each random variable takes value at most $\frac{1}{(100 \log^2 (n))^{\ell+1}}$ by thinking of each of the $m_\lambda$ copies of $\lambda$ that are chosen as a $m_\lambda$ distinct paths. What remains to do is to compute the expectation of the sum of those random variables. To this end, notice that for every $\lambda \in D(\lambda')\cap L_{\ell+1}$, the random variable $\tilde y(\lambda)$ has expectation 
\begin{align*}
    \mathbb E[\tilde y(\lambda)] &= m_{P(\lambda)}\cdot (k/10) \cdot (100 \log^2 (n)) \cdot \frac{y^*_{\mid  P(\lambda)}(\lambda)}{\sum_{\lambda' \in L_{\ell+1}} y^*_{\mid P(\lambda)}(\lambda')} \cdot \frac{1}{(100\log^2 (n))^{\ell+1}}\\
    &=m_{P(\lambda)}\cdot (k/10) \cdot \frac{y^*_{\mid  P(\lambda)}(\lambda)}{\sum_{\lambda' \in L_{\ell+1}} y^*_{\mid P(\lambda)}(\lambda')} \cdot \frac{1}{(100\log^2 (n))^{\ell}}\\
    &=m_{P(\lambda)} \cdot (k/10) \cdot \frac{y^*_{\mid  P(\lambda)}(\lambda)}{k \cdot Y^*_\ell(P(\lambda))} \cdot \frac{1}{(100\log^2 (n))^{\ell}}\\
    &=\frac{m_{P(\lambda)}}{10}\cdot \frac{y^*_{\mid  P(\lambda)}(\lambda)}{Y^*_\ell(P(\lambda))}\cdot \frac{1}{(100\log^2 (n))^{\ell}}\\
    &=\frac{1}{10}\cdot \tilde y(P(\lambda)) \cdot \frac{y^*_{\mid  P(\lambda)}(\lambda)}{Y^*_\ell(P(\lambda))} = \frac{y^*_{\mid  P(\lambda)}(\lambda)}{10}.
\end{align*}
(we used constraint \eqref{eqAggregateLP:demandbottom} from the second to third lines). By linearity of expectation, we obtain
\begin{align*}
     \mathbb E[ \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'')] &= \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}} \left[\frac{\mathbb E[\tilde y( \lambda)] }{ y^*( \lambda)} \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'')\right]\\
     &= \frac{1}{10}\cdot \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}} \left[\frac{y^*_{\mid  P(\lambda)}(\lambda)}{ y^*( \lambda)} \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'')\right]\\
      &= \frac{1}{10}\cdot \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}} \left[\frac{y^*(\lambda)\cdot \tilde y(P(\lambda))}{y^*(\lambda)\cdot y^*(P(\lambda))} \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'')\right]\\
      &= \frac{1}{10}\cdot \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}}  \sum_{\lambda '' \in D(\lambda)\cap A(v)}y^*(\lambda'')\cdot \frac{\tilde y(P(\lambda))}{y^*(P(\lambda))}\\
      &=\frac{1}{10}\cdot \sum_{\lambda \in D(\lambda')\cap L_{\ell+1}}  \sum_{\lambda '' \in D(\lambda)\cap A(v)} y_{\mid P(\lambda)}(\lambda'')\\
      &= \frac{1}{10}\cdot \sum_{\lambda'' \in D(\lambda')\cap A(v)} Y_\ell^*(\lambda'') \le \frac{1}{5}Y_\ell^*(\lambda').
\end{align*}
(we used constraint \eqref{eqAggregateLP:capacitytop} in the last line). The desired random variable can therefore be seen as a sum of independent random variables that each take a value at most $\frac{1}{(100\log^2 (n))^{\ell+1}}$ and whose total expectation is at most $\frac{1}{5}Y_\ell^*(\lambda')\le Y_\ell^*(\lambda')$. By constraint \eqref{eqAggregateLP:granularity} and induction hypothesis, we have that $Y_\ell^*(\lambda')$ is a integer multiple of $\frac{1}{(100 \log^2 (n))^{\ell}}$. If $Y_\ell^*(\lambda')=0$, the constraints remain satisfied with probability 1. Otherwise, by a standard Chernoff-Hoeffding bound (see Theorem \ref{chernoff}), we have that $ \sum_{ \lambda''\in A(v)\cap D( \lambda')} Y^*_{\ell+1}(\lambda'')$ is more than $2Y_\ell^*(\lambda')$ with probability less than 
\begin{equation*}
    \exp \left[-3Y_\ell^*(\lambda')\cdot (100 \log^2(n))^{\ell+1} \right] \le \exp(-300\log^2(n)).
\end{equation*}
There are at most $n^{h+1}\le \exp(2\log^2(n))$ such constraints to maintain hence by a simple union bound, none of these is violated with probability at least $1-\exp(-298 \log^2(n))\geq 1-1/n^{298}$.
\paragraph{Constraints \eqref{eqAggregateLP:granularity}, \eqref{eqAggregateLP:root}.} These constraints are clearly satisfied by the definition of our sampling procedure.
\end{proof}

By applying Lemma \ref{lem:sparsify} with $\ell=h$, we obtain the desired solution $\tilde y$ with high probability. 

==> deleted/deletedROUNDING.tex <==
\section{New and Improved Randomized Rounding}

This is a $\mathrm{poly}(\log\log n + \log k)$-approximation for
max-min degree arborescence. It seems like removing $\log k$ should be possible,
but requires some more technical effort.
First high level ideas:

\paragraph{Locally Consistent Solution.}
We say that a solution is locally consistent any subtree
of height $\approx \log k \cdot \log\log n$
has maximum congestion $\le O(\log\log n)$.
If we find a locally consistent solution, which has also maximum congestion $\log n$,
we can transform it to a (truly) low congestion solution,
because for various occurrences of the same vertex
the sets of $\log k \cdot \log\log n$ nearest ancestors are mostly
disjoint. It is therefore unlikely that many of
them survive. LLL should work here.

\paragraph{Sparsification.}
We perform randomized rounding in the preprocessing already,
but give each vertex $\log n$ many configurations
with $k/2$ elements each (weighted $1/\log n$ each).
W.h.p.\ each player has congestion $O(1)$.
We get a set of configurations $\mathcal C$, where each configuration in layer $i$
is specified by a set of $k/2$ players and a path from a layer $1$ player to it
(at most $h$ many other configurations). In particular, there could be multiple configurations
with the same set of players, which are still considered as being different.

\subsection{Computing locally consistent solution}

Perform sparsification as described above.
Let $L_1,\dotsc,L_h$ be the configurations is layers $1,\dotsc,h$.
We write $\mathrm{des}(C)$ for all descendants of $C$, $\mathrm{child}(C)$ for all children.
We assume that in layer $1$ there is a ``pseudo-configuration'' $R$ corresponding to the root.
For some $C$ and $v$ we denote by $\mathrm{dist}(C, v)$ the number of layers between configuration $C$ and vertex $v$.
With high probability, we get a solution for the following system.
\begin{align*}
    \sum_{\substack{C' \in \mathrm{des}(C): \\ v\in C'}} x_{C'} &\le 2 x_C &\forall C, v \\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &\ge \frac{k}{2} x_C &\forall C, \text{ where $C$ is not a terminal} \\
    x_{C'} &\in \{\frac{x_C}{\log n}, \frac{2x_C}{\log n},\dotsc, x_C\} &\forall C, C'\in \mathrm{child}(C) \\
    x_R &= 1 &
\end{align*}
We want to round now layer by layer, maintaining
the following set of constraints at some iteration $\ell$.
\begin{align*}
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le \log k \cdot \log^3\log n \cdot x_C &\forall C\in L_{1}\cup\cdots\cup L_{\ell} \text{ and } v \text{ with } \mathrm{dist}(C, v) \le \log\log n \\
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le \log^3 n \cdot x_C &\forall C\in L_{1}\cup\cdots\cup L_{\ell} \text{ and } v \text{ with } \mathrm{dist}(C, v) > \log\log n \\
    \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} &\le 2 x_C &\forall C\in L_{\ell+1}\cup\cdots\cup L_h, v \\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &\ge \frac{k}{4} x_C &\forall C, \text{ where $C\in L_{1}\cup\cdots\cup L_{\ell}$ is not a terminal} \\
    \sum_{C' \in \mathrm{child}(C)} x_{C'} &\ge \frac{k}{2} x_C &\forall C, \text{ where $C\in L_{\ell+1}\cup\cdots\cup L_h$ is not a terminal} \\
    x_{C'} &\in \{\frac{x_C}{\log n}, \frac{2x_C}{\log n},\dotsc, x_C\} &\forall C, C'\in \mathrm{child}(C) \\
    x_{C} &\in \{0, 1\} &\forall C\in L_1\cup \cdots \cup L_\ell \\
    x_R &= 1 &
\end{align*}
We perform the following rounding to round $L_{\ell+1}$:
for each $C\in L_{\ell}$, pick $k/4$ configurations $C'\in \mathrm{child}(C)$
independently with probability proportional to $x_{C'} / 2$.
This intuitively removes half of the children of $C$.
Then scale up the remaining descendants of $C$ by $1/x_{C'}$.
We will show with LLL that with positive probability the constraints remain valid.

Call the new rounded variables $x'_C$.
Consider the constraint for $C, v$. If $C$ is below layer $L_{\ell}$,
it must remain valid. Otherwise, $x_C$ was rounded to $1$ before and
\begin{equation*}
    \mathbb E[ \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x'_{C'} ] = \frac 1 2 \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'}
\end{equation*}
In order to violate the constraint, this expectation has to be exceeded by
\begin{equation*}
    \frac 1 2 \log k \cdot \log^3\log n \quad \text{or} \quad \frac 1 2 \log n ,
\end{equation*}
depending on the distance between $C$ and $v$.
Intuition why this is unlikely: This is a sum of independent variables $\le O(1)$.
Hence, probability is $\le \exp(-\Omega(\log k \cdot \log^3\log n))$ or $\le \exp(-\Omega(\log n))$.
However, for low distance this does not give us high (inversely polynomial) probability.
Hence, we need to bound dependencies and use LLL.

For fixed $C, v$ we split $\mathrm{desc}(C) \cap L_\ell$ into groups depending on how
much congestion they are expected to put on $v$. More precisely, let $G_{C,v,t}$
be the set of all $C'\in \mathrm{desc}(C) \cap L_\ell$ with $v\in C$ and
\begin{equation*}
   \sum_{\substack{C' \in \mathrm{des}(C):\\ v\in C'}} x_{C'} \in [2^{-(t+1)}, 2^{-t})
\end{equation*}
We can assume that $t \le \log^2 n$ and even $t\le \log^2 \log n$ if $\mathrm{dist}(C, v) \le \log\log n$, since too high fractionality cannot occur
(due to pre-rounding / sparsification). We define as a bad event that
\begin{equation*}
     \sum_{G_{C,v,t}} x'_{C'} - \mathbb E[\sum_{G_{C,v,t}} x'_{C'}] >
     \begin{cases}
        \log k \cdot \log\log n &\text{ if } \mathrm{dist}(C, v) \le \log\log n \\
        \log n &\text{ if } \mathrm{dist}(C, v) > \log\log n \\
     \end{cases}
\end{equation*}
The probability of this is $\le$
\begin{equation*}
    k^{- \Omega(2^t \log\log n)} \quad \text{and} \quad n^{-\Omega(2^t)} \text{, respectively}.
\end{equation*}
Because of the number of $t$'s excluding these bad event suffices to guarantee
that the constraints remain valid. We will set the values for LLL
(asymmetric version) as these probabilities scaling down the exponent
by a constant factor.

Let us now bound the dependencies. First, consider the bad event that depend
on one particular configuration variable. There can only be $2^t k^{\log\log n}$
vertices depending on it that are at distance $\le \log\log n$ for one
particular $t$ and only $n^{O(1)}$ with big distance. We argue that the product over $(1 - x(B))$ for each such
bad event is at least $1 - 1/\log^{10} n$.

One bad event for $C, v, t$ can only depend on $\le 2^t \log k \cdot \log^3\log n$
configurations if distance is $\le \log\log n$ and $\le 2^t \log^3 n$ otherwise.
The probability of the bad event is less than $1 - 1/\log^{10} n$ raised
to the power of this number, which finishes the proof.

\subsection{Deriving a globally consistent solution}
Assume locally consistent solution with low congestion such that in
every subtree of height $2\log\log n$ there is congestion $\log^{O(1)}\log n \cdot \log k$.
Split layers into consecutive groups of $\log\log n$ layers each.
Remove randomly half of the children of each vertex (TODO: Add Thanos reference).
An occurrence of a vertex in the tree is considered eliminated if
one of the ancestors in the previous group of $\log\log n$ layers is deleted.
Note that the occurrence can also be eliminated by other deletions, but
this is to bound the dependencies. Probability that an occurrence is deleted is
$1/\log n$. Dependencies are low, show with LLL that w.h.p. only $\log\log n \cdot \log k$ occurrences survive


\section{Randomized Rounding}

Assume we have a solution $x$ to $h = \log n$ many rounds of Lasserre
for the naive assignment LP. We round it as follows. At the root 
we repeat the following $k/2$ times: select a child
with probability proportional to the LP variables,
then recurse on the child with an LP solution $x'$ where we 
condition on taking this child.

This will create a flow that starts at the root and then
in each layer each flow unit splits up into $k/2$ flow units.
There is a one-to-one map of flow units (in some level $\ell$) 
to tuples $(i_1, i_2, \dotsc, i_\ell)$, where $i_1\in \{1,2,\dotsc,k/2\}$ describes
that this flow unit originates in the $i_1$th child picked at
the root, the $i_2$th child of that child, etc.

Equivalently we can imagine the random rounding to happen
in a breadth-first way, that is, layer by layer.
With this intuition we write $x^{(0)} = x$ and denote by $x^{(1)}$
the sum of all $x'$ (as above) from the $k/2$ children of the root.
Similarly we define $x^{(2)},\dotsc,x^{(h)}$.
We write $x^{(\ell)}(\delta^{-1}(v)) = \sum_{(v', v)\in \delta^{-1}(v)} x^{(\ell)}_{v'v}$.
Notice that when conditioning on the outcome of the first $\ell-1$ layers,
the random variable $x^{(\ell)}(\delta^{-1}(v))$---for a vertex $v$ in layer $\ell$ or
below---is the sum of
independent variables with value $\le 1$ and total expectation $1/2 \cdot x^{(\ell-1)}(\delta^{-1}(v))$.

We say that a flow unit $f = (i_1,i_2,\dotsc,i_{\ell})$ is bad if either
\begin{enumerate}
    \item a fraction $\ge 1/2$ of its $k/2$ children have total congestion $\ge \sqrt{\log n}$,
    \item a fraction $\ge 1 - 1/\sqrt{\log n}$ of its $k/2$ children are bad, or
    \item a fraction $\ge 1/4$ of its $k/2$ children are bad and a fraction $\ge 1/(2\sqrt{\log n})$ has congestion $\ge \log^{0.01} n$.
\end{enumerate}
A flow unit is good if it is not bad. Additionally, a flow unit $f = (i_1,i_2,\dotsc,i_{\ell})$ ending at a leaf is never bad.
Our goal is to prove that the root is good with constant probability.
From the set of good flow units we can then derive a $O(\log^{0.51} n)$-approximate solution:
Each bad flow unit we delete; for each good flow unit we scale down the flow to its
parent(s) by its congestion. It remains to show that the incoming flow (from its children)
of each good flow unit is still high.
Consider a good flow unit and the corresponding vertex $v$. Then either $\le 1/4$ of its children are bad or $\le 1/(2\sqrt{\log n})$ of them have congestion $\ge \log^{0.01} n$.
In the first case we also have that $\ge 1/2$ of the children have congestion
$\le \sqrt{\log n}$, which implies that $\ge 1/4$ of the children are not bad
and have a congestion $\le \sqrt{\log n}$. This means the incoming flow of $v$
is $\ge k/8 \cdot 1/\sqrt{\log n}$.
In the second case we have that $\le 1/(2\sqrt{\log n})$ of the children have
congestion $\ge \log^{0.01} n$, but also $\le 1 - 1/\sqrt{\log n}$ of the children
are bad. In particular, $1/(2\sqrt{\log n})$ of the children
congestion $\le \log^{0.01} n$ and are good. This means the incoming flow is
$\ge k/2 \cdot 1/(2\sqrt{\log n}) \cdot 1/\log^{0.01} n$.

The intuition of the proof is as follows:
Consider some flow unit $f = (i_1,i_2,\dotsc,i_{\ell})$. We want to show that
with a decent probability (e.g., $1 - 2^{-\sqrt{\log n}}$) it is good.
For the first criteria for badness we get such a statement relatively easily.
The second criteria follows from bounding inductively the probability of badness in
the next layer and increasing it by a factor of $(1 - 1/\sqrt{\log n})^{-1}$,
which is a rate that we can cope with.
The third criteria is the most involved. Intuitively, both of the statements are
unlikely. If they were independent we could easily get a good enough bound on
the probability. However, they might not be.
But in order to have a $\ge 1/4$ fraction of children of
$(i_1,i_2,\dotsc,i_{\ell})$ be bad,
there must be sufficiently many bad descendants, in particular, many flow units 
of the form
$(i_1,i_2,\dotsc,i_{\ell}, i'_{\ell + 1},\dotsc, i'_{\ell + O(\log\log n)})$
must be bad. We have with
high probability (e.g. $1 - 1/n^{100})$) that the congestion of a vertex is never more than $O(\log n)$. Since the congestion is expected to decrease by a factor of $1/2$
every layer, a congestion / dependence essentially vanishes after $O(\log\log n)$
layers. Hence, this event is almost independent.

\subsection{Formal proof.}

We first prove the following simple claims.
\begin{claim}
\label{cla:conditionnal_congestion}
For any $\ell\geq 0$, any flow unit $f\in V_{\ell}\cup V_{\ell+1}\cup \cdots \cup V_h$ and any $c\ge 100$, we have that
\begin{equation*}
    \mathbb P_{x^{(\ell)} \sim D} [ x^{(\ell)}(\delta^{-1}(f)) \ge c] \le  h\cdot 2^{-c/6}.
\end{equation*}
\end{claim}
\begin{proof}
  We condition on the flow unit $f$ arriving at a specific vertex $v\in V_{\ell'}$. Note that after this conditioning, the expected congestion on $f$ (which is the congestion on vertex $v$), is at most $2$. To see this, we can look at the path $(r,u_1,u_2,\ldots , v)$ that the flow unit $f$ took from the root $r$ to $v$. The congestion on vertex $v$ can come from $\ell'+1$ different processes. The first one starts at the root, where $k/2-1$ other flow units $f'=(r,u')$ are sampled. The second starts at vertex $u_1$ where $k/2-1$ other flow units $f'=(r,u_1,u')$ are sampled, and so on. Because of the prefix capacity constraints (\etienne{TODO refer to LP}) and the scaling down by $1/2$ factor, the process starting at the root induces an expected congestion of at most $1/2^{\ell'}$ on vertex $v$. Similarly, the $i$th process creates an expected congestion of at most $1/2^{\ell'-i}$ on vertex $v$. Hence by linearity of expectation, the total expected congestion on vertex $v$ is at most
  \begin{equation*}
      \sum_{i=0}^{\ell'} (1/2)^i \leq 2.
  \end{equation*}
  To analyze the deviation from expectation, we proceed as follows. Denote by $P_i$ the process starting at vertex $u_i$ (with the convention that $u_0=r$ and $u_{\ell'}=v$). At step $0$, we perform one round of randomized rounding of the process $P_0$ (i.e. we move one layer down). At step $1$ we perform one round of $P_0$ and $P_1$. At step $i\leq \ell'$, we perform one round of $P_0,P_1,\ldots , P_{i} $. By a simple Chernoff bound (\etienne{TODO refer to LP}), the probability that one step of the above process deviates from expectation by more than an additive $c-2$ is at most $2^{-(c-2)/2}$. By union bound, it does not deviate by more than $c-2$ at any layer with probability at least $h\cdot 2^{-(c-2)/2}$. Because the deviation from one step of rounding is scaled down by a factor $1/2$ at every step in expectation, this implies that with probability at least $h\cdot 2^{-(c-2)/2}$, the congestion on vertex $c$ will be no more than 
  \begin{equation*}
      2+(c-2)\cdot  \left(\sum_{i=0}^{\ell'} (1/2)^i \right)\leq 2c.
  \end{equation*} This concludes the proof.
\end{proof}

\begin{claim}
\label{cla:congestion}
With probability at least $1-1/n$, no vertex $v$ will have congestion more than $100\log(n)$. 
\end{claim}
\begin{proof}
  Note that the expected congestion on any vertex is at most $1$. By Chernoff bound \etienne{TODO refer to LP}, the probability that at any layer the rounding deviates from expectation by an additive $50\log(n)$ is at most $1/n^{25}$. Hence with probability at most $1/n^{24}$ it deviates from expectation at any layer. This implies that with probability at least $1-1/n^{24}$, the congestion is at most $1+50\log(n)\left(\sum_{i=0}^\infty (1/2)^i \right)\leq 100\log n.$
\end{proof}
Consider a layer $\ell$ and suppose that $x^{(\ell)}$ is drawn from some distribution $D$
such that for each vertex $v\in V_{\ell}\cup V_{\ell+1}\cup \cdots \cup V_h$ we have
\begin{equation*}
    \mathbb P_{x^{(\ell)} \sim D} [ x^{(\ell)}(\delta^{-1}(f)) \ge \sqrt{\log n}] \le 2^{-\sqrt{\log n}} .
\end{equation*}
Notice that this is in particular true for the first layer and the distribution
that always returns the initial solution $x$.
We will prove by induction that for each flow unit $f = (i_1,i_2,\dotsc,i_{\ell})$ we have
\begin{equation*}
    \mathbb P[f \text{ is bad}] \le 2^{-10\sqrt{\log n}} \cdot (1 - 1/\sqrt{\log n})^{\ell-h} .
\end{equation*}
Here the probability is taken over first sampling $x^{(\ell)}$ and then performing
the randomized rounding according to $x^{(\ell)}$. In particular, this
shows that with constant probability the root vertex is good.


\paragraph*{Criteria~1.} Let $i_{\ell+1}\in \{1,2,\dotsc,k/2\}$.
We have with probability $\ge 1 - 2^{-100\sqrt{\log n}}$ that
$x^{(\ell)}(\delta^{-1}(f \circ i_{\ell+1})) \le 100 \sqrt{\log n}$. Condition on this.
Since the congestion of $f \circ i_{\ell + 1}$ is the sum of random variables bounded
by one with expectation $\le 100 \sqrt{\log n}$, we have that with probability
at least $1 - 2^{-100 \sqrt{\log n}}$ the congestion is at most the expected congestion
plus $100 \sqrt{\log n}$, i.e., at most $200 \sqrt{\log n}$ with probability
$1 - 2 \cdot 2^{-100\sqrt{\log n}}$. 

Hence, in expectation $\le 2 \cdot 2^{-100\sqrt{\log n}}$
of the children of $f$ have congestion $\ge 200 \sqrt{\log n}$ and thus with
probability $\ge 1 - 4 \cdot 2^{-100\sqrt{\log n}}$ at most $1/2$ children of $f$
have congestion $\ge 200 \sqrt{\log n}$.

\paragraph*{Criteria~2.} Let $i_{\ell+1}\in \{1,2,\dotsc,k/2\}$.
By induction we have that
\begin{equation*}
    \mathbb P[f \circ i_{\ell + 1} \text{ is bad}] \le 2^{-\sqrt{\log n}} \cdot (1 - 1/\sqrt{\log n})^{h - \ell - 1} =: p .
\end{equation*}
Hence, in expectation only a fraction of $p$ of the children of $f$ are bad.
The probability that $1 - 1/\sqrt{\log n}$ of the children are bad is therefore
at most
\begin{equation*}
    p / (1 - 1/\sqrt{\log n}) = 2^{-\sqrt{\log n}} \cdot (1 - 1/\sqrt{\log n})^{h - \ell} .
\end{equation*}

\paragraph*{Criteria~3.} By the same arguments as in criteria~1, we can prove that
with probability ?? at most $1/(2\sqrt{\log n})$ of the
children of $f$ have congestion $\ge 2 \log^{0.01} n$. We condition on there being more
such children.
Now we would like to show that with decent probability there are not many bad children
of $f$. However, we cannot directly use the induction hypothesis because drawing
$x^{(\ell+1)}$ (one round of randomized rounding) is now biased by the 
conditioning: it might be that some vertices have high congestion with high probability,
because this is positively correlated with $f$ having many congested children.
Instead let $\ell' = \ell + \log\log n$ and analyze the bad descendants of the form
$f' = f \circ (i_{\ell+1}, i_{\ell + 2},\dotsc, i_{\ell'})$.
Drawing $x^{(\ell'})$ by performing $\log\log n$ rounds of randomized rounding we now
have the property that $x^{(\ell')}(\delta^{-1}(v)) \le \sqrt{\log n}$ with
probability $\ge 1 - 2^{-\sqrt{\log n}}$: this can only happen if
there is some $\ell < \ell'' \le \ell'$ with
$x^{(\ell'')}(\delta^{-1}(v)) \ge 1/2 \cdot x^{(\ell'' - 1)}(\delta^{-1}(v)) + 1/2 \cdot \sqrt{\log n}$. By a union bound this does not happen with probability $\ge$
\begin{equation*}
    1 - \log\log n \cdot 2^{-1/2 \sqrt{\log n}} \ge 1 - 2^{-1/4 \sqrt{\log n}}.
\end{equation*}
%This implies that the probability that at least $1/(2\sqrt{\log n})$ children
%of $f$ have congestion $\ge 2 \log^{0.01} n$ \emph{and} more than
%a $2^{-\sqrt{\log n}}$ fraction of descendants $f'$ are bad is at most
%\begin{equation*}
%    \cdot (2^{-1/4 \sqrt{\log n}} + 2^{-\sqrt{\log n}} (1 - 1/\sqrt{\log n})^{h - \ell'}) %. 
%\end{equation*}
This only bounds the value on all vertices, but we have to specifically bound
the value for flow units $f$. Here consider for each flow unit $f = (i_1,i_2,\dotsc,i_{\ell})$
\begin{equation*}
    \sum_{v} \mathbb P[f \text{ arrives at } v] \cdot x^{(\ell)}(\delta^{-1}(v))
\end{equation*}
Conditioning on $f$ arriving at $v$ may bias the distribution $x^{(\ell)}$,
but this can only happen in a limited way: consider separately the randomized rounding
where we omit the recursions at $i_1$, $(i_1,i_2)$, etc. This still has
low expected congestion on $v$ and is independent from this conditioning.
Then add congestion induced by the recursion starting at $i_1$, $(i_1,i_2)$, etc.,
which have expected congestion $1/2^\ell$, $1/2^{\ell-1}$, etc.

\emph{Idea of the rest:} make a union bound with the event that layers
$\ell + 1, \ell + 2, \dotsc, \ell'$ have few bad descendants of $f$ from criteria~1.
Now show that criteria~2 and~3 cannot amplify the fraction of bad flow units much.

\newpage
\section{Reductions}
We start with the following problem
\begin{definition}[max-min degree arborescence]
  Given a directed graph $G = (V, E)$ with sources
  $S\subseteq V$ and sinks $T \subseteq V \setminus S$, find $|S|$ many vertex disjoint arborescences rooted in the
  vertices $S$ such that every node in an arborescence
  that is in $V\setminus T$ has exactly $k$ children.
  Here, $k$ is to be maximized.
\end{definition}
In this section we reduce the general problem to the case
of $|S| = 1$ at a loss of $O(\log h \cdot \log(k \log n))$ in the approximation
rate, but the algorithm for $|S| = 1$ gets another constraint:
for each vertex $v$ there is a set $F_v\subseteq \{1,2,\dotsc,n\}$
and $v$ cannot be used at a distance $f$ from the root for any $f\in F$.

Assuming that $k < 2^{\log^{\epsilon} n}$ (which seems reasonable since otherwise the height cannot be very large), the loss of this reduction
is only roughly $O(\log^{\epsilon} n)$, i.e., negligible.
\subsection{Bounded depth}
First we argue that we may assume at a cost of a factor~$2$
that all arborescences have depth at most $h = O(\log n)$.
Take the optimal solution and delete from each arborescence and each of its nodes half of the children (and their subtrees) uniformly at random. Clearly, the
remaining solution is $2$-approximate.
Now consider some vertex $v$ with distance greater than $\log_2 n$ before the deletions. The probability that none
of its ancestors is deleted is less than $(1/2)^{\log_2 n} = 1/n$. By a union bound, there is a positive probability that all vertices with distance greater than $\log_2 n$
are removed. Hence, there exists a $2$-approximate solution with depth at most $\log_2 n$.

\subsection{Arborescences with overlap}
In this subsection we will use an $\alpha$-approximation for finding
a single arborescence to derive an $O(\alpha)$-approximation for many
arborescences, but we allow that a vertex is used in several arborescences
as long as the distance to the root is different in each one of them.
The algorithm is a local search. The algorithm relies on the following
lemma.
\begin{lemma}
  Consider a set of $g$ many $k$-arborescences $A$ and a set of at most $2g$ many $\le k/4$-arborescences $B$. Then there is a $k/4$-arborescence that forms a subset of some arborescence in $A$ and does not overlap with $B$
  on a vertex at the same distance from a root.
\end{lemma}
\begin{proof}
  The set $B$ has at most $2 g \cdot (k/4)^h \le 3 g \cdot (k/4)^h$ many vertices at distance $h$ from some root. If they appear at distance $h$ in $A$, then we delete them from $A$. If now a vertex in $A$ at distance $h-1$ has less than $k/4$ children, we delete this vertex as well. This way we can delete at most $3 g \cdot (k / 4)^h / (3/4 k) \le g \cdot (k / 4)^{h-1}$ vertices at distance $h-1$. Then we remove also the $2g \cdot (k / 4)^{h-1}$ vertices that may appear in $B$ at distance $h-1$, which removes a total of at most $3 g \cdot (k / 4)^{h-1}$ vertices at distance $h-1$. Repeating this argument we remove at most $3g \cdot (k / 4)$ vertices at distance $1$. Consequently, some root with many children
  must remain.
\end{proof}

The local search now works as follows. Assume we already covered some
roots and we want to add another arborescence for root $r \in S$.
\begin{enumerate}
    \item let $S' \subseteq S$ initialized as $\{r\}$
    \item let $B$ be a set of arborescences initialized with $\emptyset$
    \item loop
    \begin{enumerate}
    \item $A \gets \mathrm{nil}$
    \item for $s\in S'$ do
    \begin{enumerate}
        \item A $\gets$ $\alpha$-approximation for $s$ to find $(1/4 \cdot k/\alpha)$-arborescence with $F_v$ defined as the set distances that $v$ appears already in $B$
        \item if $A \neq \mathrm{nil}$ (algorithm was successful): break
    \end{enumerate}
    \item if $A = \mathrm{nil}$ return ``Fail''
    \item if $A$ does not overlap with any arborescences in current solution:
    \begin{enumerate}
        \item add $A$ to solution, backtrack, etc. (todo: details)
    \end{enumerate}
    \item else:
    \begin{enumerate}
        \item Add $A$ to $B$
        \item Add overlapping arborescences to $B$ and their roots to $S'$
    \end{enumerate}
    \end{enumerate}
\end{enumerate}
At all times the number of arborescences in $B$ is at most $2 |S'|$.
By the previous lemma there always exists a $1/4 \cdot k$-arborescence
from OPT that can be added.

\subsection{Final touches}
From the previous subsection we have a set of arborescences, where
one vertex might be used by multiple arborescences, but only at different
distances (in particular, at most $h = \log n$) times.
Of each arborescence and each of its vertices we remove
$1/2$ of its children uniformly at random. We will show
that with positive probability each vertex is now used in
only $O(\log h \cdot \log (k \log n))$ arborescences.
We will use the asymmetric Lov\'asz Local Lemma for this.

We define the following bad events: for a vertex $v$
and some $\ell = 2^i, \ell \le h$ the event $B_{v,\ell}$
is that $v$ appears in more than $5\log(k \log n)$ arborescences
at a distance in $[\ell, 2\ell)$ from the root.
There are only such events for $\ell \ge 5\log(k \log n) \ge \log h$, since other the events can never occur.
Vertex $v$ appears in at most $\log n$ arborescences
before the deletions and
$B_{v,\ell}$ can correlate only with bad events for vertices $u$ that appear in one of these arborescences.
For every $\ell'$ the number of such bad events is at most
\begin{equation*}
    \log n \cdot \sum_{i = \ell}^{2\ell - 1} k^{i} \le \log n \cdot k^{2\ell} \le (k \log n)^{2\ell}.
\end{equation*}
For each bad event $B_{v, \ell}$ we set
\begin{equation*}
    x(B_{v, \ell}) = (k \log n)^{-2\ell} .
\end{equation*}
\begin{lemma}
For each $v, \ell$ it holds that $\mathbb P[B_{v, \ell}] \le x(B_{v, \ell}) / h^2$ .
\end{lemma}
\begin{proof}
  Let $O$ be a set of occurrences of $v$ at distance in 
  $[\ell, 2\ell)$ from some arborescence's root
  with $|O| = \log(k \log n)$.
  Each occurrence is in a different arborescence,
  hence it being deleted is independent from other
  occurences. The probability that none of them are
  deleted is at most
  \begin{equation*}
      (2^{-\ell})^{|O|} = 2^{-\ell \cdot 5 \log(k \log n)} = (k \log n)^{-5\ell} .
  \end{equation*}
  The number of such sets
  $O$ is at most $\ell^{\log(k \log n)} = (k \log n)^{\log \ell}$. By a union bound we have that the probability
  that $\log(k \log n)$ occurrences are not deleted is
  at most
  \begin{equation*}
      (k \log n)^{\log \ell} \cdot (k \log n)^{-5\ell} \le (k \log n)^{-4\ell} .
  \end{equation*}
  Since $\ell \ge \log h$ the statement of the lemma follows.
\end{proof}
\begin{lemma}
  For some $\ell'$ let $U$ be the vertices $u$ in events
  $B_{u,\ell'}$ that correlate with $B_{v, \ell}$.
  Then
  \begin{equation*}
      \prod_{u \in U} (1 - x(B_{u,\ell'})) \ge 1/e .
  \end{equation*}
\end{lemma}
\begin{proof}
  We have that $|U| \le (k \log n)^{2\ell'}$ and $x(B_{u,\ell'}) = (k \log n)^{-2\ell'}$.
\end{proof}
Let $\Gamma(B_{v,\ell})$ be the bad events that correlate with $B_{v, \ell}$.
We conclude that
\begin{equation*}
    \mathbb P[B_{v,\ell}] \le x(B_{v, \ell}) \cdot \frac{1}{h^2} \le x(B_{v, \ell}) \prod_{\ell'} \frac{1}{e} \le x(B_{v, \ell}) \prod_{B\in \Gamma(B_{v,\ell}} (1 - x(B)) .
\end{equation*}
By LLL there is a positive probability that none of the bad events occur.

\etienne{COPY}

==> deleted/deleteddiscussion.tex <==
We first claim the following.
\begin{claim}
\label{cla:sink_degree}
With high probability, no vertex $i\in L_\ell$ is connected to more than $2(\log^5(n))^{\ell-1-j}$ leaves in layer $\ell-1$ that belong to the subtree rooted at a vertex $v\in L_j$ for some $j\leq \ell-1$.
\end{claim}
\begin{proof}
To see this, note that during the random process initiated by vertex $i$, every internal node that was selected selects in expectation $\log^{10}(n)/\log^5(n)=\log^5(n)$ of its children. By a standard Chernoff bound (see Theorem \ref{chernoff}) the probability that this internal nodes selects more than 
\begin{equation*}
    \left(1+\frac{1}{\log n}\right)\cdot \log^5(n)
\end{equation*} of its children is at most 
\begin{equation*}
    \exp\left(-\frac{1}{3\log^2 (n)}\cdot \log^5 (n) \right)\le \exp\left(-\log^3(n)/3 \right).
\end{equation*}
Therefore with high probability, no internal node selects more than $\left(1+\frac{1}{\log n}\right)\cdot \log^5(n)$ of its children which implies that the total number of selected nodes at layer $\ell-1$ that belong to the subtree $T_v$ (which are exactly the neighbors of $i$ in that subtree) is at most
\begin{align*}
     \left(1+\frac{1}{\log n}\right)^{\ell-1-j}\cdot (\log^5(n))^{\ell-1-j}&\le \exp\left(\Theta \left(\frac{\log n}{\log (n)\log \log (n)}\right) \right)\cdot (\log^5(n))^{\ell-1-j}\\
     &\le 2(\log^5(n))^{\ell-1-j}.
\end{align*}
\end{proof}



%%%%%%%



\newpage
However, one simple but crucial difference in our approach compared to theirs is that we scale down the probabilities of sampling by a constant factor. In previous works, when a path $\lambda$ is sampled, then this path samples exactly $k$ children $\lambda'$, each with probability $y(\lambda')/y(\lambda)$ whereas we allow ourselves to choose only $k/2$ children but each path $\lambda'$ is taken with probability only $y(\lambda')/(2y(\lambda))$. Then they argue with this sampling that no vertex has congestion more than $\textrm{polylog} (n)$ to obtain a $\textrm{polylog} (n)$ approximation factor. Below we prove a lemma that shows that it is seems difficult to get below $\tilde \Omega (\log n)$ factor with this approach.

\begin{lemma}
\label{lem:congestion_previousworks}
There exists a graph of depth $\Theta \left(\frac{\log n }{\log \log n}\right)$ where the rounding described above produces an integral solution where all vertices in the last layer have congestion $\Omega \left(\frac{\log n}{\log \log n} \right)$.
\end{lemma}
\begin{proof}
The graph will have $\ell+1$ layers labeled from 0 to $\ell$. $n$ will be the number of vertices in the last layer and we choose $\ell=\Theta \left(\frac{\log n}{\log \log n}\right)$ so that $(\log^5(n))^{\ell}=n$. The set of sinks is all the vertices in the last layer. The graph until layer $\ell-1$ is a complete and regular tree where every internal vertex has $\log^{10} (n)$ children. Below we describe how we connect layer $\ell-1$ to layer $\ell$. Each vertex $i\in L_\ell$ runs the following sampling process, independently of other vertices.
Start at the root $r$. From the root select each vertex $v$ at level 1 independently at random with probability $1/\log^5 (n)$. All the vertices at level 2 whose parent was selected is then selected independently at random with probability $1/\log^5 (n)$. We repeat layer by layer, each vertex in layer $t$ whose parent was selected is then selected independently at random with probability $1/\log^5 (n)$.

Finally, connect the vertex $i\in L_\ell$ to all vertices in layer $L_{\ell-1}$ that were selected by the above random process for vertex $i$.







Moreover, each vertex $j$ in layer $\L_{\ell-1}$ is connected to each vertex $i\in L_\ell$ independently with probability $1/(\log^5(n))^{\ell-1}$ therefore with high probability each vertex $j$ has at least 
\begin{equation*}
    \frac{n}{2(\log^5(n))^{\ell-1}}=\frac{\log^5 (n)}{2}
\end{equation*} many neighbors in layer $\ell$.

\begin{claim}
\label{cla:flowLPfeasible}
With high probability, the flow LP is feasible on this instance for $k=\frac{\log^{5}(n)}{4}$.
\end{claim}
\begin{proof}
We set the following fractional values.
\begin{equation*}
    y(\lambda)=
    \begin{cases}
    \frac{1}{2(\log^5(n))^{\ell-1}} & \textrm{ if $\lambda$ ends at layer $\ell$}\\
     \frac{1}{(\log^5(n))^{j}} & \textrm{ if $\lambda$ ends at layer $j\le \ell-1$}
    \end{cases}
\end{equation*}
Clearly, $y((r))=1$. We check the demand constraints easily, let $\lambda$ be a path that ends at layer $j\leq \ell-2$, then
\begin{equation*}
     \sum_{\substack{\lambda':\\ \lambda'\textrm{ is a children of } \lambda}} y(\lambda') =  \log^{10}(n)\cdot \frac{1}{(\log^5(n))^{j+1}} = \log^{5}(n) \cdot \frac{1}{(\log^5(n))^{j}}\ge \left(\frac{\log^{5}(n)}{4}\right)\cdot y(\lambda).
\end{equation*}
If $\lambda$ ends at layer $\ell-1$, then with have probability we have
\begin{equation*}
    \sum_{\substack{\lambda':\\ \lambda'\textrm{ is a children of } \lambda}} y(\lambda') \ge \frac{\log^5 (n)}{2} \cdot  \frac{1}{2(\log^5(n))^{\ell-1}} \ge \left(\frac{\log^{5}(n)}{4}\right) \cdot y(\lambda).
\end{equation*}
The capacity constraints are also easily verified with high probability.
Let $v$ be a vertex in layer $j\leq \ell-1$ and $\lambda$ a path ending in layer $j'\le j$ then
\begin{equation*}
    \sum_{\substack{\lambda': \lambda' \textrm{ ends at vertex }v,\\ \lambda'\textrm{ is a descendant of } \lambda}} y(\lambda') = \frac{1}{(\log^5(n))^{j}}\le \frac{1}{(\log^5(n))^{j'}}=y(\lambda).
\end{equation*}
If $v$ is a vertex in layer $\ell$ and $\lambda$ a path ending in layer $j'\le \ell$ then, using Claim \ref{cla:sink_degree}, we obtain
\begin{equation*}
     \sum_{\substack{\lambda': \lambda' \textrm{ ends at vertex }v,\\ \lambda'\textrm{ is a descendant of } \lambda}} y(\lambda') \leq (2(\log^5(n))^{\ell-1-j}) \cdot \frac{1}{2(\log^5(n))^{\ell-1}}=\frac{1}{(\log^5(n))^{j}} = y(\lambda). 
\end{equation*}
\end{proof}

By similar arguments, it is clear that the rounding procedure of \cite{bateni2009maxmin,chakrabarty2009allocating} will select until layer $\ell-1$ an integral tree where every vertex has at least
\begin{equation*}
   d:= \left(1-\frac{1}{\log n} \right)\cdot \log^5(n)
\end{equation*} many children. We finish the proof with the following claim.

\begin{claim}
\label{cla:integraltree}
With high probability, any tree $T$ with leaves at layer $\ell-1$ and in which every vertex has 
\begin{equation*}
    \left(1-\frac{1}{\log n} \right)\cdot \log^5(n)
\end{equation*} many children is connected to at most 
\begin{equation*}
    \frac{3}{\ell} \cdot \log(n)^{5\ell}
\end{equation*} many vertices in layer $L_\ell$.
\end{claim}




%%%%%%%%%%%



Given Lemma \ref{lem:congestion_previousworks}, it is clear that the previous techniques cannot hope to get below a $\tilde \Omega (\log n ))$ approximation factor. One might be tempted to first compute the integral solution as in previous works and then prune the high congestion vertices. For the sake of the argument let's assume we want to prune all the vertices that have congestion more than $\log^{1-\epsilon} (n)$ for some small fixed $\epsilon>0$ in the hope to get a $O(\log^{1-\epsilon} (n))$ approximation factor. However, to maintain this approximation factor, we must notice that pruning down vertices in some layer $j$ might delete a lot of children of some other vertices in layer $j-1$. To ensure that every vertex still has enough children, we should prune iteratively from the bottom layer to the top, where at each layer $j$ we remove all vertices that have congestion more than $O(\log^{1-\epsilon} (n))$ or such that more less than a $\beta$ fraction of its children survived. The final approximation ratio would then be $O(\beta \log^{1-\epsilon} (n))$. An easy way to think about this process would be to imagine that the algorithm chooses a perfect complete $k$-ary tree with congestion at most $1$ on all vertices but then we allow an adversary to delete some fraction $\alpha$ of our vertices. This will then trigger some deletions that will propagate through the layers until the root because we would like to delete all vertices that have less than a $\beta$ fraction of their children surviving.
Unfortunately, we argue below that if we argue against an adversary that can corrupt vertices it might have catastrophic effects on our tree even if the adversary is allowed to remove only a very small fraction of the leaves of our tree.

Indeed, a simple argument for this pruning would go as follows. If we allow an adversary to delete at most an $\alpha$ fraction of our leaf vertices in the last layer $L_\ell$, then it could be that a 
\begin{equation*}
    \frac{\alpha}{1-\beta}
\end{equation*} fraction of the vertices in layer $L_{\ell-1}$ loose more than a $1-\beta$ of their children. If this does not seem a lot at first, this small error will amplify as we repeat the argument across the layers. Indeed, we soon realize that it could be that a 
\begin{equation*}
      \frac{\alpha}{(1-\beta)^{\ell-1}}\approx \alpha \cdot \exp \left(\ell \cdot \beta \right)
\end{equation*} fraction of the children of the root are deleted in the process.

As a simple example, notice that if $\ell = \Theta (\log n /  \log \log n)$, then we would delete a fraction of $\alpha \cdot \exp \left(\ell \cdot \beta \right)$.
